Testing Models of Stellar Structure and Evolution I. Comparison with Detached Eclipsing Binaries

We present the results of an analysis aimed at testing the accuracy and precision of the PARSEC v1.2S library of stellar evolution models, in a Bayesian framework, to infer stellar parameters. We mainly employ the online DEBCat catalogue by Southworth, a compilation of detached eclipsing binary systems with published measurements of masses and radii to $\sim$ 2 per cent precision. We select a sample of 318 binary components, with masses between 0.10 and 14.5 Msun, at distances between 1.3 pc and ~ 8 kpc for Galactic objects and ~ 44-68 kpc for extragalactic ones. The Bayesian analysis applied takes as input effective temperature, radius, and [Fe/H], and their uncertainties, returning theoretical predictions for other stellar parameters. From the comparison with dynamical masses, we conclude that the inferred masses are precisely derived for stars on the main-sequence and in the core-helium-burning phase, with uncertainties of 4 per cent and 7 per cent, respectively, on average. Masses for subgiants and red giants are predicted within 14 per cent, and those for early asymptotic giant branch stars within 24 per cent. These results are helpful to further improve the models, in particular for advanced evolutionary stages for which our understanding is limited. We obtain distances and ages for the binary systems and compare them, whenever possible, with precise literature estimates, finding excellent agreement. We discuss evolutionary effects and challenges for inferring stellar ages from evolutionary models. We also provide useful polynomial fittings to theoretical zero-age main-sequence relationships.

==> tables_electronic_version.tex <==
\begin{landscape}
 \begin{table}
  \caption{
Literature stellar parameters of DEB stars in Sample I, with known metallicities: radius ($R$), effective temperature ($T_{eff}$), 
iron abundance [Fe/H], and mass ($M$), surface gravity ($\log g$), luminosity ($\log L$), spectral type ($SpT$)/luminosity class ($LC$), 
color excess $E(B-V)$, and distance $d$. 
References for the literature values are given in the main text.
}
%{\tiny
  \label{tab:sampleI}
  \begin{tabular}{ccccccccccc}
    \hline
    System & $R$               & $T_{eff}$ & [Fe/H]      & $M$              & $\log g$              &  $\log L$                 &  $SpT/LC$  & $E(B-V)$        &  $d$             \\
                 & ($R_{\sun}$) & ($\,K$)     & ($dex$)   &  ($M_{\sun}$) & ($g$: cm s$^{-2}$)  & ($L$:  $L_{\sun}$)     &                    & ($mag$)         &  ($pc$)      \\
    \hline
CM Dra & 0.2534 $\pm$ 0.0019 & 3133 $\pm$ 72 & -0.30 $\pm$ 0.12 & 0.2310 $\pm$ 0.0009 & 4.994 $\pm$ 0.007 & -2.25 $\pm$ 0.04 & M4.5V & 0 & 14.850 $\pm$ 0.011 \\
                        & 0.2396 $\pm$ 0.0015 & 3119 $\pm$ 101 & $\shortparallel$ & 0.2141 $\pm$ 0.0009 & 5.009 $\pm$ 0.006 & -2.31 $\pm$ 0.06 & M4.5V & $\shortparallel$ & $\shortparallel$ \\
PTFEB 132.707+19.810 & 0.363 $\pm$ 0.008 & 3258 $\pm$ 90 & 0.14 $\pm$ 0.04 & 0.3953 $\pm$ 0.0020 & 4.915 $\pm$ 0.019 & -1.87 $\pm$ 0.05 & M3.5V & 0 & 187 $\pm$ 3 \\
                        & 0.272 $\pm$ 0.012 & 3119 $\pm$ 108 & $\shortparallel$ & 0.2098 $\pm$ 0.0014 & 4.89 $\pm$ 0.04 & -2.20 $\pm$ 0.07 & M4.3V & $\shortparallel$ & $\shortparallel$ \\
HAT-TR-318-007 & 0.455 $\pm$ 0.004 & 3192 $\pm$ 110 & 0.30 $\pm$ 0.11 & 0.4480 $\pm$ 0.0010 & 4.774 $\pm$ 0.006 & -1.71 $\pm$ 0.06 & M4V & 0 & 119.8 $\pm$ 1.1 \\
                        & 0.2913 $\pm$ 0.0024 & 3097 $\pm$ 107 & $\shortparallel$ & 0.272 $\pm$ 0.004 & 4.944 $\pm$ 0.004 & -2.15 $\pm$ 0.06 & M5V & $\shortparallel$ & $\shortparallel$ \\
YY Gem & 0.620 $\pm$ 0.006 & 3819 $\pm$ 97 & 0.10 $\pm$ 0.20 & 0.597 $\pm$ 0.005 & 4.630 $\pm$ 0.008 & -1.13 $\pm$ 0.04 & M1Ve & 0 & 15.098 $\pm$ 0.012 \\
                        & 0.604 $\pm$ 0.006 & 3819 $\pm$ 97 & $\shortparallel$ & 0.601 $\pm$ 0.005 & 4.66 $\pm$ 0.05 & -1.16 $\pm$ 0.04 & M1Ve & $\shortparallel$ & $\shortparallel$ \\
M55 V54 & 1.006 $\pm$ 0.009 & 6252 $\pm$ 72 & -1.86 $\pm$ 0.15 & 0.726 $\pm$ 0.015 & 4.294 $\pm$ 0.010 & 0.144 $\pm$ 0.021 &  & 0.115 $\pm$ 0.010 & 5668 $\pm$ 288 \\
                        & 0.528 $\pm$ 0.005 & 5023 $\pm$ 93 & $\shortparallel$ & 0.555 $\pm$ 0.008 & 4.737 $\pm$ 0.010 & -0.80 $\pm$ 0.03 &  & $\shortparallel$ & $\shortparallel$ \\
M4 V69 & 0.866 $\pm$ 0.010 & 6081 $\pm$ 126 & -1.20 $\pm$ 0.10 & 0.766 $\pm$ 0.005 & 4.44 $\pm$ 0.13 & -0.03 $\pm$ 0.04 &  & 0.429 $\pm$ 0.004 & 1717 $\pm$ 82 \\
                        & 0.807 $\pm$ 0.008 & 5916 $\pm$ 136 & $\shortparallel$ & 0.728 $\pm$ 0.005 & 4.48 $\pm$ 0.12 & -0.14 $\pm$ 0.04 &  & $\shortparallel$ & $\shortparallel$ \\
M4 V66 & 0.935 $\pm$ 0.005 & 6166 $\pm$ 99 & -1.20 $\pm$ 0.10 & 0.784 $\pm$ 0.005 & 4.39 $\pm$ 0.08 & 0.056 $\pm$ 0.028 &  & 0.429 $\pm$ 0.005 & 1717 $\pm$ 82 \\
                        & 0.830 $\pm$ 0.005 & 5943 $\pm$ 109 & $\shortparallel$ & 0.744 $\pm$ 0.004 & 4.47 $\pm$ 0.09 & -0.11 $\pm$ 0.03 &  & $\shortparallel$ & $\shortparallel$ \\
M4 V65 & 1.147 $\pm$ 0.010 & 6095 $\pm$ 112 & -1.20 $\pm$ 0.10 & 0.804 $\pm$ 0.009 & 4.221 $\pm$ 0.014 & 0.21 $\pm$ 0.03 &  & 0.426 $\pm$ 0.010 & 1717 $\pm$ 82 \\
                        & 0.611 $\pm$ 0.009 & 4808 $\pm$ 122 & $\shortparallel$ & 0.605 $\pm$ 0.004 & 4.645 $\pm$ 0.017 & -0.75 $\pm$ 0.05 &  & $\shortparallel$ & $\shortparallel$ \\
NGC 6362 V41 & 1.074 $\pm$ 0.005 & 6124 $\pm$ 127 & -1.07 $\pm$ 0.05 & 0.821 $\pm$ 0.006 & 4.311 $\pm$ 0.004 & 0.16 $\pm$ 0.04 &  & 0.0644 $\pm$ 0.0008 & 8095 $\pm$ 150 \\
                        & 0.731 $\pm$ 0.005 & 5741 $\pm$ 119 & $\shortparallel$ & 0.728 $\pm$ 0.005 & 4.593 $\pm$ 0.006 & -0.28 $\pm$ 0.04 &  & $\shortparallel$ & $\shortparallel$ \\
NGC 6362 V40 & 1.325 $\pm$ 0.008 & 6152 $\pm$ 127 & -1.07 $\pm$ 0.05 & 0.834 $\pm$ 0.006 & 4.550 $\pm$ 0.005 & 0.36 $\pm$ 0.04 &  & 0.0636 $\pm$ 0.0009 & 8095 $\pm$ 150 \\
                        & 0.997 $\pm$ 0.013 & 6095 $\pm$ 154 & $\shortparallel$ & 0.795 $\pm$ 0.005 & 4.361 $\pm$ 0.011 & 0.09 $\pm$ 0.05 &  & $\shortparallel$ & $\shortparallel$ \\
47 Tuc V69 & 1.315 $\pm$ 0.005 & 5943 $\pm$ 151 & -0.71 $\pm$ 0.10 & 0.876 $\pm$ 0.005 & 4.1430 $\pm$ 0.0030 & 0.29 $\pm$ 0.04 &  & 0.0271 $\pm$ 0.0005 & 4335 $\pm$ 279 \\
                        & 1.162 $\pm$ 0.006 & 5957 $\pm$ 151 & $\shortparallel$ & 0.859 $\pm$ 0.006 & 4.2420 $\pm$ 0.0030 & 0.18 $\pm$ 0.04 &  & $\shortparallel$ & $\shortparallel$ \\
Kepler-35 & 1.0285 $\pm$ 0.0019 & 5610 $\pm$ 142 & -0.34 $\pm$ 0.20 & 0.888 $\pm$ 0.005 & 4.3623 $\pm$ 0.0020 & -0.02 $\pm$ 0.04 &  & 0.121 $\pm$ 0.004 & 1918 $\pm$ 124 \\
                        & 0.7861 $\pm$ 0.0022 & 5200 $\pm$ 96 & $\shortparallel$ & 0.809 $\pm$ 0.004 & 4.5556 $\pm$ 0.0016 & -0.39 $\pm$ 0.03 &  & $\shortparallel$ & $\shortparallel$ \\
KIC 6131659 & 0.8800 $\pm$ 0.0028 & 5794 $\pm$ 53 & -0.23 $\pm$ 0.20 & 0.922 $\pm$ 0.007 & 4.534 $\pm$ 0.007 & -0.104 $\pm$ 0.016 &  & 0.1133 $\pm$ 0.0029 &  \\
                        & 0.639 $\pm$ 0.006 & 4613 $\pm$ 42 & $\shortparallel$ & 0.685 $\pm$ 0.005 & 4.682 $\pm$ 0.009 & -0.778 $\pm$ 0.018 &  & $\shortparallel$ &  \\
RW Lac & 1.186 $\pm$ 0.004 & 5754 $\pm$ 106 & -0.30 $\pm$ 0.19 & 0.928 $\pm$ 0.006 & 4.2570 $\pm$ 0.0030 & 0.14 $\pm$ 0.03 & G5V & 0.068 $\pm$ 0.012 & 208.0 $\pm$ 1.3 \\
                        & 0.964 $\pm$ 0.004 & 5559 $\pm$ 154 & $\shortparallel$ & 0.870 $\pm$ 0.004 & 4.409 $\pm$ 0.004 & -0.10 $\pm$ 0.05 & G7V & $\shortparallel$ & $\shortparallel$ \\
Kepler-453 & 0.833 $\pm$ 0.011 & 5521 $\pm$ 102 & 0.09 $\pm$ 0.10 & 0.944 $\pm$ 0.010 & 4.571 $\pm$ 0.015 & -0.24 $\pm$ 0.03 &  & 0.056 $\pm$ 0.004 & 448.6 $\pm$ 2.8 \\
                        & 0.2150 $\pm$ 0.0014 & 3228 $\pm$ 97 & $\shortparallel$ & 0.1951 $\pm$ 0.0020 & 5.063 $\pm$ 0.005 & -2.34 $\pm$ 0.05 &  & $\shortparallel$ & $\shortparallel$ \\
Tyc 5227-1023-1 & 1.388 $\pm$ 0.010 & 6353 $\pm$ 205 & -0.63 $\pm$ 0.11 & 0.956 $\pm$ 0.016 & 4.130 $\pm$ 0.010 & 0.45 $\pm$ 0.06 &  & 0.0749 $\pm$ 0.0012 & 399 $\pm$ 8 \\
                        & 0.977 $\pm$ 0.010 & 5929 $\pm$ 218 & $\shortparallel$ & 0.839 $\pm$ 0.012 & 4.380 $\pm$ 0.010 & 0.03 $\pm$ 0.06 &  & $\shortparallel$ & $\shortparallel$ \\
IM Vir & 1.061 $\pm$ 0.016 & 5675 $\pm$ 105 & -0.10 $\pm$ 0.25 & 0.981 $\pm$ 0.012 & 4.379 $\pm$ 0.014 & 0.02 $\pm$ 0.03 & G7V & 0 & 83.39 $\pm$ 0.29 \\
                        & 0.681 $\pm$ 0.013 & 4246 $\pm$ 127 & $\shortparallel$ & 0.664 $\pm$ 0.005 & 4.594 $\pm$ 0.017 & -0.87 $\pm$ 0.05 & K7V & $\shortparallel$ & $\shortparallel$ \\
V565 Lyr & 1.101 $\pm$ 0.007 & 5598 $\pm$ 90 & 0.28 $\pm$ 0.05 & 0.995 $\pm$ 0.003 & 4.352 $\pm$ 0.005 & 0.030 $\pm$ 0.029 &  & 0.1335 $\pm$ 0.0020 & 4067 $\pm$ 188 \\
                        & 0.971 $\pm$ 0.005 & 5433 $\pm$ 125 & $\shortparallel$ & 0.929 $\pm$ 0.003 & 4.432 $\pm$ 0.008 & -0.13 $\pm$ 0.04 &  & $\shortparallel$ & $\shortparallel$ \\
V530 Ori & 0.980 $\pm$ 0.013 & 5984 $\pm$ 96 & -0.12 $\pm$ 0.08 & 1.004 $\pm$ 0.007 & 4.457 $\pm$ 0.012 & 0.045 $\pm$ 0.030 &  & 0 & 102.9 $\pm$ 0.4 \\
                        & 0.587 $\pm$ 0.007 & 3882 $\pm$ 116 & $\shortparallel$ & 0.5955 $\pm$ 0.0022 & 4.676 $\pm$ 0.010 & -1.15 $\pm$ 0.05 &  & $\shortparallel$ & $\shortparallel$ \\
KIC 7177553 & 0.940 $\pm$ 0.005 & 5794 $\pm$ 133 & -0.05 $\pm$ 0.09 & 1.043 $\pm$ 0.014 & 4.517 $\pm$ 0.008 & -0.05 $\pm$ 0.04 & G2V & 0.0756 $\pm$ 0.0015 &  \\
                        & 0.941 $\pm$ 0.005 & 5741 $\pm$ 145 & $\shortparallel$ & 0.986 $\pm$ 0.015 & 4.491 $\pm$ 0.008 & -0.06 $\pm$ 0.04 & G2V & $\shortparallel$ &  \\
Kepler-34 & 1.1617 $\pm$ 0.0029 & 5916 $\pm$ 123 & -0.07 $\pm$ 0.15 & 1.048 $\pm$ 0.003 & 4.3284 $\pm$ 0.0021 & 0.17 $\pm$ 0.04 &  & 0.167 $\pm$ 0.005 & 1896 $\pm$ 92 \\
                        & 1.0927 $\pm$ 0.0030 & 5861 $\pm$ 135 & $\shortparallel$ & 1.0207 $\pm$ 0.0021 & 4.3703 $\pm$ 0.0022 & 0.10 $\pm$ 0.04 &  & $\shortparallel$ & $\shortparallel$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleI:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    System & $R$               & $T_{eff}$ & [Fe/H]      & $M$              & $\log g$              &  $\log L$                 &  $SpT/LC$  & $E(B-V)$        &  $d$    \\
                 & ($R_{\sun}$) & ($\,K$)     & ($dex$)   &  ($M_{\sun}$) & ($g$: cm s$^{-2}$)  & ($L$:  $L_{\sun}$)     &                    & ($mag$)         &  ($pc$)     \\
    \hline
V636 Cen & 1.018 $\pm$ 0.004 & 5902 $\pm$ 82 & -0.20 $\pm$ 0.08 & 1.052 $\pm$ 0.005 & 4.444 $\pm$ 0.004 & 0.054 $\pm$ 0.024 & G0V & 0 & 71.5 $\pm$ 0.4 \\
                        & 0.830 $\pm$ 0.004 & 5000 $\pm$ 104 & $\shortparallel$ & 0.8541 $\pm$ 0.0029 & 4.532 $\pm$ 0.005 & -0.41 $\pm$ 0.04 &  & $\shortparallel$ & $\shortparallel$ \\
V568 Lyr & 1.397 $\pm$ 0.013 & 5649 $\pm$ 91 & 0.28 $\pm$ 0.05 & 1.087 $\pm$ 0.004 & 4.184 $\pm$ 0.008 & 0.253 $\pm$ 0.029 & G5V & 0.1332 $\pm$ 0.0021 & 4068 $\pm$ 188 \\
                        & 0.781 $\pm$ 0.005 & 4819 $\pm$ 144 & $\shortparallel$ & 0.8276 $\pm$ 0.0023 & 4.570 $\pm$ 0.006 & -0.53 $\pm$ 0.05 & K3V & $\shortparallel$ & $\shortparallel$ \\
V785 Cep & 1.424 $\pm$ 0.019 & 5902 $\pm$ 95 & -0.06 $\pm$ 0.06 & 1.103 $\pm$ 0.007 & 4.174 $\pm$ 0.012 & 0.346 $\pm$ 0.030 & G1V & 0.087 $\pm$ 0.010 & 1573 $\pm$ 66 \\
                        & 1.373 $\pm$ 0.019 & 5875 $\pm$ 95 & $\shortparallel$ & 1.081 $\pm$ 0.007 & 4.196 $\pm$ 0.013 & 0.306 $\pm$ 0.030 & G1V & $\shortparallel$ & $\shortparallel$ \\
WOCS 12009 & 1.071 $\pm$ 0.009 & 6095 $\pm$ 98 & 0.03 $\pm$ 0.04 & 1.111 $\pm$ 0.015 & 4.4240 $\pm$ 0.0020 & 0.154 $\pm$ 0.029 &  & 0.041 $\pm$ 0.004 & 829 $\pm$ 20 \\
                        & 0.71 $\pm$ 0.03 & 4710 $\pm$ 108 & $\shortparallel$ & 0.748 $\pm$ 0.005 & 4.61 $\pm$ 0.04 & -0.65 $\pm$ 0.06 &  & $\shortparallel$ & $\shortparallel$ \\
$\alpha$ Cen & 1.231 $\pm$ 0.004 & 5824 $\pm$ 26 & 0.24 $\pm$ 0.04 & 1.133 $\pm$ 0.005 & 4.3120 $\pm$ 0.0030 & 0.196 $\pm$ 0.008 & G2V & 0 & 1.3459 $\pm$ 0.0024 \\
                        & 0.868 $\pm$ 0.005 & 5223 $\pm$ 62 & $\shortparallel$ & 0.972 $\pm$ 0.004 & 4.549 $\pm$ 0.006 & -0.297 $\pm$ 0.021 & K1V & $\shortparallel$ & $\shortparallel$ \\
KX Cnc & 1.0639 $\pm$ 0.0020 & 5902 $\pm$ 95 & 0.07 $\pm$ 0.10 & 1.1379 $\pm$ 0.0029 & 4.441 $\pm$ 0.004 & 0.092 $\pm$ 0.028 & F9V & 0 & 49.31 $\pm$ 0.12 \\
                        & 1.0491 $\pm$ 0.0019 & 5848 $\pm$ 94 & $\shortparallel$ & 1.131 $\pm$ 0.003 & 4.450 $\pm$ 0.004 & 0.064 $\pm$ 0.028 & F9V & $\shortparallel$ & $\shortparallel$ \\
KIC 7037405 & 14.00 $\pm$ 0.09 & 4498 $\pm$ 83 & -0.27 $\pm$ 0.10 & 1.170 $\pm$ 0.020 & 2.213 $\pm$ 0.007 & 1.86 $\pm$ 0.03 &  & 0.114 $\pm$ 0.003 & 1951 $\pm$ 94 \\
                        & 1.746 $\pm$ 0.014 & 6095 $\pm$ 140 & $\shortparallel$ & 1.110 $\pm$ 0.011 & 3.999 $\pm$ 0.007 & 0.58 $\pm$ 0.04 &  & $\shortparallel$ & $\shortparallel$ \\
EW Ori & 1.168 $\pm$ 0.005 & 6067 $\pm$ 98 & 0.05 $\pm$ 0.09 & 1.173 $\pm$ 0.011 & 4.372 $\pm$ 0.005 & 0.221 $\pm$ 0.028 & G0V & 0.026 $\pm$ 0.014 & 184.7 $\pm$ 1.7 \\
                        & 1.097 $\pm$ 0.005 & 5902 $\pm$ 95 & $\shortparallel$ & 1.123 $\pm$ 0.009 & 4.408 $\pm$ 0.005 & 0.119 $\pm$ 0.028 & G2V & $\shortparallel$ & $\shortparallel$ \\
KIC 9970396 & 8.04 $\pm$ 0.07 & 4864 $\pm$ 78 & -0.35 $\pm$ 0.10 & 1.178 $\pm$ 0.015 & 2.699 $\pm$ 0.011 & 1.513 $\pm$ 0.029 &  & 0.2111 $\pm$ 0.0023 & 1075 $\pm$ 39 \\
                        & 1.109 $\pm$ 0.005 & 6223 $\pm$ 129 & $\shortparallel$ & 1.003 $\pm$ 0.009 & 4.349 $\pm$ 0.005 & 0.22 $\pm$ 0.04 &  & $\shortparallel$ & $\shortparallel$ \\
LV Her & 1.358 $\pm$ 0.012 & 6209 $\pm$ 157 & 0.08 $\pm$ 0.21 & 1.193 $\pm$ 0.010 & 4.249 $\pm$ 0.008 & 0.39 $\pm$ 0.04 & F9V & 0.030 $\pm$ 0.030 & 374 $\pm$ 3 \\
                        & 1.313 $\pm$ 0.011 & 6026 $\pm$ 153 & $\shortparallel$ & 1.170 $\pm$ 0.008 & 4.269 $\pm$ 0.008 & 0.31 $\pm$ 0.04 & F9V & $\shortparallel$ & $\shortparallel$ \\
LL Aqr & 1.321 $\pm$ 0.006 & 6081 $\pm$ 42 & 0.02 $\pm$ 0.04 & 1.1959 $\pm$ 0.0008 & 4.274 $\pm$ 0.004 & 0.332 $\pm$ 0.013 & F3V & 0 & 137.6 $\pm$ 1.0 \\
                        & 1.002 $\pm$ 0.005 & 5702 $\pm$ 53 & $\shortparallel$ & 1.0337 $\pm$ 0.0007 & 4.451 $\pm$ 0.004 & -0.020 $\pm$ 0.017 & F8V & $\shortparallel$ & $\shortparallel$ \\
V432 Aur & 2.460 $\pm$ 0.020 & 6081 $\pm$ 84 & -0.60 $\pm$ 0.05 & 1.200 $\pm$ 0.018 & 3.740 $\pm$ 0.010 & 0.872 $\pm$ 0.025 & F9IV & 0 & 127.1 $\pm$ 1.2 \\
                        & 1.230 $\pm$ 0.006 & 6683 $\pm$ 92 & $\shortparallel$ & 1.080 $\pm$ 0.014 & 4.290 $\pm$ 0.008 & 0.434 $\pm$ 0.024 & F3V & $\shortparallel$ & $\shortparallel$ \\
Kepler 1647 & 1.790 $\pm$ 0.005 & 6209 $\pm$ 100 & -0.14 $\pm$ 0.05 & 1.221 $\pm$ 0.011 & 4.0180 $\pm$ 0.0020 & 0.632 $\pm$ 0.028 &  & 0.367 $\pm$ 0.017 & 1256 $\pm$ 24 \\
                        & 0.966 $\pm$ 0.006 & 5768 $\pm$ 120 & $\shortparallel$ & 0.968 $\pm$ 0.004 & 4.453 $\pm$ 0.004 & -0.03 $\pm$ 0.04 &  & $\shortparallel$ & $\shortparallel$ \\
UX Men & 1.347 $\pm$ 0.013 & 6194 $\pm$ 100 & 0.04 $\pm$ 0.10 & 1.2229 $\pm$ 0.0014 & 4.272 $\pm$ 0.009 & 0.381 $\pm$ 0.029 & F8V & 0 & 103.69 $\pm$ 0.27 \\
                        & 1.274 $\pm$ 0.013 & 6152 $\pm$ 99 & $\shortparallel$ & 1.1877 $\pm$ 0.0014 & 4.306 $\pm$ 0.009 & 0.321 $\pm$ 0.029 & F8V & $\shortparallel$ & $\shortparallel$ \\
WZ Oph & 1.401 $\pm$ 0.012 & 6166 $\pm$ 99 & -0.27 $\pm$ 0.07 & 1.227 $\pm$ 0.007 & 4.234 $\pm$ 0.008 & 0.407 $\pm$ 0.029 & F8V & 0 & 156.9 $\pm$ 0.8 \\
                        & 1.419 $\pm$ 0.012 & 6109 $\pm$ 98 & $\shortparallel$ & 1.220 $\pm$ 0.006 & 4.221 $\pm$ 0.008 & 0.403 $\pm$ 0.029 & F8V & $\shortparallel$ & $\shortparallel$ \\
WOCS 40007 & 1.399 $\pm$ 0.007 & 6237 $\pm$ 86 & -0.03 $\pm$ 0.06 & 1.236 $\pm$ 0.020 & 4.240 $\pm$ 0.005 & 0.426 $\pm$ 0.024 &  & 0.176 $\pm$ 0.007 & 2328 $\pm$ 50 \\
                        & 1.098 $\pm$ 0.004 & 5957 $\pm$ 151 & $\shortparallel$ & 1.086 $\pm$ 0.018 & 4.381 $\pm$ 0.004 & 0.14 $\pm$ 0.04 &  & $\shortparallel$ & $\shortparallel$ \\
EF Aqr & 1.338 $\pm$ 0.012 & 6152 $\pm$ 85 & 0.00 $\pm$ 0.10 & 1.244 $\pm$ 0.008 & 4.280 $\pm$ 0.007 & 0.364 $\pm$ 0.025 & G0V & 0.025 $\pm$ 0.015 & 173.5 $\pm$ 1.8 \\
                        & 0.956 $\pm$ 0.012 & 5188 $\pm$ 108 & $\shortparallel$ & 0.946 $\pm$ 0.006 & 4.453 $\pm$ 0.011 & -0.22 $\pm$ 0.04 &  & $\shortparallel$ & $\shortparallel$ \\
AI Phe & 2.912 $\pm$ 0.014 & 5152 $\pm$ 154 & -0.14 $\pm$ 0.10 & 1.247 $\pm$ 0.004 & 3.606 $\pm$ 0.004 & 0.73 $\pm$ 0.05 & K0IV & 0 & 171.4 $\pm$ 0.8 \\
                        & 1.835 $\pm$ 0.014 & 6124 $\pm$ 155 & $\shortparallel$ & 1.197 $\pm$ 0.004 & 3.989 $\pm$ 0.007 & 0.63 $\pm$ 0.04 & F7V & $\shortparallel$ & $\shortparallel$ \\
VZ Hya & 1.314 $\pm$ 0.005 & 6442 $\pm$ 148 & -0.20 $\pm$ 0.12 & 1.271 $\pm$ 0.006 & 4.305 $\pm$ 0.005 & 0.43 $\pm$ 0.04 & F5V & 0 & 147.8 $\pm$ 1.1 \\
                        & 1.112 $\pm$ 0.007 & 6295 $\pm$ 145 & $\shortparallel$ & 1.146 $\pm$ 0.007 & 4.405 $\pm$ 0.006 & 0.24 $\pm$ 0.04 & F6V & $\shortparallel$ & $\shortparallel$ \\
V505 Per & 1.287 $\pm$ 0.024 & 6510 $\pm$ 50 & -0.120 $\pm$ 0.030 & 1.272 $\pm$ 0.007 & 4.323 $\pm$ 0.016 & 0.428 $\pm$ 0.021 & F5V & 0 & 62.62 $\pm$ 0.15 \\
                        & 1.266 $\pm$ 0.024 & 6460 $\pm$ 50 & $\shortparallel$ & 1.254 $\pm$ 0.007 & 4.331 $\pm$ 0.017 & 0.400 $\pm$ 0.021 & F5V & $\shortparallel$ & $\shortparallel$ \\
V375 Cep & 1.623 $\pm$ 0.006 & 6223 $\pm$ 43 & 0.09 $\pm$ 0.05 & 1.288 $\pm$ 0.017 & 4.129 $\pm$ 0.007 & 0.551 $\pm$ 0.012 &  & 0.423 $\pm$ 0.014 &  \\
                        & 0.897 $\pm$ 0.003 & 5047 $\pm$ 174 & $\shortparallel$ & 0.871 $\pm$ 0.008 & 4.4730 $\pm$ 0.0020 & -0.33 $\pm$ 0.06 &  & $\shortparallel$ &  \\
CO And & 1.727 $\pm$ 0.021 & 6138 $\pm$ 127 & 0.01 $\pm$ 0.15 & 1.289 $\pm$ 0.007 & 4.074 $\pm$ 0.011 & 0.58 $\pm$ 0.04 & F8V & 0.090 $\pm$ 0.030 & 393 $\pm$ 10 \\
                        & 1.694 $\pm$ 0.017 & 6166 $\pm$ 128 & $\shortparallel$ & 1.264 $\pm$ 0.007 & 4.082 $\pm$ 0.009 & 0.57 $\pm$ 0.04 & F8V & $\shortparallel$ & $\shortparallel$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleI:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    System & $R$               & $T_{eff}$ & [Fe/H]      & $M$              & $\log g$              &  $\log L$                 &  $SpT/LC$  & $E(B-V)$        &  $d$    \\
                 & ($R_{\sun}$) & ($\,K$)     & ($dex$)   &  ($M_{\sun}$) & ($g$: cm s$^{-2}$)  & ($L$:  $L_{\sun}$)     &                    & ($mag$)         &  ($pc$)     \\
    \hline
KIC 8430105 & 7.65 $\pm$ 0.05 & 5047 $\pm$ 70 & -0.49 $\pm$ 0.04 & 1.310 $\pm$ 0.020 & 2.788 $\pm$ 0.004 & 1.534 $\pm$ 0.025 &  & 0.1312 $\pm$ 0.0013 & 718 $\pm$ 13 \\
                        & 0.77 $\pm$ 0.05 & 5768 $\pm$ 80 & $\shortparallel$ & 0.830 $\pm$ 0.010 & 4.584 $\pm$ 0.012 & -0.23 $\pm$ 0.06 &  & $\shortparallel$ & $\shortparallel$ \\
NP Per & 1.372 $\pm$ 0.013 & 6427 $\pm$ 89 & 0.02 $\pm$ 0.08 & 1.321 $\pm$ 0.009 & 4.284 $\pm$ 0.008 & 0.461 $\pm$ 0.025 & F5V & 0.237 $\pm$ 0.010 & 321 $\pm$ 13 \\
                        & 1.229 $\pm$ 0.013 & 4539 $\pm$ 157 & $\shortparallel$ & 1.046 $\pm$ 0.005 & 4.278 $\pm$ 0.009 & -0.24 $\pm$ 0.06 & K5e & $\shortparallel$ & $\shortparallel$ \\
ASAS J052821+0338.5 & 1.830 $\pm$ 0.010 & 5105 $\pm$ 106 & -0.15 $\pm$ 0.14 & 1.375 $\pm$ 0.011 & 4.050 $\pm$ 0.010 & 0.31 $\pm$ 0.04 & K1PMS & 0.125 $\pm$ 0.006 &  \\
                        & 1.730 $\pm$ 0.010 & 4710 $\pm$ 98 & $\shortparallel$ & 1.329 $\pm$ 0.008 & 4.080 $\pm$ 0.010 & 0.12 $\pm$ 0.04 & K3PMS & $\shortparallel$ &  \\
KIC 9540226 & 13.06 $\pm$ 0.16 & 4677 $\pm$ 75 & -0.23 $\pm$ 0.10 & 1.38 $\pm$ 0.04 & 2.345 $\pm$ 0.010 & 1.867 $\pm$ 0.030 &  & 0.154 $\pm$ 0.010 & 2045 $\pm$ 85 \\
                        & 1.014 $\pm$ 0.014 & 6152 $\pm$ 127 & $\shortparallel$ & 1.002 $\pm$ 0.015 & 4.427 $\pm$ 0.010 & 0.12 $\pm$ 0.04 &  & $\shortparallel$ & $\shortparallel$ \\
V1130 Tau & 1.782 $\pm$ 0.011 & 6622 $\pm$ 76 & -0.25 $\pm$ 0.10 & 1.392 $\pm$ 0.008 & 4.080 $\pm$ 0.006 & 0.740 $\pm$ 0.021 & F2V & 0 & 70.15 $\pm$ 0.21 \\
                        & 1.489 $\pm$ 0.010 & 6637 $\pm$ 76 & $\shortparallel$ & 1.306 $\pm$ 0.008 & 4.208 $\pm$ 0.006 & 0.588 $\pm$ 0.021 & F2V & $\shortparallel$ & $\shortparallel$ \\
AD Boo & 1.612 $\pm$ 0.014 & 6577 $\pm$ 121 & 0.10 $\pm$ 0.15 & 1.414 $\pm$ 0.009 & 4.173 $\pm$ 0.008 & 0.64 $\pm$ 0.03 & F6V & 0.027 $\pm$ 0.021 & 195.4 $\pm$ 2.8 \\
                        & 1.216 $\pm$ 0.010 & 6152 $\pm$ 113 & $\shortparallel$ & 1.209 $\pm$ 0.006 & 4.351 $\pm$ 0.007 & 0.28 $\pm$ 0.03 & G0V & $\shortparallel$ & $\shortparallel$ \\
BK Peg & 1.988 $\pm$ 0.008 & 6266 $\pm$ 87 & -0.12 $\pm$ 0.07 & 1.414 $\pm$ 0.007 & 3.992 $\pm$ 0.004 & 0.739 $\pm$ 0.024 & F8V & 0.0638 $\pm$ 0.0017 & 319 $\pm$ 5 \\
                        & 1.474 $\pm$ 0.017 & 6324 $\pm$ 87 & $\shortparallel$ & 1.257 $\pm$ 0.005 & 4.201 $\pm$ 0.010 & 0.496 $\pm$ 0.026 & F7V & $\shortparallel$ & $\shortparallel$ \\
OGLE-LMC-ECL15260 & 42.2 $\pm$ 0.3 & 4315 $\pm$ 79 & -0.47 $\pm$ 0.15 & 1.426 $\pm$ 0.022 & 1.342 $\pm$ 0.007 & 2.74 $\pm$ 0.03 &  & 0.100 $\pm$ 0.020 &  \\
                        & 23.5 $\pm$ 0.7 & 4710 $\pm$ 87 & $\shortparallel$ & 1.440 $\pm$ 0.024 & 1.854 $\pm$ 0.025 & 2.39 $\pm$ 0.04 &  & $\shortparallel$ &  \\
BG Ind & 2.290 $\pm$ 0.017 & 6353 $\pm$ 263 & -0.20 $\pm$ 0.10 & 1.428 $\pm$ 0.008 & 3.873 $\pm$ 0.005 & 0.89 $\pm$ 0.07 &  & 0 & 51.0 $\pm$ 0.5 \\
                        & 1.68 $\pm$ 0.04 & 6653 $\pm$ 230 & $\shortparallel$ & 1.293 $\pm$ 0.008 & 4.099 $\pm$ 0.020 & 0.70 $\pm$ 0.06 &  & $\shortparallel$ & $\shortparallel$ \\
CD Tau & 1.798 $\pm$ 0.017 & 6194 $\pm$ 57 & 0.08 $\pm$ 0.15 & 1.442 $\pm$ 0.016 & 4.087 $\pm$ 0.010 & 0.632 $\pm$ 0.018 & F6V & 0 & 73.5 $\pm$ 0.4 \\
                        & 1.584 $\pm$ 0.020 & 6194 $\pm$ 57 & $\shortparallel$ & 1.368 $\pm$ 0.016 & 4.174 $\pm$ 0.012 & 0.522 $\pm$ 0.019 & F6V & $\shortparallel$ & $\shortparallel$ \\
V570 Per & 1.52 $\pm$ 0.03 & 6842 $\pm$ 50 & 0.020 $\pm$ 0.030 & 1.447 $\pm$ 0.009 & 4.234 $\pm$ 0.019 & 0.660 $\pm$ 0.023 & F3V & 0 & 119.7 $\pm$ 0.6 \\
                        & 1.386 $\pm$ 0.019 & 6562 $\pm$ 50 & $\shortparallel$ & 1.347 $\pm$ 0.008 & 4.284 $\pm$ 0.012 & 0.506 $\pm$ 0.018 & F5V & $\shortparallel$ & $\shortparallel$ \\
BW Aqr & 2.06 $\pm$ 0.04 & 6295 $\pm$ 101 & -0.07 $\pm$ 0.11 & 1.488 $\pm$ 0.022 & 3.981 $\pm$ 0.020 & 0.78 $\pm$ 0.03 & F7V & 0.0283 $\pm$ 0.0012 & 417 $\pm$ 22 \\
                        & 1.79 $\pm$ 0.04 & 6223 $\pm$ 100 & $\shortparallel$ & 1.386 $\pm$ 0.021 & 4.075 $\pm$ 0.022 & 0.64 $\pm$ 0.03 & F8V & $\shortparallel$ & $\shortparallel$ \\
GX Gem & 2.327 $\pm$ 0.012 & 6194 $\pm$ 100 & -0.12 $\pm$ 0.10 & 1.488 $\pm$ 0.011 & 3.877 $\pm$ 0.004 & 0.856 $\pm$ 0.028 & F7V & 0.0867 $\pm$ 0.0014 & 785 $\pm$ 42 \\
                        & 2.238 $\pm$ 0.012 & 6166 $\pm$ 99 & $\shortparallel$ & 1.467 $\pm$ 0.010 & 3.904 $\pm$ 0.005 & 0.814 $\pm$ 0.028 & F7V & $\shortparallel$ & $\shortparallel$ \\
HD 187669 & 22.6 $\pm$ 0.5 & 4325 $\pm$ 70 & -0.25 $\pm$ 0.10 & 1.505 $\pm$ 0.004 & 1.907 $\pm$ 0.019 & 2.21 $\pm$ 0.03 & K2.5III & 0.121 $\pm$ 0.016 & 647 $\pm$ 23 \\
                        & 11.33 $\pm$ 0.28 & 4645 $\pm$ 75 & $\shortparallel$ & 1.504 $\pm$ 0.003 & 2.507 $\pm$ 0.020 & 1.73 $\pm$ 0.04 & K0III & $\shortparallel$ & $\shortparallel$ \\
KIC 11285625 & 2.123 $\pm$ 0.010 & 6966 $\pm$ 96 & -0.58 $\pm$ 0.15 & 1.543 $\pm$ 0.013 & 3.973 $\pm$ 0.006 & 0.980 $\pm$ 0.024 & earlyF & 0.0447 $\pm$ 0.0006 & 531 $\pm$ 5 \\
                        & 1.472 $\pm$ 0.014 & 7194 $\pm$ 199 & $\shortparallel$ & 1.200 $\pm$ 0.016 & 4.180 $\pm$ 0.010 & 0.72 $\pm$ 0.05 & earlyF & $\shortparallel$ & $\shortparallel$ \\
KIC 8410637 & 10.74 $\pm$ 0.11 & 4797 $\pm$ 77 & 0.20 $\pm$ 0.11 & 1.557 $\pm$ 0.028 & 2.569 $\pm$ 0.009 & 1.741 $\pm$ 0.029 & GIII & 0.0503 $\pm$ 0.0020 & 1267 $\pm$ 32 \\
                        & 1.57 $\pm$ 0.03 & 6486 $\pm$ 164 & $\shortparallel$ & 1.322 $\pm$ 0.017 & 4.167 $\pm$ 0.016 & 0.60 $\pm$ 0.05 &  & $\shortparallel$ & $\shortparallel$ \\
KIC 9777062 & 1.744 $\pm$ 0.004 & 7691 $\pm$ 142 & -0.03 $\pm$ 0.13 & 1.603 $\pm$ 0.017 & 4.1600 $\pm$ 0.0030 & 0.98 $\pm$ 0.03 & Am & 0.1224 $\pm$ 0.0018 & 996 $\pm$ 14 \\
                        & 1.5438 $\pm$ 0.0028 & 7145 $\pm$ 99 & $\shortparallel$ & 1.419 $\pm$ 0.009 & 4.2130 $\pm$ 0.0020 & 0.748 $\pm$ 0.024 &  & $\shortparallel$ & $\shortparallel$ \\
V501 Mon & 1.888 $\pm$ 0.029 & 7516 $\pm$ 104 & 0.01 $\pm$ 0.06 & 1.646 $\pm$ 0.004 & 4.103 $\pm$ 0.013 & 1.011 $\pm$ 0.027 & A6m & 0.18 $\pm$ 0.04 & 980 $\pm$ 44 \\
                        & 1.592 $\pm$ 0.028 & 6998 $\pm$ 97 & $\shortparallel$ & 1.4588 $\pm$ 0.0024 & 4.199 $\pm$ 0.016 & 0.738 $\pm$ 0.028 & F0 & $\shortparallel$ & $\shortparallel$ \\
CoRoT 102918586 & 1.640 $\pm$ 0.010 & 7379 $\pm$ 85 & 0.11 $\pm$ 0.05 & 1.660 $\pm$ 0.020 & 4.230 $\pm$ 0.010 & 0.856 $\pm$ 0.021 &  & 0.135 $\pm$ 0.010 & 1153 $\pm$ 59 \\
                        & 1.480 $\pm$ 0.010 & 7096 $\pm$ 114 & $\shortparallel$ & 1.490 $\pm$ 0.030 & 4.270 $\pm$ 0.010 & 0.699 $\pm$ 0.029 &  & $\shortparallel$ & $\shortparallel$ \\
OGLE SMC126.1 210 & 43.5 $\pm$ 1.0 & 4477 $\pm$ 72 & -0.87 $\pm$ 0.15 & 1.67 $\pm$ 0.04 & 1.385 $\pm$ 0.029 & 2.84 $\pm$ 0.03 & K2III & 0.080 $\pm$ 0.028 &  \\
                        & 39.0 $\pm$ 1.0 & 4508 $\pm$ 73 & $\shortparallel$ & 1.67 $\pm$ 0.04 & 1.48 $\pm$ 0.03 & 2.75 $\pm$ 0.04 & K1III & $\shortparallel$ &  \\
HW CMa & 1.662 $\pm$ 0.021 & 7691 $\pm$ 142 & 0.33 $\pm$ 0.15 & 1.781 $\pm$ 0.012 & 4.247 $\pm$ 0.011 & 0.94 $\pm$ 0.03 & A7Vm & 0.300 $\pm$ 0.016 & 353 $\pm$ 4 \\
                        & 1.643 $\pm$ 0.018 & 7568 $\pm$ 157 & $\shortparallel$ & 1.721 $\pm$ 0.011 & 4.242 $\pm$ 0.010 & 0.90 $\pm$ 0.04 & A7Vm & $\shortparallel$ & $\shortparallel$ \\
OGLE-LMC-ECL03160 & 37.4 $\pm$ 0.5 & 4487 $\pm$ 83 & -0.48 $\pm$ 0.20 & 1.799 $\pm$ 0.027 & 1.547 $\pm$ 0.012 & 2.71 $\pm$ 0.03 &  & 0.123 $\pm$ 0.020 &  \\
                        & 16.4 $\pm$ 1.1 & 4955 $\pm$ 80 & $\shortparallel$ & 1.792 $\pm$ 0.027 & 2.26 $\pm$ 0.06 & 2.16 $\pm$ 0.06 &  & $\shortparallel$ &  \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleI:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    System & $R$               & $T_{eff}$ & [Fe/H]      & $M$              & $\log g$              &  $\log L$                 &  $SpT/LC$  & $E(B-V)$        &  $d$    \\
                 & ($R_{\sun}$) & ($\,K$)     & ($dex$)   &  ($M_{\sun}$) & ($g$: cm s$^{-2}$)  & ($L$:  $L_{\sun}$)     &                    & ($mag$)         &  ($pc$)     \\
    \hline
OGLE SMC130.5 4296 & 46.0 $\pm$ 0.3 & 4519 $\pm$ 73 & -0.88 $\pm$ 0.15 & 1.805 $\pm$ 0.027 & 1.369 $\pm$ 0.013 & 2.900 $\pm$ 0.029 & K1III & 0.079 $\pm$ 0.028 &  \\
                        & 25.44 $\pm$ 0.25 & 4909 $\pm$ 79 & $\shortparallel$ & 1.854 $\pm$ 0.025 & 1.895 $\pm$ 0.014 & 2.530 $\pm$ 0.029 & G7III & $\shortparallel$ &  \\
RS Cha & 2.14 $\pm$ 0.06 & 8054 $\pm$ 185 & 0.17 $\pm$ 0.07 & 1.858 $\pm$ 0.016 & 4.047 $\pm$ 0.023 & 1.24 $\pm$ 0.05 & A8V & 0 & 99.0 $\pm$ 0.4 \\
                        & 2.34 $\pm$ 0.05 & 7691 $\pm$ 177 & $\shortparallel$ & 1.821 $\pm$ 0.018 & 3.961 $\pm$ 0.021 & 1.24 $\pm$ 0.04 & A8V & $\shortparallel$ & $\shortparallel$ \\
RR Lyn & 2.570 $\pm$ 0.020 & 7568 $\pm$ 105 & 0.35 $\pm$ 0.20 & 1.927 $\pm$ 0.008 & 3.900 $\pm$ 0.005 & 1.290 $\pm$ 0.025 & A6IVm & 0 & 81.3 $\pm$ 1.0 \\
                        & 1.590 $\pm$ 0.030 & 6982 $\pm$ 96 & $\shortparallel$ & 1.507 $\pm$ 0.004 & 4.214 $\pm$ 0.018 & 0.733 $\pm$ 0.029 & F0Vm: & $\shortparallel$ & $\shortparallel$ \\
EK Cep & 1.579 $\pm$ 0.007 & 8995 $\pm$ 207 & 0.07 $\pm$ 0.05 & 2.029 $\pm$ 0.023 & 4.349 $\pm$ 0.010 & 1.17 $\pm$ 0.04 & A2V & 0.010 $\pm$ 0.020 & 172.8 $\pm$ 1.1 \\
                        & 1.315 $\pm$ 0.006 & 5702 $\pm$ 197 & $\shortparallel$ & 1.124 $\pm$ 0.012 & 4.251 $\pm$ 0.006 & 0.22 $\pm$ 0.06 & G5Vp & $\shortparallel$ & $\shortparallel$ \\
TZ For & 8.34 $\pm$ 0.11 & 4932 $\pm$ 34 & 0.02 $\pm$ 0.05 & 2.0568 $\pm$ 0.0009 & 2.915 $\pm$ 0.023 & 1.569 $\pm$ 0.017 & G8III & 0.015 $\pm$ 0.005 & 183.4 $\pm$ 0.9 \\
                        & 3.97 $\pm$ 0.08 & 6353 $\pm$ 73 & $\shortparallel$ & 1.9579 $\pm$ 0.0009 & 3.54 $\pm$ 0.04 & 1.364 $\pm$ 0.027 & F7III & $\shortparallel$ & $\shortparallel$ \\
KIC 9246715 & 8.37 $\pm$ 0.05 & 4932 $\pm$ 182 & -0.15 $\pm$ 0.08 & 2.171 $\pm$ 0.007 & 2.929 $\pm$ 0.005 & 1.57 $\pm$ 0.06 &  & 0.145 $\pm$ 0.022 & 616 $\pm$ 11 \\
                        & 8.30 $\pm$ 0.04 & 4932 $\pm$ 182 & $\shortparallel$ & 2.149 $\pm$ 0.007 & 2.932 $\pm$ 0.004 & 1.56 $\pm$ 0.06 &  & $\shortparallel$ & $\shortparallel$ \\
V1229 Tau & 1.84 $\pm$ 0.04 & 10023 $\pm$ 600 & 0.06 $\pm$ 0.05 & 2.221 $\pm$ 0.027 & 4.253 $\pm$ 0.019 & 1.49 $\pm$ 0.11 & A0V & 0 & 136.2 $\pm$ 1.2 \\
                        & 1.565 $\pm$ 0.015 & 7261 $\pm$ 368 & $\shortparallel$ & 1.59 $\pm$ 0.04 & 4.231 $\pm$ 0.024 & 0.79 $\pm$ 0.09 & AVm & $\shortparallel$ & $\shortparallel$ \\
OGLE LMC-ECL-25658 & 27.57 $\pm$ 0.24 & 4721 $\pm$ 76 & -0.65 $\pm$ 0.10 & 2.230 $\pm$ 0.019 & 1.906 $\pm$ 0.007 & 2.531 $\pm$ 0.029 & G9III & 0.091 $\pm$ 0.030 &  \\
                        & 21.41 $\pm$ 0.15 & 4677 $\pm$ 65 & $\shortparallel$ & 2.229 $\pm$ 0.019 & 2.125 $\pm$ 0.006 & 2.296 $\pm$ 0.025 & G8III & $\shortparallel$ &  \\
SW CMa & 3.014 $\pm$ 0.020 & 8204 $\pm$ 151 & 0.55 $\pm$ 0.15 & 2.239 $\pm$ 0.014 & 3.830 $\pm$ 0.006 & 1.57 $\pm$ 0.03 & A4m & 0.032 $\pm$ 0.013 & 630 $\pm$ 16 \\
                        & 2.50 $\pm$ 0.04 & 8091 $\pm$ 149 & $\shortparallel$ & 2.104 $\pm$ 0.018 & 3.967 $\pm$ 0.015 & 1.38 $\pm$ 0.04 & A5m & $\shortparallel$ & $\shortparallel$ \\
CoRoT 105906206 & 4.240 $\pm$ 0.020 & 6745 $\pm$ 155 & 0.00 $\pm$ 0.10 & 2.25 $\pm$ 0.04 & 3.530 $\pm$ 0.010 & 1.53 $\pm$ 0.04 &  & 0.21 $\pm$ 0.06 & 1010 $\pm$ 52 \\
                        & 1.340 $\pm$ 0.010 & 6152 $\pm$ 156 & $\shortparallel$ & 1.290 $\pm$ 0.030 & 4.300 $\pm$ 0.020 & 0.36 $\pm$ 0.04 &  & $\shortparallel$ & $\shortparallel$ \\
YZ Cas & 2.525 $\pm$ 0.011 & 9528 $\pm$ 110 & 0.10 $\pm$ 0.06 & 2.263 $\pm$ 0.012 & 3.988 $\pm$ 0.004 & 1.675 $\pm$ 0.020 & A1Vm & 0 & 95.5 $\pm$ 0.9 \\
                        & 1.331 $\pm$ 0.006 & 6887 $\pm$ 238 & $\shortparallel$ & 1.325 $\pm$ 0.007 & 4.311 $\pm$ 0.004 & 0.56 $\pm$ 0.06 & F2V & $\shortparallel$ & $\shortparallel$ \\
OGLE SMC101.8 14077 & 23.9 $\pm$ 0.3 & 5164 $\pm$ 95 & -1.01 $\pm$ 0.15 & 2.84 $\pm$ 0.05 & 2.136 $\pm$ 0.019 & 2.56 $\pm$ 0.03 & G4III & 0.067 $\pm$ 0.028 &  \\
                        & 17.9 $\pm$ 0.5 & 5585 $\pm$ 90 & $\shortparallel$ & 2.73 $\pm$ 0.03 & 2.368 $\pm$ 0.029 & 2.45 $\pm$ 0.04 & G0III & $\shortparallel$ &  \\
OGLE-LMC-ECL09660 & 43.9 $\pm$ 1.1 & 4677 $\pm$ 75 & -0.44 $\pm$ 0.10 & 2.988 $\pm$ 0.018 & 1.629 $\pm$ 0.023 & 2.92 $\pm$ 0.04 &  & 0.127 $\pm$ 0.020 &  \\
                        & 23.8 $\pm$ 0.7 & 5358 $\pm$ 74 & $\shortparallel$ & 2.969 $\pm$ 0.020 & 2.159 $\pm$ 0.024 & 2.62 $\pm$ 0.03 &  & $\shortparallel$ &  \\
OGLE-LMC-ECL10567 & 36.0 $\pm$ 2.0 & 4699 $\pm$ 76 & -0.81 $\pm$ 0.20 & 3.18 $\pm$ 0.04 & 1.83 $\pm$ 0.05 & 2.76 $\pm$ 0.06 &  & 0.102 $\pm$ 0.020 &  \\
                        & 25.6 $\pm$ 1.6 & 5070 $\pm$ 70 & $\shortparallel$ & 3.35 $\pm$ 0.04 & 2.15 $\pm$ 0.05 & 2.59 $\pm$ 0.06 &  & $\shortparallel$ &  \\
OGLE-LMC-ECL09114 & 26.2 $\pm$ 0.3 & 5284 $\pm$ 85 & -0.23 $\pm$ 0.10 & 3.303 $\pm$ 0.028 & 2.121 $\pm$ 0.010 & 2.683 $\pm$ 0.030 & G4III & 0.160 $\pm$ 0.020 &  \\
                        & 18.6 $\pm$ 0.3 & 5470 $\pm$ 101 & $\shortparallel$ & 3.208 $\pm$ 0.026 & 2.403 $\pm$ 0.014 & 2.45 $\pm$ 0.03 & G4III & $\shortparallel$ &  \\
V906 Sco & 4.52 $\pm$ 0.04 & 10399 $\pm$ 503 & 0.14 $\pm$ 0.06 & 3.38 $\pm$ 0.07 & 3.656 $\pm$ 0.012 & 2.33 $\pm$ 0.08 & B9V & 0.078 $\pm$ 0.010 & 315 $\pm$ 60 \\
                        & 3.51 $\pm$ 0.04 & 10691 $\pm$ 492 & $\shortparallel$ & 3.25 $\pm$ 0.07 & 3.858 $\pm$ 0.013 & 2.16 $\pm$ 0.08 & B9V & $\shortparallel$ & $\shortparallel$ \\
OGLE SMC113.3 4007 & 48.4 $\pm$ 0.7 & 4808 $\pm$ 100 & -0.50 $\pm$ 0.20 & 3.561 $\pm$ 0.025 & 1.620 $\pm$ 0.016 & 3.05 $\pm$ 0.04 & G8III & 0.060 $\pm$ 0.030 &  \\
                        & 45.8 $\pm$ 0.7 & 4797 $\pm$ 99 & $\shortparallel$ & 3.504 $\pm$ 0.028 & 1.660 $\pm$ 0.017 & 3.00 $\pm$ 0.04 & G8III & $\shortparallel$ &  \\
OGLE-LMC-ECL01866 & 47.0 $\pm$ 0.6 & 4539 $\pm$ 84 & -0.70 $\pm$ 0.10 & 3.57 $\pm$ 0.04 & 1.648 $\pm$ 0.011 & 2.93 $\pm$ 0.03 &  & 0.115 $\pm$ 0.020 &  \\
                        & 28.2 $\pm$ 1.1 & 5321 $\pm$ 74 & $\shortparallel$ & 3.575 $\pm$ 0.028 & 2.09 $\pm$ 0.03 & 2.76 $\pm$ 0.04 &  & $\shortparallel$ &  \\
OGLE-LMC-ECL26122 & 32.7 $\pm$ 0.5 & 4989 $\pm$ 80 & -0.15 $\pm$ 0.10 & 3.59 $\pm$ 0.05 & 1.964 $\pm$ 0.014 & 2.78 $\pm$ 0.03 &  & 0.140 $\pm$ 0.020 &  \\
                        & 23.0 $\pm$ 0.5 & 5000 $\pm$ 81 & $\shortparallel$ & 3.41 $\pm$ 0.05 & 2.248 $\pm$ 0.018 & 2.47 $\pm$ 0.03 &  & $\shortparallel$ &  \\
OGLE-LMC-ECL06575 & 49.4 $\pm$ 1.4 & 4677 $\pm$ 75 & -0.45 $\pm$ 0.10 & 3.97 $\pm$ 0.03 & 1.650 $\pm$ 0.026 & 3.02 $\pm$ 0.04 &  & 0.107 $\pm$ 0.020 &  \\
                        & 39.8 $\pm$ 1.4 & 4898 $\pm$ 68 & $\shortparallel$ & 4.152 $\pm$ 0.030 & 1.857 $\pm$ 0.029 & 2.91 $\pm$ 0.04 &  & $\shortparallel$ &  \\
OGLE SMC108.1 14904 & 64.0 $\pm$ 0.5 & 4955 $\pm$ 91 & -0.79 $\pm$ 0.15 & 4.43 $\pm$ 0.04 & 1.472 $\pm$ 0.010 & 3.35 $\pm$ 0.03 & G7II & 0.093 $\pm$ 0.028 &  \\
                        & 46.9 $\pm$ 0.5 & 5675 $\pm$ 105 & $\shortparallel$ & 4.42 $\pm$ 0.04 & 1.740 $\pm$ 0.014 & 3.31 $\pm$ 0.03 & F9II & $\shortparallel$ &  \\
ASAS J180057-2333.8 & 67.6 $\pm$ 1.4 & 4207 $\pm$ 78 & -0.14 $\pm$ 0.10 & 4.875 $\pm$ 0.021 & 1.466 $\pm$ 0.018 & 3.11 $\pm$ 0.04 & K4II & 0.52 $\pm$ 0.07 & 1561 $\pm$ 113 \\
                        & 52.1 $\pm$ 1.4 & 4539 $\pm$ 84 & $\shortparallel$ & 4.914 $\pm$ 0.021 & 1.696 $\pm$ 0.023 & 3.02 $\pm$ 0.04 & K1II & $\shortparallel$ & $\shortparallel$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleI:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    System & $R$               & $T_{eff}$ & [Fe/H]      & $M$              & $\log g$              &  $\log L$                 &  $SpT/LC$  & $E(B-V)$        &  $d$    \\
                 & ($R_{\sun}$) & ($\,K$)     & ($dex$)   &  ($M_{\sun}$) & ($g$: cm s$^{-2}$)  & ($L$:  $L_{\sun}$)     &                    & ($mag$)         &  ($pc$)     \\
    \hline
CV Vel & 4.080 $\pm$ 0.030 & 17989 $\pm$ 497 & -0.14 $\pm$ 0.15 & 6.067 $\pm$ 0.011 & 4.000 $\pm$ 0.008 & 3.20 $\pm$ 0.05 & B2.5V & 0.035 $\pm$ 0.020 & 652 $\pm$ 15 \\
                        & 3.940 $\pm$ 0.030 & 17783 $\pm$ 491 & $\shortparallel$ & 5.953 $\pm$ 0.011 & 4.021 $\pm$ 0.008 & 3.15 $\pm$ 0.05 & B2.5V & $\shortparallel$ & $\shortparallel$ \\
V380 Cyg & 15.71 $\pm$ 0.13 & 21677 $\pm$ 299 & -0.02 $\pm$ 0.05 & 11.43 $\pm$ 0.19 & 3.104 $\pm$ 0.006 & 4.691 $\pm$ 0.025 & B1.5III & 0.457 $\pm$ 0.015 & 649 $\pm$ 101 \\
                        & 3.82 $\pm$ 0.05 & 22699 $\pm$ 1202 & $\shortparallel$ & 7.00 $\pm$ 0.14 & 4.120 $\pm$ 0.011 & 3.54 $\pm$ 0.09 & B2V & $\shortparallel$ & $\shortparallel$ \\
V453 Cyg & 8.55 $\pm$ 0.06 & 27925 $\pm$ 386 & -0.25 $\pm$ 0.05 & 14.36 $\pm$ 0.20 & 3.731 $\pm$ 0.012 & 4.603 $\pm$ 0.025 & B0.4IV & 0.460 $\pm$ 0.030 & 1518 $\pm$ 89 \\
                        & 5.49 $\pm$ 0.06 & 25704 $\pm$ 473 & $\shortparallel$ & 11.11 $\pm$ 0.13 & 4.005 $\pm$ 0.015 & 4.07 $\pm$ 0.03 & B0.7IV & $\shortparallel$ & $\shortparallel$ \\
V578 Mon & 5.41 $\pm$ 0.04 & 29992 $\pm$ 483 & -0.30 $\pm$ 0.13 & 14.54 $\pm$ 0.08 & 4.133 $\pm$ 0.018 & 4.329 $\pm$ 0.029 & B1V & 0.455 $\pm$ 0.029 & 1600 $\pm$ 200 \\
                        & 4.29 $\pm$ 0.05 & 25763 $\pm$ 415 & $\shortparallel$ & 10.29 $\pm$ 0.06 & 4.185 $\pm$ 0.021 & 3.864 $\pm$ 0.030 & B2V & $\shortparallel$ & $\shortparallel$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}



\begin{landscape}
 \begin{table}
  \caption{
Literature stellar parameters of DEB stars in Sample II, with adopted solar metallicity: radius ($R$), effective temperature ($T_{eff}$), 
iron abundance [Fe/H], and mass ($M$), surface gravity ($\log g$), luminosity ($\log L$), spectral type ($SpT$)/luminosity class ($LC$), 
color excess $E(B-V)$, and distance $d$.
References for the literature values are given in the main text.
}
%{\tiny
  \label{tab:sampleII}
  \begin{tabular}{ccccccccccc}
    \hline
    System & $R$               & $T_{eff}$ & [Fe/H]      & $M$              & $\log g$              &  $\log L$                 &  $SpT/LC$  & $E(B-V)$        &  $d$    \\
                 & ($R_{\sun}$) & ($\,K$)     & ($dex$)   &  ($M_{\sun}$) & ($g$: cm s$^{-2}$)  & ($L$:  $L_{\sun}$)     &                    & ($mag$)         &  ($pc$) \\
    \hline
EPIC 203710387 & 0.446 $\pm$ 0.014 & 2851 $\pm$ 144 & 0.00 $\pm$ 0.19 & 0.108 $\pm$ 0.003 & 4.170 $\pm$ 0.022 & -1.93 $\pm$ 0.09 & M5V & 0 &  \\
                        & 0.420 $\pm$ 0.011 & 2891 $\pm$ 146 & $\shortparallel$ & 0.118 $\pm$ 0.004 & 4.263 $\pm$ 0.024 & -1.95 $\pm$ 0.09 & M4.5V & $\shortparallel$ &  \\
UScoCTIO 5 & 0.862 $\pm$ 0.012 & 3199 $\pm$ 74 & 0.00 $\pm$ 0.19 & 0.3336 $\pm$ 0.0022 & 4.090 $\pm$ 0.012 & -1.15 $\pm$ 0.04 & M4.5V & 0.246 $\pm$ 0.004 &  \\
                        & 0.852 $\pm$ 0.013 & 3199 $\pm$ 74 & $\shortparallel$ & 0.3200 $\pm$ 0.0022 & 4.082 $\pm$ 0.012 & -1.16 $\pm$ 0.04 & M4.5V & $\shortparallel$ &  \\
LSPM J1112+7626 & 0.386 $\pm$ 0.005 & 3062 $\pm$ 169 & 0.00 $\pm$ 0.19 & 0.3946 $\pm$ 0.0023 & 4.861 $\pm$ 0.012 & -1.93 $\pm$ 0.10 & M4V & 0 & 56.77 $\pm$ 0.16 \\
                        & 0.298 $\pm$ 0.005 & 2951 $\pm$ 156 & $\shortparallel$ & 0.2745 $\pm$ 0.0012 & 4.929 $\pm$ 0.014 & -2.22 $\pm$ 0.09 &  & $\shortparallel$ & $\shortparallel$ \\
CU Cnc & 0.432 $\pm$ 0.005 & 3162 $\pm$ 153 & 0.00 $\pm$ 0.19 & 0.4333 $\pm$ 0.0017 & 4.804 $\pm$ 0.011 & -1.77 $\pm$ 0.08 & M3.5Ve & 0 & 16.601 $\pm$ 0.022 \\
                        & 0.391 $\pm$ 0.009 & 3126 $\pm$ 151 & $\shortparallel$ & 0.3980 $\pm$ 0.0014 & 4.854 $\pm$ 0.021 & -1.88 $\pm$ 0.09 & M3.5Ve & $\shortparallel$ & $\shortparallel$ \\
MG1-2056316 & 0.4410 $\pm$ 0.0030 & 3459 $\pm$ 175 & 0.00 $\pm$ 0.19 & 0.4690 $\pm$ 0.0021 & 4.820 $\pm$ 0.006 & -1.60 $\pm$ 0.09 & M2V & 0 & 188 $\pm$ 4 \\
                        & 0.3740 $\pm$ 0.0030 & 3319 $\pm$ 168 & $\shortparallel$ & 0.3820 $\pm$ 0.0020 & 4.874 $\pm$ 0.007 & -1.82 $\pm$ 0.09 & M3V & $\shortparallel$ & $\shortparallel$ \\
MG1-78457 & 0.505 $\pm$ 0.011 & 3327 $\pm$ 100 & 0.00 $\pm$ 0.19 & 0.5270 $\pm$ 0.0019 & 4.753 $\pm$ 0.019 & -1.55 $\pm$ 0.06 & M3V & 0.084 $\pm$ 0.003 & 325 $\pm$ 11 \\
                        & 0.471 $\pm$ 0.012 & 3273 $\pm$ 98 & $\shortparallel$ & 0.4910 $\pm$ 0.0020 & 4.783 $\pm$ 0.022 & -1.64 $\pm$ 0.06 & M4V & $\shortparallel$ & $\shortparallel$ \\
MG1-116309 & 0.552 $\pm$ 0.013 & 3917 $\pm$ 99 & 0.00 $\pm$ 0.19 & 0.5670 $\pm$ 0.0020 & 4.708 $\pm$ 0.020 & -1.19 $\pm$ 0.05 & K8V & 0.0586 $\pm$ 0.0016 & 291 $\pm$ 3 \\
                        & 0.532 $\pm$ 0.009 & 3811 $\pm$ 97 & $\shortparallel$ & 0.5320 $\pm$ 0.0020 & 4.712 $\pm$ 0.015 & -1.27 $\pm$ 0.05 & M0V & $\shortparallel$ & $\shortparallel$ \\
MG1-506664 & 0.560 $\pm$ 0.005 & 3733 $\pm$ 103 & 0.00 $\pm$ 0.19 & 0.5840 $\pm$ 0.0020 & 4.708 $\pm$ 0.008 & -1.26 $\pm$ 0.05 & M1V & 0.056 $\pm$ 0.004 & 259.1 $\pm$ 2.9 \\
                        & 0.513 $\pm$ 0.008 & 3614 $\pm$ 100 & $\shortparallel$ & 0.5440 $\pm$ 0.0020 & 4.753 $\pm$ 0.013 & -1.39 $\pm$ 0.05 & M2V & $\shortparallel$ & $\shortparallel$ \\
GU Boo & 0.623 $\pm$ 0.016 & 3917 $\pm$ 126 & 0.00 $\pm$ 0.19 & 0.610 $\pm$ 0.007 & 4.634 $\pm$ 0.023 & -1.08 $\pm$ 0.06 & M1V & 0 & 162.7 $\pm$ 0.4 \\
                        & 0.620 $\pm$ 0.020 & 3811 $\pm$ 132 & $\shortparallel$ & 0.599 $\pm$ 0.006 & 4.630 $\pm$ 0.028 & -1.14 $\pm$ 0.07 & M1V & $\shortparallel$ & $\shortparallel$ \\
ASAS J082552-1622.8 & 0.694 $\pm$ 0.009 & 4207 $\pm$ 203 & 0.00 $\pm$ 0.19 & 0.703 $\pm$ 0.005 & 4.600 $\pm$ 0.016 & -0.87 $\pm$ 0.08 & K7V & 0 & 46 $\pm$ 5 \\
                        & 0.699 $\pm$ 0.013 & 4083 $\pm$ 197 & $\shortparallel$ & 0.687 $\pm$ 0.005 & 4.585 $\pm$ 0.016 & -0.91 $\pm$ 0.09 & M0V & $\shortparallel$ & $\shortparallel$ \\
1SWASP J093010.78+533859.5 & 0.757 $\pm$ 0.008 & 5000 $\pm$ 196 & 0.00 $\pm$ 0.19 & 0.766 $\pm$ 0.014 & 4.564 $\pm$ 0.012 & -0.49 $\pm$ 0.07 & K1V & 0 & 42.4 $\pm$ 2.4 \\
                        & 0.743 $\pm$ 0.010 & 4236 $\pm$ 205 & $\shortparallel$ & 0.644 $\pm$ 0.012 & 4.505 $\pm$ 0.014 & -0.80 $\pm$ 0.08 & K5V & $\shortparallel$ & $\shortparallel$ \\
ASAS J212954-5620.1 & 0.845 $\pm$ 0.012 & 4753 $\pm$ 153 & 0.00 $\pm$ 0.19 & 0.833 $\pm$ 0.017 & 4.506 $\pm$ 0.012 & -0.48 $\pm$ 0.06 &  & 0 & 120.5 $\pm$ 0.4 \\
                        & 0.718 $\pm$ 0.017 & 4217 $\pm$ 184 & $\shortparallel$ & 0.703 $\pm$ 0.013 & 4.574 $\pm$ 0.020 & -0.83 $\pm$ 0.08 &  & $\shortparallel$ & $\shortparallel$ \\
ASAS J045304-0700.4 & 0.848 $\pm$ 0.005 & 5321 $\pm$ 196 & 0.00 $\pm$ 0.19 & 0.834 $\pm$ 0.004 & 4.503 $\pm$ 0.005 & -0.28 $\pm$ 0.06 & K2V & 0 & 133.7 $\pm$ 0.6 \\
                        & 0.833 $\pm$ 0.005 & 5105 $\pm$ 200 & $\shortparallel$ & 0.828 $\pm$ 0.004 & 4.515 $\pm$ 0.005 & -0.37 $\pm$ 0.07 & K4V & $\shortparallel$ & $\shortparallel$ \\
HS Aur & 1.004 $\pm$ 0.024 & 5346 $\pm$ 74 & 0.00 $\pm$ 0.19 & 0.900 $\pm$ 0.019 & 4.389 $\pm$ 0.023 & -0.13 $\pm$ 0.03 & G8V & 0 & 135.8 $\pm$ 0.7 \\
                        & 0.873 $\pm$ 0.024 & 5200 $\pm$ 72 & $\shortparallel$ & 0.879 $\pm$ 0.017 & 4.500 $\pm$ 0.025 & -0.30 $\pm$ 0.03 & K0V & $\shortparallel$ & $\shortparallel$ \\
CG Cyg & 0.890 $\pm$ 0.013 & 5260 $\pm$ 182 & 0.00 $\pm$ 0.19 & 0.940 $\pm$ 0.012 & 4.512 $\pm$ 0.014 & -0.26 $\pm$ 0.06 & G9V & 0 & 97.5 $\pm$ 0.3 \\
                        & 0.840 $\pm$ 0.014 & 4721 $\pm$ 65 & $\shortparallel$ & 0.810 $\pm$ 0.013 & 4.505 $\pm$ 0.016 & -0.501 $\pm$ 0.028 & K3V & $\shortparallel$ & $\shortparallel$ \\
HP Aur & 1.028 $\pm$ 0.004 & 5808 $\pm$ 120 & 0.00 $\pm$ 0.19 & 0.954 $\pm$ 0.004 & 4.394 $\pm$ 0.004 & 0.03 $\pm$ 0.04 & G2V & 0.048 $\pm$ 0.020 & 191.9 $\pm$ 3.0 \\
                        & 0.776 $\pm$ 0.003 & 5164 $\pm$ 119 & $\shortparallel$ & 0.809 $\pm$ 0.004 & 4.567 $\pm$ 0.004 & -0.41 $\pm$ 0.04 & K1V & $\shortparallel$ & $\shortparallel$ \\
V1174 Ori & 1.339 $\pm$ 0.015 & 4467 $\pm$ 123 & 0.00 $\pm$ 0.19 & 1.009 $\pm$ 0.015 & 4.190 $\pm$ 0.010 & -0.19 $\pm$ 0.05 & K4.5V & 0.100 $\pm$ 0.010 & 367 $\pm$ 3 \\
                        & 1.065 $\pm$ 0.011 & 3614 $\pm$ 100 & $\shortparallel$ & 0.731 $\pm$ 0.008 & 4.250 $\pm$ 0.010 & -0.76 $\pm$ 0.05 & M1.5V & $\shortparallel$ & $\shortparallel$ \\
CV Boo & 1.262 $\pm$ 0.023 & 5754 $\pm$ 146 & 0.00 $\pm$ 0.19 & 1.032 $\pm$ 0.013 & 4.294 $\pm$ 0.016 & 0.20 $\pm$ 0.05 & G2V & 0.0153 $\pm$ 0.0005 & 251.8 $\pm$ 1.5 \\
                        & 1.173 $\pm$ 0.023 & 5675 $\pm$ 144 & $\shortparallel$ & 0.968 $\pm$ 0.012 & 4.285 $\pm$ 0.017 & 0.11 $\pm$ 0.05 & G3V & $\shortparallel$ & $\shortparallel$ \\
V1094 Tau & 1.411 $\pm$ 0.006 & 5848 $\pm$ 94 & 0.00 $\pm$ 0.19 & 1.096 $\pm$ 0.004 & 4.179 $\pm$ 0.004 & 0.322 $\pm$ 0.028 & G0V & 0 & 123.7 $\pm$ 0.8 \\
                        & 1.106 $\pm$ 0.007 & 5702 $\pm$ 105 & $\shortparallel$ & 1.0120 $\pm$ 0.0028 & 4.355 $\pm$ 0.005 & 0.07 $\pm$ 0.03 & G3V & $\shortparallel$ & $\shortparallel$ \\
HP Dra & 1.371 $\pm$ 0.012 & 5998 $\pm$ 152 & 0.00 $\pm$ 0.19 & 1.133 $\pm$ 0.005 & 4.218 $\pm$ 0.010 & 0.34 $\pm$ 0.04 & F9V & 0 & 80.06 $\pm$ 0.19 \\
                        & 1.052 $\pm$ 0.010 & 5888 $\pm$ 149 & $\shortparallel$ & 1.094 $\pm$ 0.007 & 4.433 $\pm$ 0.011 & 0.08 $\pm$ 0.04 & F9V & $\shortparallel$ & $\shortparallel$ \\
ZZ UMa & 1.520 $\pm$ 0.020 & 5957 $\pm$ 69 & 0.00 $\pm$ 0.19 & 1.142 $\pm$ 0.007 & 4.135 $\pm$ 0.011 & 0.418 $\pm$ 0.023 & F8V & 0.008 $\pm$ 0.004 & 178.9 $\pm$ 1.1 \\
                        & 1.160 $\pm$ 0.010 & 5272 $\pm$ 85 & $\shortparallel$ & 0.972 $\pm$ 0.007 & 4.299 $\pm$ 0.007 & -0.028 $\pm$ 0.029 & G6V & $\shortparallel$ & $\shortparallel$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleII:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    System & $R$               & $T_{eff}$ & [Fe/H]      & $M$              & $\log g$              &  $\log L$                 &  $SpT/LC$  & $E(B-V)$        &  $d$    \\
                 & ($R_{\sun}$) & ($\,K$)     & ($dex$)   &  ($M_{\sun}$) & ($g$: cm s$^{-2}$)  & ($L$:  $L_{\sun}$)     &                    & ($mag$)         &  ($pc$) \\
    \hline
V2080 Cyg & 1.596 $\pm$ 0.008 & 5998 $\pm$ 69 & 0.00 $\pm$ 0.19 & 1.191 $\pm$ 0.017 & 4.1080 $\pm$ 0.0030 & 0.473 $\pm$ 0.020 & F4V & 0 & 85.45 $\pm$ 0.24 \\
                        & 1.599 $\pm$ 0.008 & 5984 $\pm$ 69 & $\shortparallel$ & 1.157 $\pm$ 0.017 & 4.0930 $\pm$ 0.0030 & 0.470 $\pm$ 0.020 & F4V & $\shortparallel$ & $\shortparallel$ \\
FL Lyr & 1.282 $\pm$ 0.028 & 6152 $\pm$ 99 & 0.00 $\pm$ 0.19 & 1.221 $\pm$ 0.016 & 4.309 $\pm$ 0.020 & 0.33 $\pm$ 0.03 & F8V & 0 & 135.0 $\pm$ 0.5 \\
                        & 0.962 $\pm$ 0.028 & 5297 $\pm$ 98 & $\shortparallel$ & 0.960 $\pm$ 0.012 & 4.454 $\pm$ 0.026 & -0.18 $\pm$ 0.04 & G8V & $\shortparallel$ & $\shortparallel$ \\
V2154 Cyg & 1.477 $\pm$ 0.012 & 6776 $\pm$ 156 & 0.00 $\pm$ 0.19 & 1.269 $\pm$ 0.017 & 4.203 $\pm$ 0.009 & 0.62 $\pm$ 0.04 & F3V & 0 & 93 $\pm$ 5 \\
                        & 0.723 $\pm$ 0.009 & 5023 $\pm$ 150 & $\shortparallel$ & 0.754 $\pm$ 0.006 & 4.597 $\pm$ 0.012 & -0.52 $\pm$ 0.05 & K2V & $\shortparallel$ & $\shortparallel$ \\
V1061 Cyg & 1.615 $\pm$ 0.017 & 6180 $\pm$ 100 & 0.00 $\pm$ 0.19 & 1.282 $\pm$ 0.015 & 4.129 $\pm$ 0.011 & 0.535 $\pm$ 0.029 & F9V & 0 & 169.8 $\pm$ 0.9 \\
                        & 0.974 $\pm$ 0.020 & 5297 $\pm$ 146 & $\shortparallel$ & 0.932 $\pm$ 0.007 & 4.430 $\pm$ 0.018 & -0.17 $\pm$ 0.05 & G8V & $\shortparallel$ & $\shortparallel$ \\
CF Tau & 2.797 $\pm$ 0.011 & 5200 $\pm$ 156 & 0.00 $\pm$ 0.19 & 1.282 $\pm$ 0.009 & 3.653 $\pm$ 0.005 & 0.71 $\pm$ 0.05 & K0 & 0.280 $\pm$ 0.010 & 272 $\pm$ 7 \\
                        & 2.048 $\pm$ 0.016 & 5998 $\pm$ 152 & $\shortparallel$ & 1.251 $\pm$ 0.011 & 3.913 $\pm$ 0.008 & 0.69 $\pm$ 0.04 & G0 & $\shortparallel$ & $\shortparallel$ \\
HS Hya & 1.293 $\pm$ 0.009 & 6500 $\pm$ 49 & 0.00 $\pm$ 0.19 & 1.308 $\pm$ 0.018 & 4.332 $\pm$ 0.005 & 0.429 $\pm$ 0.015 & F5V & 0 & 105.6 $\pm$ 0.8 \\
                        & 1.234 $\pm$ 0.009 & 6400 $\pm$ 50 & $\shortparallel$ & 1.267 $\pm$ 0.017 & 4.359 $\pm$ 0.005 & 0.362 $\pm$ 0.015 & F5V & $\shortparallel$ & $\shortparallel$ \\
UZ Dra & 1.310 $\pm$ 0.030 & 6209 $\pm$ 114 & 0.00 $\pm$ 0.19 & 1.340 $\pm$ 0.020 & 4.330 $\pm$ 0.030 & 0.36 $\pm$ 0.04 & F7V & 0.012 $\pm$ 0.007 & 186.6 $\pm$ 0.9 \\
                        & 1.150 $\pm$ 0.020 & 5984 $\pm$ 110 & $\shortparallel$ & 1.230 $\pm$ 0.020 & 4.400 $\pm$ 0.030 & 0.18 $\pm$ 0.04 & G0V & $\shortparallel$ & $\shortparallel$ \\
V1143 Cyg & 1.346 $\pm$ 0.023 & 6457 $\pm$ 104 & 0.00 $\pm$ 0.19 & 1.355 $\pm$ 0.004 & 4.323 $\pm$ 0.016 & 0.45 $\pm$ 0.03 & F5V & 0 & 40.47 $\pm$ 0.07 \\
                        & 1.323 $\pm$ 0.023 & 6397 $\pm$ 103 & $\shortparallel$ & 1.327 $\pm$ 0.003 & 4.324 $\pm$ 0.016 & 0.42 $\pm$ 0.03 & F5V & $\shortparallel$ & $\shortparallel$ \\
VZ Cep & 1.534 $\pm$ 0.012 & 6668 $\pm$ 154 & 0.00 $\pm$ 0.19 & 1.402 $\pm$ 0.015 & 4.213 $\pm$ 0.008 & 0.62 $\pm$ 0.04 & F3V & 0.044 $\pm$ 0.010 & 228.1 $\pm$ 1.6 \\
                        & 1.04 $\pm$ 0.04 & 5715 $\pm$ 118 & $\shortparallel$ & 1.108 $\pm$ 0.008 & 4.45 $\pm$ 0.03 & 0.02 $\pm$ 0.05 & G4V & $\shortparallel$ & $\shortparallel$ \\
BF Dra & 2.086 $\pm$ 0.012 & 6353 $\pm$ 161 & 0.00 $\pm$ 0.19 & 1.4138 $\pm$ 0.0029 & 3.950 $\pm$ 0.005 & 0.81 $\pm$ 0.04 & F6V & 0.026 $\pm$ 0.010 & 347 $\pm$ 3 \\
                        & 1.922 $\pm$ 0.012 & 6397 $\pm$ 147 & $\shortparallel$ & 1.3750 $\pm$ 0.0028 & 4.008 $\pm$ 0.005 & 0.75 $\pm$ 0.04 & F6V & $\shortparallel$ & $\shortparallel$ \\
DM Vir & 1.763 $\pm$ 0.017 & 6501 $\pm$ 105 & 0.00 $\pm$ 0.19 & 1.454 $\pm$ 0.008 & 4.108 $\pm$ 0.009 & 0.699 $\pm$ 0.029 & F7V & 0.023 $\pm$ 0.010 & 191.7 $\pm$ 2.6 \\
                        & 1.763 $\pm$ 0.017 & 6501 $\pm$ 105 & $\shortparallel$ & 1.448 $\pm$ 0.008 & 4.106 $\pm$ 0.009 & 0.699 $\pm$ 0.029 & F7V & $\shortparallel$ & $\shortparallel$ \\
HD 71636 & 1.571 $\pm$ 0.009 & 6950 $\pm$ 128 & 0.00 $\pm$ 0.19 & 1.513 $\pm$ 0.009 & 4.230 $\pm$ 0.010 & 0.72 $\pm$ 0.03 & F2V & 0 & 121.3 $\pm$ 1.0 \\
                        & 1.361 $\pm$ 0.008 & 6442 $\pm$ 133 & $\shortparallel$ & 1.285 $\pm$ 0.007 & 4.280 $\pm$ 0.010 & 0.46 $\pm$ 0.04 & F5V & $\shortparallel$ & $\shortparallel$ \\
RZ Cha & 2.264 $\pm$ 0.017 & 6457 $\pm$ 149 & 0.00 $\pm$ 0.19 & 1.518 $\pm$ 0.021 & 3.909 $\pm$ 0.009 & 0.90 $\pm$ 0.04 & F5V & 0.038 $\pm$ 0.020 & 174.7 $\pm$ 0.8 \\
                        & 2.264 $\pm$ 0.017 & 6457 $\pm$ 149 & $\shortparallel$ & 1.509 $\pm$ 0.027 & 3.907 $\pm$ 0.010 & 0.90 $\pm$ 0.04 & F5V & $\shortparallel$ & $\shortparallel$ \\
EY Cep & 1.463 $\pm$ 0.008 & 7096 $\pm$ 163 & 0.00 $\pm$ 0.19 & 1.523 $\pm$ 0.008 & 4.290 $\pm$ 0.006 & 0.69 $\pm$ 0.04 & F0V & 0.049 $\pm$ 0.012 & 299.3 $\pm$ 2.5 \\
                        & 1.468 $\pm$ 0.010 & 6966 $\pm$ 160 & $\shortparallel$ & 1.498 $\pm$ 0.014 & 4.280 $\pm$ 0.006 & 0.66 $\pm$ 0.04 & F0V & $\shortparallel$ & $\shortparallel$ \\
V442 Cyg & 2.07 $\pm$ 0.03 & 6902 $\pm$ 95 & 0.00 $\pm$ 0.19 & 1.564 $\pm$ 0.024 & 3.999 $\pm$ 0.016 & 0.943 $\pm$ 0.028 & F1V & 0.080 $\pm$ 0.010 & 340 $\pm$ 4 \\
                        & 1.66 $\pm$ 0.03 & 6808 $\pm$ 94 & $\shortparallel$ & 1.410 $\pm$ 0.023 & 4.146 $\pm$ 0.019 & 0.728 $\pm$ 0.030 & F2V & $\shortparallel$ & $\shortparallel$ \\
PV Pup & 1.542 $\pm$ 0.018 & 6918 $\pm$ 303 & 0.00 $\pm$ 0.19 & 1.565 $\pm$ 0.011 & 4.257 $\pm$ 0.010 & 0.69 $\pm$ 0.08 & A8V & 0 & 86.2 $\pm$ 0.3 \\
                        & 1.499 $\pm$ 0.018 & 6934 $\pm$ 303 & $\shortparallel$ & 1.554 $\pm$ 0.013 & 4.278 $\pm$ 0.011 & 0.67 $\pm$ 0.08 & A8V & $\shortparallel$ & $\shortparallel$ \\
FS Mon & 2.051 $\pm$ 0.012 & 6714 $\pm$ 93 & 0.00 $\pm$ 0.19 & 1.632 $\pm$ 0.012 & 4.026 $\pm$ 0.005 & 0.887 $\pm$ 0.025 & F2V & 0.023 $\pm$ 0.008 & 339 $\pm$ 5 \\
                        & 1.629 $\pm$ 0.012 & 6546 $\pm$ 106 & $\shortparallel$ & 1.462 $\pm$ 0.010 & 4.179 $\pm$ 0.006 & 0.642 $\pm$ 0.029 & F4V & $\shortparallel$ & $\shortparallel$ \\
IO Aqr & 2.493 $\pm$ 0.017 & 6339 $\pm$ 131 & 0.00 $\pm$ 0.19 & 1.655 $\pm$ 0.004 & 3.863 $\pm$ 0.006 & 0.96 $\pm$ 0.04 & F6V-IV & 0.0698 $\pm$ 0.0012 & 255.4 $\pm$ 2.3 \\
                        & 2.191 $\pm$ 0.015 & 6471 $\pm$ 134 & $\shortparallel$ & 1.569 $\pm$ 0.004 & 3.952 $\pm$ 0.006 & 0.88 $\pm$ 0.04 & F5V-IV & $\shortparallel$ & $\shortparallel$ \\
EI Cep & 2.90 $\pm$ 0.05 & 6745 $\pm$ 109 & 0.00 $\pm$ 0.19 & 1.772 $\pm$ 0.007 & 3.763 $\pm$ 0.014 & 1.19 $\pm$ 0.03 & F3IV & 0.007 $\pm$ 0.005 & 199.1 $\pm$ 1.1 \\
                        & 2.33 $\pm$ 0.04 & 6950 $\pm$ 96 & $\shortparallel$ & 1.680 $\pm$ 0.006 & 3.929 $\pm$ 0.016 & 1.057 $\pm$ 0.029 & F1V & $\shortparallel$ & $\shortparallel$ \\
XY Cet & 1.87 $\pm$ 0.03 & 7870 $\pm$ 109 & 0.00 $\pm$ 0.19 & 1.773 $\pm$ 0.016 & 4.142 $\pm$ 0.016 & 1.084 $\pm$ 0.029 & A8Vm & 0.040 $\pm$ 0.020 & 296 $\pm$ 5 \\
                        & 1.773 $\pm$ 0.029 & 7621 $\pm$ 123 & $\shortparallel$ & 1.615 $\pm$ 0.014 & 4.149 $\pm$ 0.014 & 0.98 $\pm$ 0.03 & F0Vm & $\shortparallel$ & $\shortparallel$ \\
MY Cyg & 2.280 $\pm$ 0.020 & 7031 $\pm$ 194 & 0.00 $\pm$ 0.19 & 1.800 $\pm$ 0.030 & 3.980 $\pm$ 0.010 & 1.06 $\pm$ 0.05 & F0Vm & 0.048 $\pm$ 0.030 & 250.5 $\pm$ 2.4 \\
                        & 2.220 $\pm$ 0.020 & 7096 $\pm$ 196 & $\shortparallel$ & 1.820 $\pm$ 0.030 & 4.010 $\pm$ 0.010 & 1.05 $\pm$ 0.05 & F0Vm & $\shortparallel$ & $\shortparallel$ \\
HY Vir & 2.806 $\pm$ 0.008 & 6855 $\pm$ 126 & 0.00 $\pm$ 0.19 & 1.838 $\pm$ 0.009 & 3.8060 $\pm$ 0.0030 & 1.19 $\pm$ 0.03 & F0m & 0.0230 $\pm$ 0.0005 & 182.3 $\pm$ 2.3 \\
                        & 1.519 $\pm$ 0.008 & 6546 $\pm$ 121 & $\shortparallel$ & 1.404 $\pm$ 0.006 & 4.222 $\pm$ 0.004 & 0.58 $\pm$ 0.03 & F5V & $\shortparallel$ & $\shortparallel$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleII:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    System & $R$               & $T_{eff}$ & [Fe/H]      & $M$              & $\log g$              &  $\log L$                 &  $SpT/LC$  & $E(B-V)$        &  $d$    \\
                 & ($R_{\sun}$) & ($\,K$)     & ($dex$)   &  ($M_{\sun}$) & ($g$: cm s$^{-2}$)  & ($L$:  $L_{\sun}$)     &                    & ($mag$)         &  ($pc$) \\
    \hline
WW Aur & 1.927 $\pm$ 0.011 & 7962 $\pm$ 440 & 0.00 $\pm$ 0.19 & 1.964 $\pm$ 0.007 & 4.162 $\pm$ 0.007 & 1.13 $\pm$ 0.10 & A4Vm & 0 & 90.9 $\pm$ 0.7 \\
                        & 1.841 $\pm$ 0.011 & 7674 $\pm$ 424 & $\shortparallel$ & 1.814 $\pm$ 0.007 & 4.167 $\pm$ 0.007 & 1.02 $\pm$ 0.10 & A5Vm & $\shortparallel$ & $\shortparallel$ \\
V2365 Oph & 2.190 $\pm$ 0.009 & 9506 $\pm$ 197 & 0.00 $\pm$ 0.19 & 1.965 $\pm$ 0.017 & 4.0510 $\pm$ 0.0030 & 1.55 $\pm$ 0.04 & A1V & 0.250 $\pm$ 0.010 & 254.4 $\pm$ 2.8 \\
                        & 0.934 $\pm$ 0.004 & 6397 $\pm$ 206 & $\shortparallel$ & 1.056 $\pm$ 0.010 & 4.521 $\pm$ 0.004 & 0.12 $\pm$ 0.06 &  & $\shortparallel$ & $\shortparallel$ \\
VV Crv & 3.375 $\pm$ 0.010 & 6501 $\pm$ 195 & 0.00 $\pm$ 0.19 & 1.978 $\pm$ 0.010 & 3.678 $\pm$ 0.006 & 1.26 $\pm$ 0.05 & F5IV & 0 & 81.5 $\pm$ 0.6 \\
                        & 1.650 $\pm$ 0.008 & 6637 $\pm$ 199 & $\shortparallel$ & 1.513 $\pm$ 0.008 & 4.183 $\pm$ 0.009 & 0.68 $\pm$ 0.05 & F5V & $\shortparallel$ & $\shortparallel$ \\
KW Hya & 2.125 $\pm$ 0.016 & 7998 $\pm$ 203 & 0.00 $\pm$ 0.19 & 1.98 $\pm$ 0.04 & 4.079 $\pm$ 0.013 & 1.22 $\pm$ 0.04 & A5Vm & 0 & 85.7 $\pm$ 0.7 \\
                        & 1.480 $\pm$ 0.014 & 6902 $\pm$ 175 & $\shortparallel$ & 1.488 $\pm$ 0.017 & 4.270 $\pm$ 0.010 & 0.65 $\pm$ 0.04 & F0V & $\shortparallel$ & $\shortparallel$ \\
TV Nor & 1.839 $\pm$ 0.012 & 9120 $\pm$ 147 & 0.00 $\pm$ 0.19 & 2.053 $\pm$ 0.022 & 4.221 $\pm$ 0.010 & 1.324 $\pm$ 0.029 &  & 0.184 $\pm$ 0.019 & 305 $\pm$ 4 \\
                        & 1.550 $\pm$ 0.014 & 7798 $\pm$ 108 & $\shortparallel$ & 1.665 $\pm$ 0.018 & 4.278 $\pm$ 0.012 & 0.903 $\pm$ 0.025 &  & $\shortparallel$ & $\shortparallel$ \\
V596 Pup & 2.167 $\pm$ 0.020 & 9506 $\pm$ 197 & 0.00 $\pm$ 0.19 & 2.101 $\pm$ 0.022 & 4.089 $\pm$ 0.009 & 1.54 $\pm$ 0.04 & A1V & 0.022 $\pm$ 0.010 & 179 $\pm$ 26 \\
                        & 2.167 $\pm$ 0.020 & 9506 $\pm$ 197 & $\shortparallel$ & 2.099 $\pm$ 0.019 & 4.088 $\pm$ 0.009 & 1.54 $\pm$ 0.04 & A1V & $\shortparallel$ & $\shortparallel$ \\
V335 Ser & 2.030 $\pm$ 0.030 & 9016 $\pm$ 145 & 0.00 $\pm$ 0.19 & 2.147 $\pm$ 0.014 & 4.155 $\pm$ 0.011 & 1.39 $\pm$ 0.03 & A1V & 0.068 $\pm$ 0.007 & 202.3 $\pm$ 2.1 \\
                        & 1.73 $\pm$ 0.04 & 8511 $\pm$ 157 & $\shortparallel$ & 1.906 $\pm$ 0.008 & 4.241 $\pm$ 0.017 & 1.15 $\pm$ 0.04 & A3V & $\shortparallel$ & $\shortparallel$ \\
EE Peg & 2.090 $\pm$ 0.025 & 8710 $\pm$ 201 & 0.00 $\pm$ 0.19 & 2.151 $\pm$ 0.024 & 4.131 $\pm$ 0.010 & 1.35 $\pm$ 0.04 & A3m & 0 & 144.6 $\pm$ 1.4 \\
                        & 1.312 $\pm$ 0.013 & 6457 $\pm$ 297 & $\shortparallel$ & 1.332 $\pm$ 0.011 & 4.327 $\pm$ 0.008 & 0.43 $\pm$ 0.08 & F5V & $\shortparallel$ & $\shortparallel$ \\
V1647 Sgr & 1.831 $\pm$ 0.018 & 9594 $\pm$ 309 & 0.00 $\pm$ 0.19 & 2.19 $\pm$ 0.04 & 4.253 $\pm$ 0.012 & 1.41 $\pm$ 0.06 & A1V & 0 & 175.1 $\pm$ 2.8 \\
                        & 1.666 $\pm$ 0.017 & 9099 $\pm$ 293 & $\shortparallel$ & 1.97 $\pm$ 0.03 & 4.289 $\pm$ 0.012 & 1.23 $\pm$ 0.06 & A1V & $\shortparallel$ & $\shortparallel$ \\
PT Vel & 2.094 $\pm$ 0.020 & 9247 $\pm$ 149 & 0.00 $\pm$ 0.19 & 2.198 $\pm$ 0.016 & 4.138 $\pm$ 0.008 & 1.461 $\pm$ 0.029 & A0V & 0 & 173.6 $\pm$ 1.3 \\
                        & 1.559 $\pm$ 0.020 & 7638 $\pm$ 176 & $\shortparallel$ & 1.626 $\pm$ 0.009 & 4.263 $\pm$ 0.011 & 0.87 $\pm$ 0.04 & A8V & $\shortparallel$ & $\shortparallel$ \\
GZ CMa & 2.49 $\pm$ 0.03 & 8810 $\pm$ 345 & 0.00 $\pm$ 0.19 & 2.206 $\pm$ 0.019 & 3.989 $\pm$ 0.012 & 1.53 $\pm$ 0.07 & A3Vm & 0.070 $\pm$ 0.030 & 293 $\pm$ 4 \\
                        & 2.13 $\pm$ 0.04 & 8531 $\pm$ 334 & $\shortparallel$ & 2.005 $\pm$ 0.018 & 4.083 $\pm$ 0.016 & 1.34 $\pm$ 0.07 & A4:V & $\shortparallel$ & $\shortparallel$ \\
V624 Her & 3.03 $\pm$ 0.03 & 8147 $\pm$ 150 & 0.00 $\pm$ 0.19 & 2.282 $\pm$ 0.015 & 3.834 $\pm$ 0.010 & 1.56 $\pm$ 0.03 & A3Vm & 0 & 140.6 $\pm$ 1.2 \\
                        & 2.21 $\pm$ 0.03 & 7943 $\pm$ 146 & $\shortparallel$ & 1.881 $\pm$ 0.013 & 4.024 $\pm$ 0.014 & 1.24 $\pm$ 0.03 & A7V & $\shortparallel$ & $\shortparallel$ \\
$\beta$ Aur & 2.762 $\pm$ 0.017 & 9354 $\pm$ 194 & 0.00 $\pm$ 0.19 & 2.376 $\pm$ 0.027 & 3.932 $\pm$ 0.005 & 1.72 $\pm$ 0.04 & A1Vm & 0 & 24.87 $\pm$ 0.14 \\
                        & 2.568 $\pm$ 0.017 & 9204 $\pm$ 191 & $\shortparallel$ & 2.291 $\pm$ 0.027 & 3.979 $\pm$ 0.005 & 1.63 $\pm$ 0.04 & A1Vm & $\shortparallel$ & $\shortparallel$ \\
V1031 Ori & 4.32 $\pm$ 0.03 & 7852 $\pm$ 506 & 0.00 $\pm$ 0.19 & 2.473 $\pm$ 0.018 & 3.560 $\pm$ 0.008 & 1.81 $\pm$ 0.11 & A3V & 0 & 205 $\pm$ 31 \\
                        & 2.98 $\pm$ 0.06 & 8395 $\pm$ 503 & $\shortparallel$ & 2.286 $\pm$ 0.016 & 3.850 $\pm$ 0.019 & 1.60 $\pm$ 0.11 & A6V & $\shortparallel$ & $\shortparallel$ \\
TZ Men & 2.016 $\pm$ 0.020 & 10399 $\pm$ 407 & 0.00 $\pm$ 0.19 & 2.487 $\pm$ 0.025 & 4.225 $\pm$ 0.011 & 1.63 $\pm$ 0.07 & A0V & 0 & 123.0 $\pm$ 0.7 \\
                        & 1.432 $\pm$ 0.015 & 7194 $\pm$ 298 & $\shortparallel$ & 1.504 $\pm$ 0.010 & 4.303 $\pm$ 0.009 & 0.69 $\pm$ 0.07 & A8V & $\shortparallel$ & $\shortparallel$ \\
AR Aur & 1.799 $\pm$ 0.013 & 10940 $\pm$ 302 & 0.00 $\pm$ 0.19 & 2.544 $\pm$ 0.009 & 4.333 $\pm$ 0.008 & 1.62 $\pm$ 0.05 & B9V & 0 & 148.9 $\pm$ 2.1 \\
                        & 1.834 $\pm$ 0.019 & 10351 $\pm$ 310 & $\shortparallel$ & 2.358 $\pm$ 0.008 & 4.284 $\pm$ 0.010 & 1.54 $\pm$ 0.05 & B9V & $\shortparallel$ & $\shortparallel$ \\
V4089 Sgr & 3.964 $\pm$ 0.020 & 8433 $\pm$ 97 & 0.00 $\pm$ 0.19 & 2.584 $\pm$ 0.012 & 3.654 $\pm$ 0.005 & 1.855 $\pm$ 0.020 & A3III & 0 & 149.4 $\pm$ 2.0 \\
                        & 1.605 $\pm$ 0.007 & 7362 $\pm$ 102 & $\shortparallel$ & 1.607 $\pm$ 0.008 & 4.233 $\pm$ 0.004 & 0.834 $\pm$ 0.024 &  & $\shortparallel$ & $\shortparallel$ \\
V451 Oph & 2.64 $\pm$ 0.03 & 10789 $\pm$ 795 & 0.00 $\pm$ 0.19 & 2.78 $\pm$ 0.06 & 4.038 $\pm$ 0.015 & 1.93 $\pm$ 0.13 & B9V & 0.158 $\pm$ 0.010 & 303 $\pm$ 8 \\
                        & 2.028 $\pm$ 0.028 & 9795 $\pm$ 496 & $\shortparallel$ & 2.36 $\pm$ 0.05 & 4.196 $\pm$ 0.015 & 1.53 $\pm$ 0.09 & A0V & $\shortparallel$ & $\shortparallel$ \\
$\psi$ Cen & 3.621 $\pm$ 0.016 & 10447 $\pm$ 289 & 0.00 $\pm$ 0.19 & 3.08 $\pm$ 0.04 & 3.8100 $\pm$ 0.0030 & 2.15 $\pm$ 0.05 &  & 0 & 69.2 $\pm$ 2.2 \\
                        & 1.801 $\pm$ 0.008 & 8790 $\pm$ 304 & $\shortparallel$ & 1.891 $\pm$ 0.026 & 4.2040 $\pm$ 0.0030 & 1.24 $\pm$ 0.06 &  & $\shortparallel$ & $\shortparallel$ \\
IQ Per & 2.446 $\pm$ 0.026 & 12303 $\pm$ 227 & 0.00 $\pm$ 0.19 & 3.52 $\pm$ 0.07 & 4.208 $\pm$ 0.019 & 2.09 $\pm$ 0.03 & B8V & 0.140 $\pm$ 0.010 & 307 $\pm$ 5 \\
                        & 1.503 $\pm$ 0.017 & 7674 $\pm$ 141 & $\shortparallel$ & 1.74 $\pm$ 0.03 & 4.323 $\pm$ 0.013 & 0.85 $\pm$ 0.03 & A6V & $\shortparallel$ & $\shortparallel$ \\
$\chi^2$ Hya & 4.38 $\pm$ 0.04 & 11641 $\pm$ 268 & 0.00 $\pm$ 0.19 & 3.61 $\pm$ 0.08 & 3.712 $\pm$ 0.015 & 2.50 $\pm$ 0.04 & B8V & 0.016 $\pm$ 0.010 & 217 $\pm$ 4 \\
                        & 2.17 $\pm$ 0.04 & 10990 $\pm$ 253 & $\shortparallel$ & 2.64 $\pm$ 0.05 & 4.188 $\pm$ 0.019 & 1.79 $\pm$ 0.04 & B8V & $\shortparallel$ & $\shortparallel$ \\
$\zeta$ Phe & 2.851 $\pm$ 0.015 & 14555 $\pm$ 335 & 0.00 $\pm$ 0.19 & 3.930 $\pm$ 0.015 & 4.122 $\pm$ 0.009 & 2.52 $\pm$ 0.04 & B6V & 0 & 68 $\pm$ 3 \\
                        & 1.853 $\pm$ 0.023 & 11912 $\pm$ 192 & $\shortparallel$ & 2.551 $\pm$ 0.026 & 4.309 $\pm$ 0.012 & 1.794 $\pm$ 0.030 & B8V & $\shortparallel$ & $\shortparallel$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleII:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    System & $R$               & $T_{eff}$ & [Fe/H]      & $M$              & $\log g$              &  $\log L$                 &  $SpT/LC$  & $E(B-V)$        &  $d$    \\
                 & ($R_{\sun}$) & ($\,K$)     & ($dex$)   &  ($M_{\sun}$) & ($g$: cm s$^{-2}$)  & ($L$:  $L_{\sun}$)     &                    & ($mag$)         &  ($pc$) \\
    \hline
GG Lup & 2.379 $\pm$ 0.025 & 14757 $\pm$ 442 & 0.00 $\pm$ 0.19 & 4.12 $\pm$ 0.04 & 4.301 $\pm$ 0.011 & 2.38 $\pm$ 0.05 & B7V & 0 & 143 $\pm$ 4 \\
                        & 1.725 $\pm$ 0.019 & 10990 $\pm$ 607 & $\shortparallel$ & 2.509 $\pm$ 0.024 & 4.364 $\pm$ 0.010 & 1.59 $\pm$ 0.10 & B9V & $\shortparallel$ & $\shortparallel$ \\
V760 Sco & 3.01 $\pm$ 0.07 & 16904 $\pm$ 506 & 0.00 $\pm$ 0.19 & 4.98 $\pm$ 0.09 & 4.177 $\pm$ 0.021 & 2.82 $\pm$ 0.06 & B4V & 0.330 $\pm$ 0.010 & 295 $\pm$ 8 \\
                        & 2.64 $\pm$ 0.05 & 16218 $\pm$ 485 & $\shortparallel$ & 4.62 $\pm$ 0.07 & 4.259 $\pm$ 0.019 & 2.64 $\pm$ 0.05 & B4V & $\shortparallel$ & $\shortparallel$ \\
U Oph & 3.438 $\pm$ 0.020 & 16440 $\pm$ 250 & 0.00 $\pm$ 0.19 & 5.27 $\pm$ 0.09 & 4.068 $\pm$ 0.010 & 2.891 $\pm$ 0.027 & B5V & 0.198 $\pm$ 0.009 & 267 $\pm$ 9 \\
                        & 3.11 $\pm$ 0.03 & 15588 $\pm$ 251 & $\shortparallel$ & 4.74 $\pm$ 0.07 & 4.128 $\pm$ 0.012 & 2.711 $\pm$ 0.030 & B6V & $\shortparallel$ & $\shortparallel$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}




\begin{landscape}
 \begin{table}
  \caption{
Inferred stellar parameters of DEB stars in Sample I: absolute magnitudes in the B-band ($M_B$) and the V-band ($M_V$), bolometric correction ($BC$), mass ($M_m$), evolution stage ($ES$), probability $Pr$, distance ($d_m$), age ($\tau$), and grid used.}
%{\tiny
  \label{tab:sampleIb}
  \begin{tabular}{cccccccccc}
    \hline
    Binary & $M_B$       &  $M_V$         & $BC$        &    $M_m$          & $ES$  &  $Pr$    & $d_m$      &  $\tau$  & Grid \\
                 & ($mag$)     & ($mag$)        &  ($mag$)  &    ($M_{\sun}$)  &            &              & ($pc$)      & ($Gyr$)  &        \\
    \hline
CM Dra A & 14.47 $\pm$ 0.26 & 12.88 $\pm$ 0.26 & -2.50 $\pm$ 0.18 & 0.235 $\pm$ 0.004 & MS & 94 & 13.7 $\pm$ 2.8 & 7 $_{- 4}^{+ 4}$ & $I$ \\
CM Dra B & 14.7 $\pm$ 0.3 & 13.1 $\pm$ 0.3 & -2.59 $\pm$ 0.23 & 0.219 $\pm$ 0.003 & MS & 95 & $\shortparallel$ & 7 $_{- 4}^{+ 4}$ & $I$ \\
PTFEB 132.707+19.810 A & 13.43 $\pm$ 0.14 & 11.95 $\pm$ 0.14 & -2.43 $\pm$ 0.08 & 0.359 $\pm$ 0.010 & MS & 80 & 205 $\pm$ 69 & 3.2 $_{- 0.5}^{+ 7}$ & $I$ \\
PTFEB 132.707+19.810 B & 14.81 $\pm$ 0.26 & 13.27 $\pm$ 0.26 & -2.91 $\pm$ 0.13 & 0.254 $\pm$ 0.014 & MS & 96 & $\shortparallel$ & $\shortparallel$ & $I$ \\
PTFEB 132.707+19.810 A & 13.37 $\pm$ 0.14 & 11.89 $\pm$ 0.14 & -2.39 $\pm$ 0.08 & 0.367 $\pm$ 0.011 & PMS & 20 & 210 $\pm$ 71 & 0.77 $_{- 0.09}^{+ 1.2}$ & $I$ \\
PTFEB 132.707+19.810 B & 14.81 $\pm$ 0.26 & 13.27 $\pm$ 0.26 & -2.91 $\pm$ 0.13 & 0.254 $\pm$ 0.014 & MS & 96 & $\shortparallel$ & $\shortparallel$ & $I$ \\
HAT-TR-318-007 A & 12.60 $\pm$ 0.15 & 11.21 $\pm$ 0.16 & -2.30 $\pm$ 0.11 & 0.456 $\pm$ 0.005 & MS & 90 & 115 $\pm$ 24 & 3.3 $_{- 1.1}^{+ 7}$ & $I$ \\
HAT-TR-318-007 B & 14.77 $\pm$ 0.26 & 13.26 $\pm$ 0.28 & -3.00 $\pm$ 0.20 & 0.272 $\pm$ 0.006 & MS & 96 & $\shortparallel$ & $\shortparallel$ & $I$ \\
HAT-TR-318-007 A & 12.59 $\pm$ 0.26 & 11.20 $\pm$ 0.26 & -2.30 $\pm$ 0.17 & 0.455 $\pm$ 0.028 & PMS & 10 & 116 $\pm$ 26 & 1.2 $_{- 0.4}^{+ 0.4}$ & $I$ \\
HAT-TR-318-007 B & 14.77 $\pm$ 0.26 & 13.26 $\pm$ 0.28 & -3.00 $\pm$ 0.20 & 0.272 $\pm$ 0.006 & MS & 96 & $\shortparallel$ & $\shortparallel$ & $I$ \\
YY Gem A & 10.26 $\pm$ 0.21 & 8.91 $\pm$ 0.22 & -1.37 $\pm$ 0.13 & 0.620 $\pm$ 0.012 & MS & 95 & 14.4 $\pm$ 2.2 & 7 $_{- 4}^{+ 4}$ & $I$ \\
YY Gem B & 10.37 $\pm$ 0.23 & 9.01 $\pm$ 0.24 & -1.38 $\pm$ 0.14 & 0.604 $\pm$ 0.011 & MS & 92 & $\shortparallel$ & $\shortparallel$ & $I$ \\
M55 V54 A & 4.87 $\pm$ 0.04 & 4.47 $\pm$ 0.03 & -0.168 $\pm$ 0.005 & 0.746 $\pm$ 0.009 & MS & 99 & 4914 $\pm$ 1815 & 13.0 $_{- 1.0}^{+ 0.8}$ & $I$ \\
M55 V54 B & 7.68 $\pm$ 0.08 & 6.94 $\pm$ 0.07 & -0.297 $\pm$ 0.012 & 0.579 $\pm$ 0.014 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
M4 V69 A & 5.38 $\pm$ 0.08 & 4.92 $\pm$ 0.07 & -0.152 $\pm$ 0.006 & 0.764 $\pm$ 0.030 & MS & 100 & 1787 $\pm$ 394 & 13.0 $_{- 2.9}^{+ 0.8}$ & $I$ \\
M4 V69 B & 5.64 $\pm$ 0.08 & 5.15 $\pm$ 0.06 & -0.157 $\pm$ 0.005 & 0.743 $\pm$ 0.028 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
M4 V66 A & 5.15 $\pm$ 0.06 & 4.70 $\pm$ 0.05 & -0.147 $\pm$ 0.006 & 0.770 $\pm$ 0.025 & MS & 100 & 1786 $\pm$ 357 & 13.0 $_{- 2.1}^{+ 0.8}$ & $I$ \\
M4 V66 B & 5.56 $\pm$ 0.06 & 5.08 $\pm$ 0.05 & -0.155 $\pm$ 0.005 & 0.741 $\pm$ 0.022 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
M4 V65 A & 4.65 $\pm$ 0.06 & 4.22 $\pm$ 0.04 & -0.140 $\pm$ 0.005 & 0.783 $\pm$ 0.016 & MS & 99 & 1926 $\pm$ 410 & 13.0 $_{- 1.3}^{+ 0.8}$ & $I$ \\
M4 V65 B & 7.39 $\pm$ 0.14 & 6.64 $\pm$ 0.11 & -0.282 $\pm$ 0.024 & 0.620 $\pm$ 0.014 & MS & 53 & $\shortparallel$ & 13.0 $_{- 1.3}^{+ 0.8}$ & $I$ \\
M4 V65 A & 4.65 $\pm$ 0.06 & 4.22 $\pm$ 0.04 & -0.140 $\pm$ 0.005 & 0.783 $\pm$ 0.016 & MS & 99 & 1941 $\pm$ 413 & 12.2 $_{- 0.9}^{+ 0.9}$ & $I$ \\
M4 V65 B & 7.89 $\pm$ 0.22 & 7.03 $\pm$ 0.17 & -0.42 $\pm$ 0.06 & 0.585 $\pm$ 0.013 & PMS & 47 & $\shortparallel$ & 0.032 $_{- 0.004}^{+ 0.004}$ & $I$ \\
NGC 6362 V41 A & 4.81 $\pm$ 0.06 & 4.37 $\pm$ 0.05 & -0.137 $\pm$ 0.004 & 0.789 $\pm$ 0.022 & MS & 100 & 7498 $\pm$ 3441 & 13.0 $_{- 2.1}^{+ 0.8}$ & $I$ \\
NGC 6362 V41 B & 6.09 $\pm$ 0.08 & 5.54 $\pm$ 0.06 & -0.165 $\pm$ 0.006 & 0.718 $\pm$ 0.025 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
NGC 6362 V40 A & 4.32 $\pm$ 0.07 & 3.89 $\pm$ 0.05 & -0.132 $\pm$ 0.005 & 0.818 $\pm$ 0.019 & MS & 64 & 7740 $\pm$ 2798 & 11.8 $_{- 1.3}^{+ 0.6}$ & $I$ \\
NGC 6362 V40 B & 4.99 $\pm$ 0.08 & 4.54 $\pm$ 0.07 & -0.139 $\pm$ 0.005 & 0.788 $\pm$ 0.029 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
NGC 6362 V40 A & 4.427 $\pm$ 0.028 & 3.972 $\pm$ 0.021 & -0.1394 $\pm$ 0.0018 & 0.789 $\pm$ 0.005 & SGB & 36 & 7706 $\pm$ 2786 & 13.0 $_{- 0.6}^{+ 0.8}$ & $I$ \\
NGC 6362 V40 B & 4.99 $\pm$ 0.08 & 4.54 $\pm$ 0.07 & -0.139 $\pm$ 0.005 & 0.788 $\pm$ 0.029 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
47 Tuc V69 A & 4.48 $\pm$ 0.09 & 3.99 $\pm$ 0.06 & -0.116 $\pm$ 0.008 & 0.862 $\pm$ 0.028 & MS & 56 & 4332 $\pm$ 913 & 11.3 $_{- 1.3}^{+ 0.9}$ & $I$ \\
47 Tuc V69 B & 4.76 $\pm$ 0.09 & 4.27 $\pm$ 0.06 & -0.118 $\pm$ 0.008 & 0.84 $\pm$ 0.03 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
47 Tuc V69 A & 4.45 $\pm$ 0.08 & 3.97 $\pm$ 0.06 & -0.113 $\pm$ 0.008 & 0.871 $\pm$ 0.029 & MS & 31 & 4340 $\pm$ 915 & 10.2 $_{- 0.7}^{+ 1.4}$ & $O$ \\
47 Tuc V69 B & 4.76 $\pm$ 0.09 & 4.27 $\pm$ 0.06 & -0.118 $\pm$ 0.008 & 0.84 $\pm$ 0.03 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
Kepler-35 A & 5.49 $\pm$ 0.15 & 4.82 $\pm$ 0.10 & -0.118 $\pm$ 0.015 & 0.90 $\pm$ 0.05 & MS & 100 & 1601 $\pm$ 236 & 13.0 $_{- 3}^{+ 0.8}$ & $I$ \\
Kepler-35 B & 6.75 $\pm$ 0.15 & 5.92 $\pm$ 0.10 & -0.239 $\pm$ 0.030 & 0.81 $\pm$ 0.04 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
KIC 6131659 A & 5.76 $\pm$ 0.06 & 5.12 $\pm$ 0.05 & -0.120 $\pm$ 0.010 & 0.88 $\pm$ 0.06 & MS & 100 & 319 $\pm$ 14 & 3.3 $_{- 2.0}^{+ 5}$ & $I$ \\
KIC 6131659 B & 8.29 $\pm$ 0.10 & 7.25 $\pm$ 0.07 & -0.56 $\pm$ 0.03 & 0.664 $\pm$ 0.018 & MS & 98 & $\shortparallel$ & $\shortparallel$ & $I$ \\
RW Lac A & 5.08 $\pm$ 0.11 & 4.43 $\pm$ 0.08 & -0.105 $\pm$ 0.011 & 0.92 $\pm$ 0.05 & MS & 100 & 187 $\pm$ 14 & 13.0 $_{- 2.7}^{+ 0.8}$ & $I$ \\
RW Lac B & 5.70 $\pm$ 0.16 & 5.01 $\pm$ 0.11 & -0.128 $\pm$ 0.018 & 0.89 $\pm$ 0.05 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
Kepler-453 A & 6.35 $\pm$ 0.13 & 5.57 $\pm$ 0.10 & -0.178 $\pm$ 0.023 & 0.90 $\pm$ 0.04 & MS & 99 & 408 $\pm$ 29 & 0.94 $_{- 0.15}^{+ 4}$ & $I$ \\
Kepler-453 B & 15.5 $\pm$ 0.3 & 13.9 $\pm$ 0.3 & -2.95 $\pm$ 0.23 & 0.1883 $\pm$ 0.0026 & MS & 97 & $\shortparallel$ & $\shortparallel$ & $I$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleIb:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    Binary & $M_B$       &  $M_V$         & $BC$        &    $M_m$          & $ES$  &  $Pr$    & $d_m$      &  $\tau$  & Grid \\
                 & ($mag$)     & ($mag$)        &  ($mag$)  &    ($M_{\sun}$)  &            &              & ($pc$)      & ($Gyr$)  &        \\
    \hline
Tyc 5227-1023-1 A & 4.11 $\pm$ 0.16 & 3.68 $\pm$ 0.12 & -0.094 $\pm$ 0.012 & 0.97 $\pm$ 0.06 & MS & 88 & 437 $\pm$ 42 & 7.3 $_{- 1.7}^{+ 1.8}$ & $I$ \\
Tyc 5227-1023-1 B & 5.18 $\pm$ 0.14 & 4.67 $\pm$ 0.10 & -0.117 $\pm$ 0.010 & 0.85 $\pm$ 0.05 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
Tyc 5227-1023-1 A & 4.43 $\pm$ 0.08 & 3.93 $\pm$ 0.06 & -0.121 $\pm$ 0.006 & 0.854 $\pm$ 0.020 & SGB & 12 & 431 $\pm$ 40 & 10.7 $_{- 0.7}^{+ 1.4}$ & $I$ \\
Tyc 5227-1023-1 B & 5.18 $\pm$ 0.14 & 4.67 $\pm$ 0.10 & -0.117 $\pm$ 0.010 & 0.85 $\pm$ 0.05 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
IM Vir A & 5.49 $\pm$ 0.13 & 4.8 $\pm$ 0.1 & -0.117 $\pm$ 0.016 & 0.95 $\pm$ 0.07 & MS & 100 & 97 $\pm$ 6 & 11.8 $_{- 5}^{+ 0.6}$ & $I$ \\
IM Vir B & 8.96 $\pm$ 0.28 & 7.73 $\pm$ 0.24 & -0.86 $\pm$ 0.11 & 0.694 $\pm$ 0.021 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V565 Lyr A & 5.57 $\pm$ 0.11 & 4.80 $\pm$ 0.09 & -0.134 $\pm$ 0.020 & 1.00 $\pm$ 0.04 & MS & 100 & 4007 $\pm$ 1160 & 7.6 $_{- 2.0}^{+ 2.1}$ & $I$ \\
V565 Lyr B & 6.05 $\pm$ 0.14 & 5.23 $\pm$ 0.11 & -0.174 $\pm$ 0.028 & 0.96 $\pm$ 0.05 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V530 Ori A & 5.33 $\pm$ 0.11 & 4.73 $\pm$ 0.08 & -0.087 $\pm$ 0.010 & 0.99 $\pm$ 0.05 & MS & 99 & 117 $\pm$ 6 & 3.0 $_{- 1.2}^{+ 2.9}$ & $I$ \\
V530 Ori B & 10.05 $\pm$ 0.20 & 8.70 $\pm$ 0.18 & -1.15 $\pm$ 0.09 & 0.586 $\pm$ 0.011 & MS & 96 & $\shortparallel$ & $\shortparallel$ & $I$ \\
KIC 7177553 A & 5.67 $\pm$ 0.14 & 4.99 $\pm$ 0.10 & -0.111 $\pm$ 0.017 & 0.95 $\pm$ 0.05 & MS & 99 & 252 $\pm$ 24 & 3.0 $_{- 1.7}^{+ 4}$ & $I$ \\
KIC 7177553 B & 5.71 $\pm$ 0.14 & 5.02 $\pm$ 0.11 & -0.117 $\pm$ 0.019 & 0.94 $\pm$ 0.06 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
Kepler-34 A & 5.01 $\pm$ 0.14 & 4.39 $\pm$ 0.10 & -0.087 $\pm$ 0.016 & 0.99 $\pm$ 0.07 & MS & 100 & 1399 $\pm$ 165 & 7.3 $_{- 2.2}^{+ 2.6}$ & $I$ \\
Kepler-34 B & 5.21 $\pm$ 0.14 & 4.56 $\pm$ 0.10 & -0.094 $\pm$ 0.017 & 0.98 $\pm$ 0.07 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V636 Cen A & 5.32 $\pm$ 0.09 & 4.70 $\pm$ 0.07 & -0.099 $\pm$ 0.011 & 0.92 $\pm$ 0.05 & MS & 100 & 72 $\pm$ 3 & 11.3 $_{- 2.6}^{+ 1.1}$ & $I$ \\
V636 Cen B & 6.62 $\pm$ 0.11 & 5.78 $\pm$ 0.08 & -0.230 $\pm$ 0.022 & 0.808 $\pm$ 0.017 & MS & 74 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V636 Cen A & 5.32 $\pm$ 0.09 & 4.70 $\pm$ 0.07 & -0.099 $\pm$ 0.011 & 0.92 $\pm$ 0.05 & MS & 100 & 73 $\pm$ 4 & 0.064 $_{- 0.010}^{+ 0.015}$ & $I$ \\
V636 Cen B & 7.01 $\pm$ 0.18 & 6.11 $\pm$ 0.14 & -0.34 $\pm$ 0.05 & 0.809 $\pm$ 0.012 & PMS & 26 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V568 Lyr A & 4.92 $\pm$ 0.09 & 4.18 $\pm$ 0.07 & -0.110 $\pm$ 0.014 & 1.08 $\pm$ 0.04 & MS & 74 & 3721 $\pm$ 904 & 8.8 $_{- 1.9}^{+ 0.8}$ & $I$ \\
V568 Lyr B & 7.43 $\pm$ 0.13 & 6.42 $\pm$ 0.10 & -0.41 $\pm$ 0.04 & 0.825 $\pm$ 0.029 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V568 Lyr A & 5.09 $\pm$ 0.08 & 4.31 $\pm$ 0.06 & -0.141 $\pm$ 0.013 & 1.013 $\pm$ 0.019 & SGB & 26 & 3661 $\pm$ 889 & 10.2 $_{- 0.7}^{+ 1.2}$ & $I$ \\
V568 Lyr B & 7.43 $\pm$ 0.13 & 6.42 $\pm$ 0.10 & -0.41 $\pm$ 0.04 & 0.825 $\pm$ 0.029 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V785 Cep A & 4.55 $\pm$ 0.10 & 3.93 $\pm$ 0.07 & -0.080 $\pm$ 0.009 & 1.03 $\pm$ 0.03 & MS & 73 & 1699 $\pm$ 173 & 8.4 $_{- 1.0}^{+ 0.8}$ & $I$ \\
V785 Cep B & 4.68 $\pm$ 0.10 & 4.05 $\pm$ 0.08 & -0.087 $\pm$ 0.011 & 1.01 $\pm$ 0.04 & MS & 86 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V785 Cep A & 4.55 $\pm$ 0.10 & 3.93 $\pm$ 0.07 & -0.080 $\pm$ 0.009 & 1.03 $\pm$ 0.03 & MS & 73 & 1708 $\pm$ 175 & 9.7 $_{- 0.5}^{+ 0.7}$ & $I$ \\
V785 Cep B & 4.84 $\pm$ 0.08 & 4.17 $\pm$ 0.06 & -0.111 $\pm$ 0.007 & 0.944 $\pm$ 0.022 & SGB & 14 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V785 Cep A & 4.69 $\pm$ 0.09 & 4.04 $\pm$ 0.07 & -0.102 $\pm$ 0.009 & 0.976 $\pm$ 0.025 & SGB & 27 & 1675 $\pm$ 170 & 9.7 $_{- 0.8}^{+ 0.8}$ & $I$ \\
V785 Cep B & 4.68 $\pm$ 0.10 & 4.05 $\pm$ 0.08 & -0.087 $\pm$ 0.011 & 1.01 $\pm$ 0.04 & MS & 86 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V785 Cep A & 4.69 $\pm$ 0.09 & 4.04 $\pm$ 0.07 & -0.102 $\pm$ 0.009 & 0.976 $\pm$ 0.025 & SGB & 27 & 1684 $\pm$ 172 & 10.7 $_{- 0.8}^{+ 0.8}$ & $I$ \\
V785 Cep B & 4.84 $\pm$ 0.08 & 4.17 $\pm$ 0.06 & -0.111 $\pm$ 0.007 & 0.944 $\pm$ 0.022 & SGB & 14 & $\shortparallel$ & $\shortparallel$ & $I$ \\
WOCS 12009 A & 5.03 $\pm$ 0.10 & 4.44 $\pm$ 0.07 & -0.066 $\pm$ 0.007 & 1.10 $\pm$ 0.04 & MS & 99 & 833 $\pm$ 62 & 1.7 $_{- 0.9}^{+ 1.8}$ & $I$ \\
WOCS 12009 B & 7.93 $\pm$ 0.24 & 6.88 $\pm$ 0.20 & -0.50 $\pm$ 0.07 & 0.743 $\pm$ 0.024 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
$\alpha$ Cen A & 5.03 $\pm$ 0.03 & 4.339 $\pm$ 0.025 & -0.088 $\pm$ 0.005 & 1.086 $\pm$ 0.021 & MS & 100 & 1.35 $\pm$ 0.03 & 5.7 $_{- 0.6}^{+ 0.9}$ & $I$ \\
$\alpha$ Cen B & 6.61 $\pm$ 0.09 & 5.73 $\pm$ 0.07 & -0.245 $\pm$ 0.021 & 0.90 $\pm$ 0.03 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
KX Cnc A & 5.25 $\pm$ 0.11 & 4.60 $\pm$ 0.08 & -0.085 $\pm$ 0.013 & 1.04 $\pm$ 0.06 & MS & 99 & 44.7 $\pm$ 2.8 & 4.2 $_{- 1.8}^{+ 1.9}$ & $I$ \\
KX Cnc B & 5.34 $\pm$ 0.11 & 4.68 $\pm$ 0.08 & -0.092 $\pm$ 0.014 & 1.02 $\pm$ 0.06 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
KIC 7037405 A & 1.70 $\pm$ 0.15 & 0.61 $\pm$ 0.11 & -0.55 $\pm$ 0.05 & 1.14 $\pm$ 0.17 & RGB & 76 & 1735 $\pm$ 92 & 5.4 $_{- 0.7}^{+ 1.6}$ & $O$ \\
KIC 7037405 B & 3.91 $\pm$ 0.15 & 3.37 $\pm$ 0.11 & -0.082 $\pm$ 0.015 & 1.07 $\pm$ 0.05 & SGB & 96 & $\shortparallel$ & $\shortparallel$ & $I$ \\
KIC 7037405 A & 1.54 $\pm$ 0.12 & 0.47 $\pm$ 0.08 & -0.49 $\pm$ 0.03 & 1.00 $\pm$ 0.17 & CHeB & 24 & 1785 $\pm$ 92 & 6.9 $_{- 0.9}^{+ 0.9}$ & $O$ \\
KIC 7037405 B & 3.91 $\pm$ 0.15 & 3.37 $\pm$ 0.11 & -0.082 $\pm$ 0.015 & 1.07 $\pm$ 0.05 & SGB & 96 & $\shortparallel$ & $\shortparallel$ & $I$ \\
EW Ori A & 4.85 $\pm$ 0.11 & 4.25 $\pm$ 0.08 & -0.065 $\pm$ 0.010 & 1.09 $\pm$ 0.06 & MS & 100 & 169 $\pm$ 11 & 4.2 $_{- 1.4}^{+ 1.6}$ & $I$ \\
EW Ori B & 5.18 $\pm$ 0.11 & 4.53 $\pm$ 0.08 & -0.084 $\pm$ 0.014 & 1.03 $\pm$ 0.06 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleIb:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    Binary & $M_B$       &  $M_V$         & $BC$        &    $M_m$          & $ES$  &  $Pr$    & $d_m$      &  $\tau$  & Grid \\
                 & ($mag$)     & ($mag$)        &  ($mag$)  &    ($M_{\sun}$)  &            &              & ($pc$)      & ($Gyr$)  &        \\
    \hline
KIC 9970396 A & 2.26 $\pm$ 0.12 & 1.35 $\pm$ 0.09 & -0.374 $\pm$ 0.028 & 1.17 $\pm$ 0.17 & RGB & 100 & 885 $\pm$ 40 & 3.8 $_{- 0.9}^{+ 2.4}$ & $O$ \\
KIC 9970396 B & 4.78 $\pm$ 0.13 & 4.28 $\pm$ 0.10 & -0.086 $\pm$ 0.012 & 0.98 $\pm$ 0.06 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
LV Her A & 4.37 $\pm$ 0.17 & 3.82 $\pm$ 0.12 & -0.053 $\pm$ 0.018 & 1.17 $\pm$ 0.10 & MS & 99 & 354 $\pm$ 37 & 3.7 $_{- 1.1}^{+ 2.1}$ & $I$ \\
LV Her B & 4.64 $\pm$ 0.17 & 4.04 $\pm$ 0.12 & -0.069 $\pm$ 0.019 & 1.10 $\pm$ 0.09 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
LL Aqr A & 4.55 $\pm$ 0.05 & 3.97 $\pm$ 0.03 & -0.062 $\pm$ 0.004 & 1.101 $\pm$ 0.026 & MS & 100 & 133 $\pm$ 4 & 5.7 $_{- 0.7}^{+ 0.7}$ & $I$ \\
LL Aqr B & 5.61 $\pm$ 0.07 & 4.91 $\pm$ 0.05 & -0.117 $\pm$ 0.009 & 0.945 $\pm$ 0.029 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V432 Aur A & 3.16 $\pm$ 0.08 & 2.66 $\pm$ 0.06 & -0.110 $\pm$ 0.009 & 1.161 $\pm$ 0.028 & SGB & 100 & 141 $\pm$ 6 & 3.8 $_{- 0.3}^{+ 0.4}$ & $I$ \\
V432 Aur B & 4.12 $\pm$ 0.08 & 3.74 $\pm$ 0.06 & -0.083 $\pm$ 0.005 & 1.04 $\pm$ 0.03 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
Kepler 1647 A & 3.74 $\pm$ 0.10 & 3.22 $\pm$ 0.07 & -0.062 $\pm$ 0.007 & 1.16 $\pm$ 0.03 & SGB & 78 & 791 $\pm$ 55 & 4.9 $_{- 0.6}^{+ 0.8}$ & $I$ \\
Kepler 1647 B & 5.58 $\pm$ 0.12 & 4.92 $\pm$ 0.09 & -0.112 $\pm$ 0.015 & 0.91 $\pm$ 0.05 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
Kepler 1647 A & 3.62 $\pm$ 0.06 & 3.14 $\pm$ 0.04 & -0.053 $\pm$ 0.003 & 1.285 $\pm$ 0.016 & MS & 22 & 795 $\pm$ 55 & 3.33 $_{- 0.27}^{+ 0.25}$ & $I$ \\
Kepler 1647 B & 5.58 $\pm$ 0.12 & 4.92 $\pm$ 0.09 & -0.112 $\pm$ 0.015 & 0.91 $\pm$ 0.05 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
UX Men A & 4.40 $\pm$ 0.11 & 3.85 $\pm$ 0.08 & -0.054 $\pm$ 0.010 & 1.15 $\pm$ 0.06 & MS & 100 & 101 $\pm$ 6 & 3.7 $_{- 0.8}^{+ 1.2}$ & $I$ \\
UX Men B & 4.56 $\pm$ 0.11 & 4.00 $\pm$ 0.08 & -0.057 $\pm$ 0.010 & 1.13 $\pm$ 0.06 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
WZ Oph A & 4.32 $\pm$ 0.10 & 3.80 $\pm$ 0.08 & -0.078 $\pm$ 0.009 & 1.02 $\pm$ 0.04 & MS & 98 & 159 $\pm$ 11 & 6.9 $_{- 0.9}^{+ 1.1}$ & $I$ \\
WZ Oph B & 4.33 $\pm$ 0.10 & 3.81 $\pm$ 0.07 & -0.081 $\pm$ 0.009 & 1.01 $\pm$ 0.04 & MS & 92 & $\shortparallel$ & $\shortparallel$ & $I$ \\
WOCS 40007 A & 4.26 $\pm$ 0.09 & 3.73 $\pm$ 0.06 & -0.055 $\pm$ 0.006 & 1.15 $\pm$ 0.04 & MS & 100 & 2253 $\pm$ 284 & 4.2 $_{- 0.9}^{+ 1.1}$ & $I$ \\
WOCS 40007 B & 5.11 $\pm$ 0.16 & 4.49 $\pm$ 0.12 & -0.082 $\pm$ 0.017 & 1.01 $\pm$ 0.06 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
EF Aqr A & 4.45 $\pm$ 0.10 & 3.89 $\pm$ 0.07 & -0.059 $\pm$ 0.009 & 1.12 $\pm$ 0.06 & MS & 100 & 168 $\pm$ 8 & 6.0 $_{- 1.3}^{+ 1.6}$ & $I$ \\
EF Aqr B & 6.16 $\pm$ 0.12 & 5.34 $\pm$ 0.09 & -0.191 $\pm$ 0.021 & 0.883 $\pm$ 0.023 & MS & 97 & $\shortparallel$ & $\shortparallel$ & $I$ \\
AI Phe A & 4.17 $\pm$ 0.13 & 3.31 $\pm$ 0.09 & -0.298 $\pm$ 0.029 & 1.09 $\pm$ 0.12 & RGB & 86 & 149 $\pm$ 14 & 4.7 $_{- 0.6}^{+ 1.0}$ & $I$ \\
AI Phe B & 3.78 $\pm$ 0.16 & 3.24 $\pm$ 0.11 & -0.070 $\pm$ 0.014 & 1.15 $\pm$ 0.05 & SGB & 79 & $\shortparallel$ & $\shortparallel$ & $I$ \\
AI Phe A & 4.17 $\pm$ 0.13 & 3.31 $\pm$ 0.09 & -0.298 $\pm$ 0.029 & 1.09 $\pm$ 0.12 & RGB & 86 & 149 $\pm$ 14 & 3.67 $_{-undef.}^{+ 0.18}$ & $I$ \\
AI Phe B & 3.60 $\pm$ 0.10 & 3.10 $\pm$ 0.07 & -0.051 $\pm$ 0.005 & 1.311 $\pm$ 0.027 & MS & 20 & $\shortparallel$ & $\shortparallel$ & $I$ \\
AI Phe A & 3.87 $\pm$ 0.11 & 3.07 $\pm$ 0.08 & -0.228 $\pm$ 0.021 & 1.32 $\pm$ 0.05 & SGB & 14 & 156 $\pm$ 15 & 3.85 $_{- 0.24}^{+ 0.30}$ & $I$ \\
AI Phe B & 3.78 $\pm$ 0.16 & 3.24 $\pm$ 0.11 & -0.070 $\pm$ 0.014 & 1.15 $\pm$ 0.05 & SGB & 79 & $\shortparallel$ & $\shortparallel$ & $I$ \\
AI Phe A & 3.87 $\pm$ 0.11 & 3.07 $\pm$ 0.08 & -0.228 $\pm$ 0.021 & 1.32 $\pm$ 0.05 & SGB & 14 & 155 $\pm$ 15 & 3.33 $_{- 0.20}^{+ 0.25}$ & $I$ \\
AI Phe B & 3.60 $\pm$ 0.10 & 3.10 $\pm$ 0.07 & -0.051 $\pm$ 0.005 & 1.311 $\pm$ 0.027 & MS & 20 & $\shortparallel$ & $\shortparallel$ & $I$ \\
VZ Hya A & 4.20 $\pm$ 0.14 & 3.74 $\pm$ 0.11 & -0.059 $\pm$ 0.012 & 1.13 $\pm$ 0.07 & MS & 100 & 138 $\pm$ 11 & 3.0 $_{- 1.0}^{+ 1.4}$ & $I$ \\
VZ Hya B & 4.73 $\pm$ 0.14 & 4.22 $\pm$ 0.10 & -0.071 $\pm$ 0.011 & 1.06 $\pm$ 0.07 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V505 Per A & 4.17 $\pm$ 0.06 & 3.72 $\pm$ 0.05 & -0.048 $\pm$ 0.003 & 1.190 $\pm$ 0.024 & MS & 100 & 58.1 $\pm$ 2.8 & 2.3 $_{- 0.4}^{+ 0.4}$ & $I$ \\
V505 Per B & 4.25 $\pm$ 0.06 & 3.80 $\pm$ 0.06 & -0.051 $\pm$ 0.003 & 1.170 $\pm$ 0.024 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V375 Cep A & 3.95 $\pm$ 0.05 & 3.41 $\pm$ 0.03 & -0.046 $\pm$ 0.005 & 1.282 $\pm$ 0.028 & MS & 72 & 1980 $\pm$ 283 & 3.17 $_{- 0.27}^{+ 0.5}$ & $I$ \\
V375 Cep B & 6.35 $\pm$ 0.12 & 5.52 $\pm$ 0.09 & -0.205 $\pm$ 0.023 & 0.87 $\pm$ 0.03 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V375 Cep A & 3.96 $\pm$ 0.05 & 3.42 $\pm$ 0.03 & -0.049 $\pm$ 0.003 & 1.206 $\pm$ 0.017 & SGB & 28 & 1978 $\pm$ 283 & 4.24 $_{- 0.28}^{+ 0.4}$ & $I$ \\
V375 Cep B & 6.35 $\pm$ 0.12 & 5.52 $\pm$ 0.09 & -0.205 $\pm$ 0.023 & 0.87 $\pm$ 0.03 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CO And A & 3.93 $\pm$ 0.13 & 3.37 $\pm$ 0.09 & -0.063 $\pm$ 0.012 & 1.16 $\pm$ 0.05 & SGB & 60 & 375 $\pm$ 36 & 4.7 $_{- 0.5}^{+ 0.9}$ & $I$ \\
CO And B & 3.95 $\pm$ 0.13 & 3.40 $\pm$ 0.09 & -0.061 $\pm$ 0.011 & 1.16 $\pm$ 0.05 & SGB & 56 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CO And A & 3.93 $\pm$ 0.13 & 3.37 $\pm$ 0.09 & -0.063 $\pm$ 0.012 & 1.16 $\pm$ 0.05 & SGB & 60 & 374 $\pm$ 35 & 3.85 $_{- 0.18}^{+ 1.0}$ & $I$ \\
CO And B & 3.86 $\pm$ 0.13 & 3.32 $\pm$ 0.08 & -0.05 $\pm$ 0.01 & 1.30 $\pm$ 0.04 & MS & 43 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CO And A & 3.84 $\pm$ 0.13 & 3.30 $\pm$ 0.09 & -0.048 $\pm$ 0.009 & 1.31 $\pm$ 0.04 & MS & 39 & 379 $\pm$ 36 & 3.85 $_{- 0.18}^{+ 0.5}$ & $I$ \\
CO And B & 3.95 $\pm$ 0.13 & 3.40 $\pm$ 0.09 & -0.061 $\pm$ 0.011 & 1.16 $\pm$ 0.05 & SGB & 56 & $\shortparallel$ & $\shortparallel$ & $I$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleIb:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    Binary & $M_B$       &  $M_V$         & $BC$        &    $M_m$          & $ES$  &  $Pr$    & $d_m$      &  $\tau$  & Grid \\
                 & ($mag$)     & ($mag$)        &  ($mag$)  &    ($M_{\sun}$)  &            &              & ($pc$)      & ($Gyr$)  &        \\
    \hline
CO And A & 3.84 $\pm$ 0.13 & 3.30 $\pm$ 0.09 & -0.048 $\pm$ 0.009 & 1.31 $\pm$ 0.04 & MS & 39 & 378 $\pm$ 36 & 3.3 $_{- 0.4}^{+ 0.3}$ & $I$ \\
CO And B & 3.86 $\pm$ 0.13 & 3.32 $\pm$ 0.08 & -0.05 $\pm$ 0.01 & 1.30 $\pm$ 0.04 & MS & 43 & $\shortparallel$ & $\shortparallel$ & $I$ \\
KIC 8430105 A & 2.10 $\pm$ 0.09 & 1.28 $\pm$ 0.07 & -0.317 $\pm$ 0.020 & 1.30 $\pm$ 0.14 & RGB & 98 & 627 $\pm$ 23 & 2.4 $_{- 0.5}^{+ 1.5}$ & $O$ \\
KIC 8430105 B & 6.04 $\pm$ 0.15 & 5.43 $\pm$ 0.13 & -0.142 $\pm$ 0.010 & 0.81 $\pm$ 0.03 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
NP Per A & 4.11 $\pm$ 0.09 & 3.63 $\pm$ 0.07 & -0.040 $\pm$ 0.009 & 1.24 $\pm$ 0.05 & MS & 100 & 268 $\pm$ 19 & 2.4 $_{- 0.8}^{+ 0.8}$ & $I$ \\
NP Per B & 7.2 $\pm$ 0.3 & 6.04 $\pm$ 0.27 & -0.66 $\pm$ 0.12 & 1.00 $\pm$ 0.08 & PMS & 100 & $\shortparallel$ & 0.0081 $_{- 0.0015}^{+ 0.0015}$ & $I$ \\
ASAS J052821+0338.5 A & 4.95 $\pm$ 0.13 & 4.12 $\pm$ 0.09 & -0.241 $\pm$ 0.025 & 0.95 $\pm$ 0.04 & SGB & 98 & 344 $\pm$ 29 & 12.1 $_{- 0.9}^{+ 0.9}$ & $I$ \\
ASAS J052821+0338.5 B & 5.93 $\pm$ 0.19 & 4.92 $\pm$ 0.15 & -0.48 $\pm$ 0.06 & 1.15 $\pm$ 0.11 & PMS & 100 & $\shortparallel$ & 0.0028 $_{- 0.0005}^{+ 0.0005}$ & $I$ \\
KIC 9540226 A & 1.51 $\pm$ 0.12 & 0.49 $\pm$ 0.08 & -0.433 $\pm$ 0.030 & 1.17 $\pm$ 0.26 & CHeB & 69 & 1579 $\pm$ 78 & 3.5 $_{- 1.2}^{+ 2.2}$ & $O$ \\
KIC 9540226 B & 5.08 $\pm$ 0.13 & 4.54 $\pm$ 0.09 & -0.083 $\pm$ 0.011 & 1.00 $\pm$ 0.06 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
KIC 9540226 A & 1.60 $\pm$ 0.14 & 0.58 $\pm$ 0.10 & -0.47 $\pm$ 0.04 & 1.38 $\pm$ 0.21 & RGB & 31 & 1550 $\pm$ 78 & 2.1 $_{- 0.4}^{+ 1.6}$ & $O$ \\
KIC 9540226 B & 5.08 $\pm$ 0.13 & 4.54 $\pm$ 0.09 & -0.083 $\pm$ 0.011 & 1.00 $\pm$ 0.06 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V1130 Tau A & 3.34 $\pm$ 0.07 & 2.94 $\pm$ 0.05 & -0.047 $\pm$ 0.009 & 1.30 $\pm$ 0.04 & MS & 70 & 67.1 $\pm$ 2.9 & 2.61 $_{- 0.22}^{+ 0.3}$ & $I$ \\
V1130 Tau B & 3.74 $\pm$ 0.07 & 3.33 $\pm$ 0.06 & -0.052 $\pm$ 0.009 & 1.21 $\pm$ 0.05 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V1130 Tau A & 3.39 $\pm$ 0.06 & 2.98 $\pm$ 0.05 & -0.056 $\pm$ 0.007 & 1.196 $\pm$ 0.028 & SGB & 30 & 66.8 $\pm$ 2.9 & 3.49 $_{- 0.17}^{+ 0.3}$ & $I$ \\
V1130 Tau B & 3.74 $\pm$ 0.07 & 3.33 $\pm$ 0.06 & -0.052 $\pm$ 0.009 & 1.21 $\pm$ 0.05 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
AD Boo A & 3.61 $\pm$ 0.12 & 3.17 $\pm$ 0.09 & -0.023 $\pm$ 0.015 & 1.37 $\pm$ 0.07 & MS & 98 & 197 $\pm$ 13 & 1.9 $_{- 0.5}^{+ 0.6}$ & $I$ \\
AD Boo B & 4.68 $\pm$ 0.13 & 4.10 $\pm$ 0.09 & -0.056 $\pm$ 0.012 & 1.14 $\pm$ 0.07 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
BK Peg A & 3.47 $\pm$ 0.08 & 2.96 $\pm$ 0.06 & -0.058 $\pm$ 0.007 & 1.23 $\pm$ 0.03 & SGB & 51 & 282 $\pm$ 14 & 3.85 $_{- 0.23}^{+ 0.5}$ & $I$ \\
BK Peg B & 4.05 $\pm$ 0.09 & 3.56 $\pm$ 0.06 & -0.056 $\pm$ 0.006 & 1.16 $\pm$ 0.05 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
BK Peg A & 3.41 $\pm$ 0.07 & 2.92 $\pm$ 0.05 & -0.052 $\pm$ 0.005 & 1.343 $\pm$ 0.023 & MS & 49 & 283 $\pm$ 14 & 3.17 $_{- 0.26}^{+ 0.22}$ & $I$ \\
BK Peg B & 4.05 $\pm$ 0.09 & 3.56 $\pm$ 0.06 & -0.056 $\pm$ 0.006 & 1.16 $\pm$ 0.05 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE-LMC-ECL15260 A & -0.12 $\pm$ 0.19 & -1.36 $\pm$ 0.14 & -0.73 $\pm$ 0.06 & 1.5 $\pm$ 0.4 & AGB & 73 & 44830 $\pm$ 9398 & 1.1 $_{- 0.3}^{+ 1.0}$ & $O$ \\
OGLE-LMC-ECL15260 B & 0.27 $\pm$ 0.18 & -0.72 $\pm$ 0.14 & -0.46 $\pm$ 0.04 & 1.7 $\pm$ 0.5 & AGB & 66 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE-LMC-ECL15260 A & -0.12 $\pm$ 0.19 & -1.36 $\pm$ 0.14 & -0.73 $\pm$ 0.06 & 1.5 $\pm$ 0.4 & AGB & 73 & 44933 $\pm$ 9425 & 1.6 $_{- 0.6}^{+ 0.7}$ & $O$ \\
OGLE-LMC-ECL15260 B & 0.33 $\pm$ 0.18 & -0.67 $\pm$ 0.14 & -0.48 $\pm$ 0.05 & 1.7 $\pm$ 0.4 & RGB & 25 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE-LMC-ECL15260 A & -0.03 $\pm$ 0.20 & -1.27 $\pm$ 0.14 & -0.77 $\pm$ 0.07 & 1.35 $\pm$ 0.24 & RGB & 27 & 43792 $\pm$ 9190 & 1.9 $_{- 0.4}^{+ 1.1}$ & $O$ \\
OGLE-LMC-ECL15260 B & 0.27 $\pm$ 0.18 & -0.72 $\pm$ 0.14 & -0.46 $\pm$ 0.04 & 1.7 $\pm$ 0.5 & AGB & 66 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE-LMC-ECL15260 A & -0.03 $\pm$ 0.20 & -1.27 $\pm$ 0.14 & -0.77 $\pm$ 0.07 & 1.35 $\pm$ 0.24 & RGB & 27 & 43890 $\pm$ 9216 & 1.9 $_{- 0.4}^{+ 0.8}$ & $O$ \\
OGLE-LMC-ECL15260 B & 0.33 $\pm$ 0.18 & -0.67 $\pm$ 0.14 & -0.48 $\pm$ 0.05 & 1.7 $\pm$ 0.4 & RGB & 25 & $\shortparallel$ & $\shortparallel$ & $O$ \\
BG Ind A & 2.94 $\pm$ 0.17 & 2.50 $\pm$ 0.12 & -0.045 $\pm$ 0.011 & 1.43 $\pm$ 0.05 & MS & 64 & 64 $\pm$ 8 & 2.61 $_{- 0.4}^{+ 0.26}$ & $I$ \\
BG Ind B & 3.47 $\pm$ 0.19 & 3.07 $\pm$ 0.15 & -0.044 $\pm$ 0.012 & 1.29 $\pm$ 0.07 & MS & 75 & $\shortparallel$ & $\shortparallel$ & $I$ \\
BG Ind A & 2.94 $\pm$ 0.17 & 2.50 $\pm$ 0.12 & -0.045 $\pm$ 0.011 & 1.43 $\pm$ 0.05 & MS & 64 & 65 $\pm$ 9 & 3.33 $_{- 0.16}^{+ 0.17}$ & $I$ \\
BG Ind B & 3.65 $\pm$ 0.17 & 3.20 $\pm$ 0.12 & -0.059 $\pm$ 0.010 & 1.16 $\pm$ 0.05 & SGB & 25 & $\shortparallel$ & $\shortparallel$ & $I$ \\
BG Ind A & 3.25 $\pm$ 0.20 & 2.73 $\pm$ 0.15 & -0.072 $\pm$ 0.018 & 1.26 $\pm$ 0.05 & SGB & 36 & 63 $\pm$ 8 & 3.33 $_{- 0.24}^{+ 0.4}$ & $I$ \\
BG Ind B & 3.47 $\pm$ 0.19 & 3.07 $\pm$ 0.15 & -0.044 $\pm$ 0.012 & 1.29 $\pm$ 0.07 & MS & 75 & $\shortparallel$ & $\shortparallel$ & $I$ \\
BG Ind A & 3.25 $\pm$ 0.20 & 2.73 $\pm$ 0.15 & -0.072 $\pm$ 0.018 & 1.26 $\pm$ 0.05 & SGB & 36 & 63 $\pm$ 8 & 3.67 $_{- 0.26}^{+ 0.4}$ & $I$ \\
BG Ind B & 3.65 $\pm$ 0.17 & 3.20 $\pm$ 0.12 & -0.059 $\pm$ 0.010 & 1.16 $\pm$ 0.05 & SGB & 25 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CD Tau A & 3.75 $\pm$ 0.07 & 3.20 $\pm$ 0.05 & -0.045 $\pm$ 0.008 & 1.34 $\pm$ 0.04 & MS & 57 & 66.7 $\pm$ 2.7 & 3.2 $_{- 0.3}^{+ 0.3}$ & $I$ \\
CD Tau B & 4.03 $\pm$ 0.07 & 3.49 $\pm$ 0.05 & -0.049 $\pm$ 0.010 & 1.24 $\pm$ 0.07 & MS & 84 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CD Tau A & 3.75 $\pm$ 0.07 & 3.20 $\pm$ 0.05 & -0.045 $\pm$ 0.008 & 1.34 $\pm$ 0.04 & MS & 57 & 66.7 $\pm$ 2.7 & 4.04 $_{- 0.19}^{+ 0.21}$ & $I$ \\
CD Tau B & 4.05 $\pm$ 0.08 & 3.50 $\pm$ 0.06 & -0.054 $\pm$ 0.008 & 1.18 $\pm$ 0.05 & SGB & 16 & $\shortparallel$ & $\shortparallel$ & $I$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleIb:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    Binary & $M_B$       &  $M_V$         & $BC$        &    $M_m$          & $ES$  &  $Pr$    & $d_m$      &  $\tau$  & Grid \\
                 & ($mag$)     & ($mag$)        &  ($mag$)  &    ($M_{\sun}$)  &            &              & ($pc$)      & ($Gyr$)  &        \\
    \hline
CD Tau A & 3.76 $\pm$ 0.06 & 3.22 $\pm$ 0.05 & -0.054 $\pm$ 0.008 & 1.21 $\pm$ 0.04 & SGB & 42 & 66.3 $\pm$ 2.7 & 3.85 $_{- 0.18}^{+ 1.0}$ & $I$ \\
CD Tau B & 4.03 $\pm$ 0.07 & 3.49 $\pm$ 0.05 & -0.049 $\pm$ 0.010 & 1.24 $\pm$ 0.07 & MS & 84 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CD Tau A & 3.76 $\pm$ 0.06 & 3.22 $\pm$ 0.05 & -0.054 $\pm$ 0.008 & 1.21 $\pm$ 0.04 & SGB & 42 & 66.3 $\pm$ 2.7 & 4.24 $_{- 0.20}^{+ 0.4}$ & $I$ \\
CD Tau B & 4.05 $\pm$ 0.08 & 3.50 $\pm$ 0.06 & -0.054 $\pm$ 0.008 & 1.18 $\pm$ 0.05 & SGB & 16 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V570 Per A & 3.50 $\pm$ 0.07 & 3.12 $\pm$ 0.06 & -0.019 $\pm$ 0.004 & 1.394 $\pm$ 0.021 & MS & 99 & 126 $\pm$ 6 & 1.38 $_{- 0.18}^{+ 0.19}$ & $I$ \\
V570 Per B & 3.95 $\pm$ 0.06 & 3.51 $\pm$ 0.05 & -0.033 $\pm$ 0.004 & 1.285 $\pm$ 0.022 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
BW Aqr A & 3.33 $\pm$ 0.11 & 2.83 $\pm$ 0.08 & -0.047 $\pm$ 0.008 & 1.38 $\pm$ 0.04 & MS & 64 & 380 $\pm$ 26 & 3.85 $_{- 0.3}^{+ 0.19}$ & $I$ \\
BW Aqr B & 3.76 $\pm$ 0.11 & 3.23 $\pm$ 0.09 & -0.059 $\pm$ 0.009 & 1.18 $\pm$ 0.05 & SGB & 59 & $\shortparallel$ & $\shortparallel$ & $I$ \\
BW Aqr A & 3.33 $\pm$ 0.11 & 2.83 $\pm$ 0.08 & -0.047 $\pm$ 0.008 & 1.38 $\pm$ 0.04 & MS & 64 & 379 $\pm$ 26 & 3.02 $_{- 0.26}^{+ 0.27}$ & $I$ \\
BW Aqr B & 3.69 $\pm$ 0.10 & 3.18 $\pm$ 0.08 & -0.049 $\pm$ 0.006 & 1.31 $\pm$ 0.03 & MS & 40 & $\shortparallel$ & $\shortparallel$ & $I$ \\
BW Aqr A & 3.39 $\pm$ 0.11 & 2.89 $\pm$ 0.08 & -0.056 $\pm$ 0.008 & 1.25 $\pm$ 0.04 & SGB & 35 & 377 $\pm$ 26 & 4.04 $_{- 0.28}^{+ 0.4}$ & $I$ \\
BW Aqr B & 3.76 $\pm$ 0.11 & 3.23 $\pm$ 0.09 & -0.059 $\pm$ 0.009 & 1.18 $\pm$ 0.05 & SGB & 59 & $\shortparallel$ & $\shortparallel$ & $I$ \\
BW Aqr A & 3.39 $\pm$ 0.11 & 2.89 $\pm$ 0.08 & -0.056 $\pm$ 0.008 & 1.25 $\pm$ 0.04 & SGB & 35 & 377 $\pm$ 26 & 3.49 $_{- 0.17}^{+ 0.24}$ & $I$ \\
BW Aqr B & 3.69 $\pm$ 0.10 & 3.18 $\pm$ 0.08 & -0.049 $\pm$ 0.006 & 1.31 $\pm$ 0.03 & MS & 40 & $\shortparallel$ & $\shortparallel$ & $I$ \\
GX Gem A & 3.13 $\pm$ 0.09 & 2.62 $\pm$ 0.06 & -0.051 $\pm$ 0.006 & 1.43 $\pm$ 0.03 & MS & 65 & 643 $\pm$ 42 & 2.87 $_{- 0.19}^{+ 0.15}$ & $I$ \\
GX Gem B & 3.23 $\pm$ 0.09 & 2.72 $\pm$ 0.06 & -0.052 $\pm$ 0.005 & 1.409 $\pm$ 0.028 & MS & 51 & $\shortparallel$ & $\shortparallel$ & $I$ \\
GX Gem A & 3.13 $\pm$ 0.09 & 2.62 $\pm$ 0.06 & -0.051 $\pm$ 0.006 & 1.43 $\pm$ 0.03 & MS & 65 & 645 $\pm$ 42 & 3.17 $_{- 0.15}^{+ 0.16}$ & $I$ \\
GX Gem B & 3.32 $\pm$ 0.10 & 2.79 $\pm$ 0.07 & -0.066 $\pm$ 0.010 & 1.27 $\pm$ 0.04 & SGB & 49 & $\shortparallel$ & $\shortparallel$ & $I$ \\
GX Gem A & 3.21 $\pm$ 0.10 & 2.69 $\pm$ 0.07 & -0.065 $\pm$ 0.010 & 1.30 $\pm$ 0.04 & SGB & 34 & 638 $\pm$ 42 & 3.17 $_{- 0.15}^{+ 0.16}$ & $I$ \\
GX Gem B & 3.23 $\pm$ 0.09 & 2.72 $\pm$ 0.06 & -0.052 $\pm$ 0.005 & 1.409 $\pm$ 0.028 & MS & 51 & $\shortparallel$ & $\shortparallel$ & $I$ \\
GX Gem A & 3.21 $\pm$ 0.10 & 2.69 $\pm$ 0.07 & -0.065 $\pm$ 0.010 & 1.30 $\pm$ 0.04 & SGB & 34 & 640 $\pm$ 42 & 3.49 $_{- 0.17}^{+ 0.23}$ & $I$ \\
GX Gem B & 3.32 $\pm$ 0.10 & 2.79 $\pm$ 0.07 & -0.066 $\pm$ 0.010 & 1.27 $\pm$ 0.04 & SGB & 49 & $\shortparallel$ & $\shortparallel$ & $I$ \\
HD 187669 A & 1.09 $\pm$ 0.14 & -0.14 $\pm$ 0.10 & -0.67 $\pm$ 0.04 & 1.03 $\pm$ 0.19 & AGB & 57 & 578 $\pm$ 35 & 5.7 $_{- 1.7}^{+ 2.9}$ & $O$ \\
HD 187669 B & 1.90 $\pm$ 0.13 & 0.89 $\pm$ 0.10 & -0.47 $\pm$ 0.03 & 1.17 $\pm$ 0.17 & RGB & 59 & $\shortparallel$ & $\shortparallel$ & $O$ \\
HD 187669 A & 1.09 $\pm$ 0.14 & -0.14 $\pm$ 0.10 & -0.67 $\pm$ 0.04 & 1.03 $\pm$ 0.19 & AGB & 57 & 575 $\pm$ 35 & 4.2 $_{- 0.9}^{+ 3}$ & $O$ \\
HD 187669 B & 1.77 $\pm$ 0.12 & 0.76 $\pm$ 0.09 & -0.411 $\pm$ 0.029 & 1.15 $\pm$ 0.17 & CHeB & 41 & $\shortparallel$ & $\shortparallel$ & $O$ \\
HD 187669 A & 1.16 $\pm$ 0.16 & -0.07 $\pm$ 0.12 & -0.70 $\pm$ 0.05 & 1.18 $\pm$ 0.20 & RGB & 42 & 567 $\pm$ 35 & 2.9 $_{- 0.4}^{+ 3}$ & $O$ \\
HD 187669 B & 1.90 $\pm$ 0.13 & 0.89 $\pm$ 0.10 & -0.47 $\pm$ 0.03 & 1.17 $\pm$ 0.17 & RGB & 59 & $\shortparallel$ & $\shortparallel$ & $O$ \\
HD 187669 A & 1.16 $\pm$ 0.16 & -0.07 $\pm$ 0.12 & -0.70 $\pm$ 0.05 & 1.18 $\pm$ 0.20 & RGB & 42 & 564 $\pm$ 35 & 3.8 $_{- 0.8}^{+ 2.6}$ & $O$ \\
HD 187669 B & 1.77 $\pm$ 0.12 & 0.76 $\pm$ 0.09 & -0.411 $\pm$ 0.029 & 1.15 $\pm$ 0.17 & CHeB & 41 & $\shortparallel$ & $\shortparallel$ & $O$ \\
KIC 11285625 A & 2.66 $\pm$ 0.08 & 2.34 $\pm$ 0.06 & -0.048 $\pm$ 0.009 & 1.36 $\pm$ 0.04 & MS & 77 & 415 $\pm$ 26 & 2.36 $_{- 0.21}^{+ 0.22}$ & $I$ \\
KIC 11285625 B & 3.34 $\pm$ 0.16 & 3.04 $\pm$ 0.13 & -0.058 $\pm$ 0.012 & 1.20 $\pm$ 0.08 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
KIC 11285625 A & 2.69 $\pm$ 0.08 & 2.38 $\pm$ 0.06 & -0.060 $\pm$ 0.008 & 1.23 $\pm$ 0.03 & SGB & 23 & 412 $\pm$ 25 & 3.02 $_{- 0.14}^{+ 0.23}$ & $I$ \\
KIC 11285625 B & 3.34 $\pm$ 0.16 & 3.04 $\pm$ 0.13 & -0.058 $\pm$ 0.012 & 1.20 $\pm$ 0.08 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
KIC 8410637 A & 1.88 $\pm$ 0.14 & 0.84 $\pm$ 0.10 & -0.42 $\pm$ 0.04 & 1.8 $\pm$ 0.4 & CHeB & 97 & 1175 $\pm$ 54 & 2.14 $_{- 0.7}^{+ 0.20}$ & $O$ \\
KIC 8410637 B & 3.77 $\pm$ 0.17 & 3.29 $\pm$ 0.13 & -0.021 $\pm$ 0.014 & 1.37 $\pm$ 0.06 & MS & 98 & $\shortparallel$ & $\shortparallel$ & $I$ \\
KIC 9777062 A & 2.53 $\pm$ 0.10 & 2.29 $\pm$ 0.08 & -0.001 $\pm$ 0.010 & 1.63 $\pm$ 0.07 & MS & 100 & 1013 $\pm$ 64 & 0.94 $_{- 0.22}^{+ 0.24}$ & $I$ \\
KIC 9777062 B & 3.21 $\pm$ 0.08 & 2.89 $\pm$ 0.06 & -0.013 $\pm$ 0.011 & 1.46 $\pm$ 0.06 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V501 Mon A & 2.48 $\pm$ 0.08 & 2.22 $\pm$ 0.07 & 0.003 $\pm$ 0.005 & 1.65 $\pm$ 0.04 & MS & 100 & 983 $\pm$ 78 & 1.14 $_{- 0.13}^{+ 0.12}$ & $I$ \\
V501 Mon B & 3.27 $\pm$ 0.09 & 2.92 $\pm$ 0.07 & -0.014 $\pm$ 0.007 & 1.44 $\pm$ 0.04 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CoRoT 102918586 A & 2.89 $\pm$ 0.07 & 2.60 $\pm$ 0.05 & 0.006 $\pm$ 0.005 & 1.60 $\pm$ 0.03 & MS & 99 & 976 $\pm$ 57 & 0.60 $_{- 0.12}^{+ 0.13}$ & $I$ \\
CoRoT 102918586 B & 3.36 $\pm$ 0.09 & 3.01 $\pm$ 0.07 & -0.005 $\pm$ 0.005 & 1.49 $\pm$ 0.04 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleIb:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    Binary & $M_B$       &  $M_V$         & $BC$        &    $M_m$          & $ES$  &  $Pr$    & $d_m$      &  $\tau$  & Grid \\
                 & ($mag$)     & ($mag$)        &  ($mag$)  &    ($M_{\sun}$)  &            &              & ($pc$)      & ($Gyr$)  &        \\
    \hline
OGLE SMC126.1 210 A & -0.64 $\pm$ 0.17 & -1.73 $\pm$ 0.13 & -0.58 $\pm$ 0.05 & 1.5 $\pm$ 0.4 & AGB & 72 & 59168 $\pm$ 12185 & 1.3 $_{- 0.3}^{+ 1.2}$ & $O$ \\
OGLE SMC126.1 210 B & -0.48 $\pm$ 0.16 & -1.55 $\pm$ 0.12 & -0.56 $\pm$ 0.05 & 1.4 $\pm$ 0.4 & AGB & 70 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE SMC126.1 210 A & -0.64 $\pm$ 0.17 & -1.73 $\pm$ 0.13 & -0.58 $\pm$ 0.05 & 1.5 $\pm$ 0.4 & AGB & 72 & 59432 $\pm$ 12241 & 1.68 $_{- 0.16}^{+ 1.0}$ & $O$ \\
OGLE SMC126.1 210 B & -0.41 $\pm$ 0.14 & -1.49 $\pm$ 0.11 & -0.58 $\pm$ 0.04 & 1.31 $\pm$ 0.21 & RGB & 30 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE SMC126.1 210 A & -0.56 $\pm$ 0.14 & -1.66 $\pm$ 0.11 & -0.61 $\pm$ 0.04 & 1.34 $\pm$ 0.20 & RGB & 28 & 58215 $\pm$ 11940 & 1.60 $_{- 0.13}^{+ 0.9}$ & $O$ \\
OGLE SMC126.1 210 B & -0.48 $\pm$ 0.16 & -1.55 $\pm$ 0.12 & -0.56 $\pm$ 0.05 & 1.4 $\pm$ 0.4 & AGB & 70 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE SMC126.1 210 A & -0.56 $\pm$ 0.14 & -1.66 $\pm$ 0.11 & -0.61 $\pm$ 0.04 & 1.34 $\pm$ 0.20 & RGB & 28 & 58472 $\pm$ 11994 & 1.52 $_{- 0.09}^{+ 0.8}$ & $O$ \\
OGLE SMC126.1 210 B & -0.41 $\pm$ 0.14 & -1.49 $\pm$ 0.11 & -0.58 $\pm$ 0.04 & 1.31 $\pm$ 0.21 & RGB & 30 & $\shortparallel$ & $\shortparallel$ & $O$ \\
HW CMa A & 2.64 $\pm$ 0.11 & 2.39 $\pm$ 0.08 & 0.020 $\pm$ 0.009 & 1.73 $\pm$ 0.05 & MS & 99 & 293 $\pm$ 24 & 0.15 $_{- 0.08}^{+ 0.19}$ & $I$ \\
HW CMa B & 2.76 $\pm$ 0.12 & 2.49 $\pm$ 0.09 & 0.019 $\pm$ 0.009 & 1.70 $\pm$ 0.06 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE-LMC-ECL03160 A & -0.27 $\pm$ 0.19 & -1.40 $\pm$ 0.14 & -0.59 $\pm$ 0.06 & 1.9 $\pm$ 0.5 & AGB & 71 & 46474 $\pm$ 10559 & 0.57 $_{- 0.12}^{+ 0.28}$ & $O$ \\
OGLE-LMC-ECL03160 B & 0.52 $\pm$ 0.21 & -0.34 $\pm$ 0.19 & -0.31 $\pm$ 0.03 & 2.4 $\pm$ 0.5 & CHeB & 43 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE-LMC-ECL03160 A & -0.27 $\pm$ 0.19 & -1.40 $\pm$ 0.14 & -0.59 $\pm$ 0.06 & 1.9 $\pm$ 0.5 & AGB & 71 & 46477 $\pm$ 10560 & 0.57 $_{- 0.12}^{+ 0.28}$ & $O$ \\
OGLE-LMC-ECL03160 B & 0.53 $\pm$ 0.20 & -0.33 $\pm$ 0.19 & -0.311 $\pm$ 0.030 & 2.4 $\pm$ 0.5 & CHeB & 37 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE-LMC-ECL03160 A & -0.17 $\pm$ 0.17 & -1.31 $\pm$ 0.12 & -0.63 $\pm$ 0.05 & 1.5 $\pm$ 0.4 & RGB & 27 & 45518 $\pm$ 10324 & 0.389 $_{- 0.029}^{+ 1.2}$ & $O$ \\
OGLE-LMC-ECL03160 B & 0.52 $\pm$ 0.21 & -0.34 $\pm$ 0.19 & -0.31 $\pm$ 0.03 & 2.4 $\pm$ 0.5 & CHeB & 43 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE-LMC-ECL03160 A & -0.17 $\pm$ 0.17 & -1.31 $\pm$ 0.12 & -0.63 $\pm$ 0.05 & 1.5 $\pm$ 0.4 & RGB & 27 & 45521 $\pm$ 10324 & 0.389 $_{- 0.030}^{+ 1.2}$ & $O$ \\
OGLE-LMC-ECL03160 B & 0.53 $\pm$ 0.20 & -0.33 $\pm$ 0.19 & -0.311 $\pm$ 0.030 & 2.4 $\pm$ 0.5 & CHeB & 37 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE SMC130.5 4296 A & -0.87 $\pm$ 0.17 & -1.93 $\pm$ 0.13 & -0.55 $\pm$ 0.05 & 1.8 $\pm$ 0.5 & AGB & 80 & 56339 $\pm$ 11111 & 0.57 $_{- 0.03}^{+ 0.5}$ & $O$ \\
OGLE SMC130.5 4296 B & -0.32 $\pm$ 0.13 & -1.18 $\pm$ 0.09 & -0.365 $\pm$ 0.029 & 1.9 $\pm$ 0.4 & AGB & 67 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE SMC130.5 4296 A & -0.87 $\pm$ 0.17 & -1.93 $\pm$ 0.13 & -0.55 $\pm$ 0.05 & 1.8 $\pm$ 0.5 & AGB & 80 & 56425 $\pm$ 11136 & 0.63 $_{- 0.14}^{+ 1.0}$ & $O$ \\
OGLE SMC130.5 4296 B & -0.27 $\pm$ 0.16 & -1.13 $\pm$ 0.12 & -0.38 $\pm$ 0.04 & 2.0 $\pm$ 0.5 & RGB & 17 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE SMC130.5 4296 A & -0.71 $\pm$ 0.14 & -1.80 $\pm$ 0.11 & -0.60 $\pm$ 0.04 & 1.37 $\pm$ 0.23 & RGB & 20 & 54720 $\pm$ 10755 & 1.60 $_{- 0.13}^{+ 0.24}$ & $O$ \\
OGLE SMC130.5 4296 B & -0.32 $\pm$ 0.13 & -1.18 $\pm$ 0.09 & -0.365 $\pm$ 0.029 & 1.9 $\pm$ 0.4 & AGB & 67 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE SMC130.5 4296 A & -0.71 $\pm$ 0.14 & -1.80 $\pm$ 0.11 & -0.60 $\pm$ 0.04 & 1.37 $\pm$ 0.23 & RGB & 20 & 54801 $\pm$ 10778 & 1.45 $_{- 0.07}^{+ 0.5}$ & $O$ \\
OGLE SMC130.5 4296 B & -0.27 $\pm$ 0.16 & -1.13 $\pm$ 0.12 & -0.38 $\pm$ 0.04 & 2.0 $\pm$ 0.5 & RGB & 17 & $\shortparallel$ & $\shortparallel$ & $O$ \\
RS Cha A & 1.83 $\pm$ 0.14 & 1.65 $\pm$ 0.11 & 0.012 $\pm$ 0.010 & 1.93 $\pm$ 0.06 & MS & 99 & 103 $\pm$ 10 & 0.81 $_{- 0.09}^{+ 0.09}$ & $I$ \\
RS Cha B & 1.88 $\pm$ 0.14 & 1.64 $\pm$ 0.11 & 0.024 $\pm$ 0.006 & 1.90 $\pm$ 0.06 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
RR Lyn A & 1.74 $\pm$ 0.08 & 1.49 $\pm$ 0.06 & 0.033 $\pm$ 0.011 & 1.97 $\pm$ 0.07 & MS & 100 & 71.7 $\pm$ 2.9 & 0.81 $_{- 0.07}^{+ 0.16}$ & $I$ \\
RR Lyn B & 3.28 $\pm$ 0.09 & 2.91 $\pm$ 0.08 & 0.007 $\pm$ 0.012 & 1.53 $\pm$ 0.06 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
EK Cep A & 2.02 $\pm$ 0.09 & 1.94 $\pm$ 0.07 & -0.085 $\pm$ 0.029 & 1.91 $\pm$ 0.05 & MS & 99 & 157 $\pm$ 10 & 0.078 $_{- 0.027}^{+ 0.08}$ & $I$ \\
EK Cep B & 4.89 $\pm$ 0.17 & 4.22 $\pm$ 0.13 & -0.097 $\pm$ 0.022 & 1.02 $\pm$ 0.05 & MS & 91 & $\shortparallel$ & $\shortparallel$ & $I$ \\
TZ For A & 2.08 $\pm$ 0.06 & 1.13 $\pm$ 0.04 & -0.326 $\pm$ 0.011 & 1.97 $\pm$ 0.06 & CHeB & 99 & 162 $\pm$ 6 & 1.32 $_{- 0.06}^{+ 0.10}$ & $I$ \\
TZ For B & 1.80 $\pm$ 0.08 & 1.33 $\pm$ 0.06 & -0.021 $\pm$ 0.004 & 1.92 $\pm$ 0.03 & MS & 96 & $\shortparallel$ & $\shortparallel$ & $I$ \\
KIC 9246715 A & 1.86 $\pm$ 0.09 & 0.99 $\pm$ 0.06 & -0.283 $\pm$ 0.017 & 1.96 $\pm$ 0.07 & CHeB & 70 & 552 $\pm$ 81 & 1.45 $_{- 0.29}^{+ 0.07}$ & $I$ \\
KIC 9246715 B & 1.88 $\pm$ 0.09 & 1.01 $\pm$ 0.06 & -0.284 $\pm$ 0.017 & 1.95 $\pm$ 0.07 & CHeB & 68 & $\shortparallel$ & $\shortparallel$ & $I$ \\
KIC 9246715 A & 1.86 $\pm$ 0.09 & 0.99 $\pm$ 0.06 & -0.283 $\pm$ 0.017 & 1.96 $\pm$ 0.07 & CHeB & 70 & 553 $\pm$ 81 & 1.45 $_{- 0.3}^{+ 0.07}$ & $I$ \\
KIC 9246715 B & 1.88 $\pm$ 0.09 & 1.01 $\pm$ 0.06 & -0.285 $\pm$ 0.017 & 1.95 $\pm$ 0.07 & CHeB & 14 & $\shortparallel$ & $\shortparallel$ & $O$ \\
KIC 9246715 A & 1.87 $\pm$ 0.08 & 0.99 $\pm$ 0.05 & -0.284 $\pm$ 0.015 & 1.97 $\pm$ 0.07 & CHeB & 14 & 552 $\pm$ 80 & 1.25 $_{- 0.16}^{+ 0.17}$ & $O$ \\
KIC 9246715 B & 1.88 $\pm$ 0.09 & 1.01 $\pm$ 0.06 & -0.284 $\pm$ 0.017 & 1.95 $\pm$ 0.07 & CHeB & 68 & $\shortparallel$ & $\shortparallel$ & $I$ \\
KIC 9246715 A & 1.87 $\pm$ 0.08 & 0.99 $\pm$ 0.05 & -0.284 $\pm$ 0.015 & 1.97 $\pm$ 0.07 & CHeB & 14 & 552 $\pm$ 80 & 1.38 $_{- 0.26}^{+ 0.10}$ & $O$ \\
KIC 9246715 B & 1.88 $\pm$ 0.09 & 1.01 $\pm$ 0.06 & -0.285 $\pm$ 0.017 & 1.95 $\pm$ 0.07 & CHeB & 14 & $\shortparallel$ & $\shortparallel$ & $O$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleIb:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    Binary & $M_B$       &  $M_V$         & $BC$        &    $M_m$          & $ES$  &  $Pr$    & $d_m$      &  $\tau$  & Grid \\
                 & ($mag$)     & ($mag$)        &  ($mag$)  &    ($M_{\sun}$)  &            &              & ($pc$)      & ($Gyr$)  &        \\
    \hline
V1229 Tau A & 1.36 $\pm$ 0.20 & 1.36 $\pm$ 0.16 & -0.25 $\pm$ 0.11 & 2.24 $\pm$ 0.16 & MS & 100 & 134 $\pm$ 19 & 0.25 $_{- 0.09}^{+ 0.15}$ & $I$ \\
V1229 Tau B & 3.18 $\pm$ 0.30 & 2.85 $\pm$ 0.23 & -0.008 $\pm$ 0.011 & 1.50 $\pm$ 0.10 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE LMC-ECL-25658 A & -0.13 $\pm$ 0.14 & -1.10 $\pm$ 0.10 & -0.45 $\pm$ 0.04 & 1.9 $\pm$ 0.4 & AGB & 66 & 45436 $\pm$ 9854 & 1.6 $_{- 0.3}^{+ 0.8}$ & $O$ \\
OGLE LMC-ECL-25658 B & 0.41 $\pm$ 0.12 & -0.55 $\pm$ 0.08 & -0.448 $\pm$ 0.030 & 1.26 $\pm$ 0.29 & AGB & 80 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE LMC-ECL-25658 A & -0.13 $\pm$ 0.14 & -1.10 $\pm$ 0.10 & -0.45 $\pm$ 0.04 & 1.9 $\pm$ 0.4 & AGB & 66 & 45608 $\pm$ 9896 & 1.4 $_{- 0.4}^{+ 0.7}$ & $O$ \\
OGLE LMC-ECL-25658 B & 0.49 $\pm$ 0.12 & -0.49 $\pm$ 0.09 & -0.47 $\pm$ 0.03 & 1.42 $\pm$ 0.23 & RGB & 19 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE LMC-ECL-25658 A & -0.26 $\pm$ 0.14 & -1.20 $\pm$ 0.10 & -0.41 $\pm$ 0.03 & 2.44 $\pm$ 0.29 & CHeB & 17 & 46435 $\pm$ 10069 & 1.03 $_{- 0.14}^{+ 0.10}$ & $O$ \\
OGLE LMC-ECL-25658 B & 0.41 $\pm$ 0.12 & -0.55 $\pm$ 0.08 & -0.448 $\pm$ 0.030 & 1.26 $\pm$ 0.29 & AGB & 80 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE LMC-ECL-25658 A & -0.26 $\pm$ 0.14 & -1.20 $\pm$ 0.10 & -0.41 $\pm$ 0.03 & 2.44 $\pm$ 0.29 & CHeB & 17 & 46615 $\pm$ 10113 & 0.94 $_{- 0.22}^{+ 0.11}$ & $O$ \\
OGLE LMC-ECL-25658 B & 0.49 $\pm$ 0.12 & -0.49 $\pm$ 0.09 & -0.47 $\pm$ 0.03 & 1.42 $\pm$ 0.23 & RGB & 19 & $\shortparallel$ & $\shortparallel$ & $O$ \\
SW CMa A & 0.94 $\pm$ 0.09 & 0.80 $\pm$ 0.07 & 0.023 $\pm$ 0.012 & 2.32 $\pm$ 0.05 & MS & 100 & 723 $\pm$ 49 & 0.60 $_{- 0.05}^{+ 0.05}$ & $I$ \\
SW CMa B & 1.44 $\pm$ 0.10 & 1.27 $\pm$ 0.08 & 0.026 $\pm$ 0.010 & 2.13 $\pm$ 0.05 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CoRoT 105906206 A & 1.31 $\pm$ 0.14 & 0.93 $\pm$ 0.10 & 0.003 $\pm$ 0.009 & 2.07 $\pm$ 0.05 & MS & 99 & 1109 $\pm$ 113 & 1.08 $_{- 0.10}^{+ 0.09}$ & $I$ \\
CoRoT 105906206 B & 4.46 $\pm$ 0.17 & 3.90 $\pm$ 0.12 & -0.061 $\pm$ 0.014 & 1.12 $\pm$ 0.07 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
YZ Cas A & 0.74 $\pm$ 0.04 & 0.736 $\pm$ 0.030 & -0.182 $\pm$ 0.022 & 2.42 $\pm$ 0.05 & MS & 100 & 96 $\pm$ 3 & 0.43 $_{- 0.05}^{+ 0.04}$ & $I$ \\
YZ Cas B & 3.99 $\pm$ 0.14 & 3.56 $\pm$ 0.10 & -0.026 $\pm$ 0.007 & 1.33 $\pm$ 0.05 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE SMC101.8 14077 A & -0.61 $\pm$ 0.13 & -1.35 $\pm$ 0.10 & -0.281 $\pm$ 0.024 & 2.72 $\pm$ 0.20 & CHeB & 82 & 59213 $\pm$ 13986 & 0.408 $_{- 0.022}^{+ 0.06}$ & $I$ \\
OGLE SMC101.8 14077 B & -0.60 $\pm$ 0.13 & -1.19 $\pm$ 0.10 & -0.178 $\pm$ 0.017 & 2.48 $\pm$ 0.15 & CHeB & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE SMC101.8 14077 A & -0.62 $\pm$ 0.13 & -1.35 $\pm$ 0.10 & -0.281 $\pm$ 0.023 & 2.73 $\pm$ 0.19 & CHeB & 30 & 59247 $\pm$ 13993 & 0.408 $_{- 0.019}^{+ 0.05}$ & $O$ \\
OGLE SMC101.8 14077 B & -0.60 $\pm$ 0.13 & -1.19 $\pm$ 0.10 & -0.178 $\pm$ 0.017 & 2.48 $\pm$ 0.15 & CHeB & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE-LMC-ECL09660 A & -0.91 $\pm$ 0.14 & -1.97 $\pm$ 0.11 & -0.50 $\pm$ 0.04 & 3.1 $\pm$ 0.3 & AGB & 46 & 44073 $\pm$ 7147 & 0.276 $_{- 0.014}^{+ 0.06}$ & $O$ \\
OGLE-LMC-ECL09660 B & -0.87 $\pm$ 0.12 & -1.60 $\pm$ 0.10 & -0.200 $\pm$ 0.017 & 3.15 $\pm$ 0.11 & CHeB & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE-LMC-ECL09660 A & -1.04 $\pm$ 0.15 & -2.07 $\pm$ 0.11 & -0.46 $\pm$ 0.04 & 3.7 $\pm$ 0.3 & CHeB & 28 & 45096 $\pm$ 7331 & 0.276 $_{- 0.013}^{+ 0.025}$ & $O$ \\
OGLE-LMC-ECL09660 B & -0.87 $\pm$ 0.12 & -1.60 $\pm$ 0.10 & -0.200 $\pm$ 0.017 & 3.15 $\pm$ 0.11 & CHeB & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE-LMC-ECL10567 A & -0.64 $\pm$ 0.19 & -1.61 $\pm$ 0.16 & -0.46 $\pm$ 0.04 & 1.9 $\pm$ 0.5 & AGB & 79 & 45515 $\pm$ 8933 & 0.35 $_{- 0.04}^{+ 0.10}$ & $O$ \\
OGLE-LMC-ECL10567 B & -0.62 $\pm$ 0.17 & -1.40 $\pm$ 0.15 & -0.296 $\pm$ 0.021 & 2.86 $\pm$ 0.25 & CHeB & 82 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE-LMC-ECL10567 A & -0.64 $\pm$ 0.19 & -1.61 $\pm$ 0.16 & -0.46 $\pm$ 0.04 & 1.9 $\pm$ 0.5 & AGB & 79 & 45514 $\pm$ 8933 & 0.35 $_{- 0.04}^{+ 0.10}$ & $O$ \\
OGLE-LMC-ECL10567 B & -0.61 $\pm$ 0.17 & -1.39 $\pm$ 0.15 & -0.296 $\pm$ 0.022 & 2.86 $\pm$ 0.25 & CHeB & 31 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE-LMC-ECL10567 A & -0.52 $\pm$ 0.19 & -1.51 $\pm$ 0.17 & -0.48 $\pm$ 0.04 & 1.6 $\pm$ 0.6 & RGB & 18 & 44794 $\pm$ 8781 & 0.30 $_{- 0.03}^{+ 0.06}$ & $O$ \\
OGLE-LMC-ECL10567 B & -0.62 $\pm$ 0.17 & -1.40 $\pm$ 0.15 & -0.296 $\pm$ 0.021 & 2.86 $\pm$ 0.25 & CHeB & 82 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE-LMC-ECL10567 A & -0.52 $\pm$ 0.19 & -1.51 $\pm$ 0.17 & -0.48 $\pm$ 0.04 & 1.6 $\pm$ 0.6 & RGB & 18 & 44793 $\pm$ 8781 & 0.30 $_{- 0.03}^{+ 0.06}$ & $O$ \\
OGLE-LMC-ECL10567 B & -0.61 $\pm$ 0.17 & -1.39 $\pm$ 0.15 & -0.296 $\pm$ 0.022 & 2.86 $\pm$ 0.25 & CHeB & 31 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE-LMC-ECL09114 A & -0.91 $\pm$ 0.13 & -1.70 $\pm$ 0.09 & -0.221 $\pm$ 0.022 & 3.39 $\pm$ 0.08 & CHeB & 100 & 47555 $\pm$ 9111 & 0.336 $_{- 0.016}^{+ 0.017}$ & $I$ \\
OGLE-LMC-ECL09114 B & -0.27 $\pm$ 0.14 & -1.0 $\pm$ 0.1 & -0.218 $\pm$ 0.018 & 2.87 $\pm$ 0.08 & CHeB & 89 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE-LMC-ECL09114 A & -0.91 $\pm$ 0.13 & -1.70 $\pm$ 0.09 & -0.221 $\pm$ 0.022 & 3.39 $\pm$ 0.08 & CHeB & 100 & 47550 $\pm$ 9110 & 0.336 $_{- 0.016}^{+ 0.017}$ & $I$ \\
OGLE-LMC-ECL09114 B & -0.27 $\pm$ 0.14 & -1.01 $\pm$ 0.09 & -0.218 $\pm$ 0.019 & 2.87 $\pm$ 0.08 & CHeB & 10 & $\shortparallel$ & $\shortparallel$ & $O$ \\
V906 Sco A & -0.77 $\pm$ 0.14 & -0.71 $\pm$ 0.12 & -0.34 $\pm$ 0.10 & 3.31 $\pm$ 0.17 & MS & 100 & 250 $\pm$ 45 & 0.263 $_{- 0.030}^{+ 0.04}$ & $I$ \\
V906 Sco B & -0.29 $\pm$ 0.13 & -0.23 $\pm$ 0.11 & -0.40 $\pm$ 0.10 & 3.09 $\pm$ 0.16 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE SMC113.3 4007 A & -1.30 $\pm$ 0.17 & -2.29 $\pm$ 0.12 & -0.46 $\pm$ 0.04 & 3.2 $\pm$ 0.4 & AGB & 37 & 54393 $\pm$ 8499 & 0.250 $_{- 0.023}^{+ 0.09}$ & $O$ \\
OGLE SMC113.3 4007 B & -1.17 $\pm$ 0.17 & -2.17 $\pm$ 0.12 & -0.46 $\pm$ 0.04 & 3.0 $\pm$ 0.4 & AGB & 44 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE SMC113.3 4007 A & -1.30 $\pm$ 0.17 & -2.29 $\pm$ 0.12 & -0.46 $\pm$ 0.04 & 3.2 $\pm$ 0.4 & AGB & 37 & 53810 $\pm$ 8362 & 0.227 $_{- 0.04}^{+ 0.015}$ & $O$ \\
OGLE SMC113.3 4007 B & -1.34 $\pm$ 0.17 & -2.31 $\pm$ 0.13 & -0.41 $\pm$ 0.04 & 3.9 $\pm$ 0.3 & CHeB & 32 & $\shortparallel$ & $\shortparallel$ & $O$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleIb:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    Binary & $M_B$       &  $M_V$         & $BC$        &    $M_m$          & $ES$  &  $Pr$    & $d_m$      &  $\tau$  & Grid \\
                 & ($mag$)     & ($mag$)        &  ($mag$)  &    ($M_{\sun}$)  &            &              & ($pc$)      & ($Gyr$)  &        \\
    \hline
OGLE SMC113.3 4007 A & -1.47 $\pm$ 0.17 & -2.44 $\pm$ 0.13 & -0.40 $\pm$ 0.04 & 4.0 $\pm$ 0.3 & CHeB & 36 & 56367 $\pm$ 8858 & 0.196 $_{- 0.009}^{+ 0.04}$ & $O$ \\
OGLE SMC113.3 4007 B & -1.17 $\pm$ 0.17 & -2.17 $\pm$ 0.12 & -0.46 $\pm$ 0.04 & 3.0 $\pm$ 0.4 & AGB & 44 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE SMC113.3 4007 A & -1.47 $\pm$ 0.17 & -2.44 $\pm$ 0.13 & -0.40 $\pm$ 0.04 & 4.0 $\pm$ 0.3 & CHeB & 36 & 55748 $\pm$ 8712 & 0.146 $_{- 0.007}^{+ 0.028}$ & $O$ \\
OGLE SMC113.3 4007 B & -1.34 $\pm$ 0.17 & -2.31 $\pm$ 0.13 & -0.41 $\pm$ 0.04 & 3.9 $\pm$ 0.3 & CHeB & 32 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE-LMC-ECL01866 A & -0.90 $\pm$ 0.18 & -1.98 $\pm$ 0.13 & -0.55 $\pm$ 0.05 & 2.3 $\pm$ 0.4 & AGB & 91 & 42956 $\pm$ 6793 & 0.30 $_{- 0.06}^{+ 0.04}$ & $O$ \\
OGLE-LMC-ECL01866 B & -1.21 $\pm$ 0.13 & -1.91 $\pm$ 0.11 & -0.217 $\pm$ 0.019 & 3.21 $\pm$ 0.14 & CHeB & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE-LMC-ECL26122 A & -0.94 $\pm$ 0.14 & -1.89 $\pm$ 0.10 & -0.301 $\pm$ 0.030 & 3.82 $\pm$ 0.11 & CHeB & 100 & 49288 $\pm$ 9139 & 0.263 $_{- 0.013}^{+ 0.013}$ & $I$ \\
OGLE-LMC-ECL26122 B & -0.21 $\pm$ 0.13 & -1.13 $\pm$ 0.09 & -0.301 $\pm$ 0.025 & 3.30 $\pm$ 0.11 & CHeB & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE-LMC-ECL06575 A & -1.13 $\pm$ 0.14 & -2.20 $\pm$ 0.11 & -0.50 $\pm$ 0.04 & 3.4 $\pm$ 0.3 & AGB & 41 & 66424 $\pm$ 12823 & 0.216 $_{- 0.026}^{+ 0.017}$ & $O$ \\
OGLE-LMC-ECL06575 B & -1.23 $\pm$ 0.14 & -2.16 $\pm$ 0.12 & -0.350 $\pm$ 0.030 & 3.87 $\pm$ 0.17 & CHeB & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE-LMC-ECL06575 A & -1.27 $\pm$ 0.15 & -2.31 $\pm$ 0.12 & -0.46 $\pm$ 0.04 & 4.0 $\pm$ 0.3 & CHeB & 31 & 68185 $\pm$ 13202 & 0.170 $_{- 0.011}^{+ 0.025}$ & $O$ \\
OGLE-LMC-ECL06575 B & -1.23 $\pm$ 0.14 & -2.16 $\pm$ 0.12 & -0.350 $\pm$ 0.030 & 3.87 $\pm$ 0.17 & CHeB & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
OGLE SMC108.1 14904 A & -2.35 $\pm$ 0.18 & -3.23 $\pm$ 0.13 & -0.35 $\pm$ 0.04 & 4.61 $\pm$ 0.14 & CHeB & 75 & 56275 $\pm$ 7015 & 0.115 $_{- 0.005}^{+ 0.013}$ & $O$ \\
OGLE SMC108.1 14904 B & -2.81 $\pm$ 0.14 & -3.39 $\pm$ 0.10 & -0.139 $\pm$ 0.021 & 4.40 $\pm$ 0.14 & CHeB & 83 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE SMC108.1 14904 A & -2.35 $\pm$ 0.18 & -3.23 $\pm$ 0.13 & -0.35 $\pm$ 0.04 & 4.61 $\pm$ 0.14 & CHeB & 75 & 56290 $\pm$ 7019 & 0.094 $_{- 0.004}^{+ 0.007}$ & $O$ \\
OGLE SMC108.1 14904 B & -2.81 $\pm$ 0.14 & -3.39 $\pm$ 0.11 & -0.140 $\pm$ 0.021 & 5.16 $\pm$ 0.15 & SGB & 17 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE SMC108.1 14904 A & -2.27 $\pm$ 0.17 & -3.16 $\pm$ 0.13 & -0.37 $\pm$ 0.04 & 5.1 $\pm$ 0.5 & RGB & 14 & 55517 $\pm$ 6897 & 0.127 $_{- 0.006}^{+ 0.007}$ & $O$ \\
OGLE SMC108.1 14904 B & -2.81 $\pm$ 0.14 & -3.39 $\pm$ 0.10 & -0.139 $\pm$ 0.021 & 4.40 $\pm$ 0.14 & CHeB & 83 & $\shortparallel$ & $\shortparallel$ & $O$ \\
OGLE SMC108.1 14904 A & -2.27 $\pm$ 0.17 & -3.16 $\pm$ 0.13 & -0.37 $\pm$ 0.04 & 5.1 $\pm$ 0.5 & RGB & 14 & 55532 $\pm$ 6902 & 0.086 $_{- 0.008}^{+ 0.004}$ & $O$ \\
OGLE SMC108.1 14904 B & -2.81 $\pm$ 0.14 & -3.39 $\pm$ 0.11 & -0.140 $\pm$ 0.021 & 5.16 $\pm$ 0.15 & SGB & 17 & $\shortparallel$ & $\shortparallel$ & $O$ \\
ASAS J180057-2333.8 A & -0.75 $\pm$ 0.19 & -2.15 $\pm$ 0.15 & -0.85 $\pm$ 0.07 & 3.2 $\pm$ 0.5 & AGB & 81 & 1878 $\pm$ 250 & 0.146 $_{- 0.007}^{+ 0.08}$ & $O$ \\
ASAS J180057-2333.8 B & -1.03 $\pm$ 0.18 & -2.22 $\pm$ 0.14 & -0.55 $\pm$ 0.06 & 4.3 $\pm$ 0.4 & CHeB & 87 & $\shortparallel$ & $\shortparallel$ & $I$ \\
ASAS J180057-2333.8 A & -0.75 $\pm$ 0.19 & -2.15 $\pm$ 0.15 & -0.85 $\pm$ 0.07 & 3.2 $\pm$ 0.5 & AGB & 81 & 1904 $\pm$ 255 & 0.206 $_{- 0.011}^{+ 0.09}$ & $O$ \\
ASAS J180057-2333.8 B & -0.80 $\pm$ 0.16 & -2.04 $\pm$ 0.12 & -0.63 $\pm$ 0.05 & 3.6 $\pm$ 0.3 & AGB & 34 & $\shortparallel$ & $\shortparallel$ & $O$ \\
ASAS J180057-2333.8 A & -0.96 $\pm$ 0.15 & -2.32 $\pm$ 0.11 & -0.76 $\pm$ 0.05 & 4.1 $\pm$ 0.3 & CHeB & 47 & 1978 $\pm$ 260 & 0.154 $_{- 0.025}^{+ 0.03}$ & $I$ \\
ASAS J180057-2333.8 B & -1.03 $\pm$ 0.18 & -2.22 $\pm$ 0.14 & -0.55 $\pm$ 0.06 & 4.3 $\pm$ 0.4 & CHeB & 87 & $\shortparallel$ & $\shortparallel$ & $I$ \\
ASAS J180057-2333.8 A & -0.96 $\pm$ 0.15 & -2.32 $\pm$ 0.11 & -0.76 $\pm$ 0.05 & 4.1 $\pm$ 0.3 & CHeB & 47 & 2006 $\pm$ 265 & 0.206 $_{- 0.018}^{+ 0.010}$ & $I$ \\
ASAS J180057-2333.8 B & -0.80 $\pm$ 0.16 & -2.04 $\pm$ 0.12 & -0.63 $\pm$ 0.05 & 3.6 $\pm$ 0.3 & AGB & 34 & $\shortparallel$ & $\shortparallel$ & $O$ \\
CV Vel A & -1.72 $\pm$ 0.06 & -1.54 $\pm$ 0.05 & -1.70 $\pm$ 0.07 & 5.77 $\pm$ 0.28 & MS & 100 & 560 $\pm$ 69 & 0.050 $_{- 0.007}^{+ 0.008}$ & $I$ \\
CV Vel B & -1.62 $\pm$ 0.06 & -1.44 $\pm$ 0.05 & -1.67 $\pm$ 0.07 & 5.61 $\pm$ 0.27 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V380 Cyg A & -5.119 $\pm$ 0.028 & -4.897 $\pm$ 0.027 & -2.150 $\pm$ 0.028 & 14.90 $\pm$ 0.27 & PMS & 69 & 664 $\pm$ 31 & 0.0122 $_{- 0.0006}^{+ 14}$ & $I$ \\
V380 Cyg B & -2.02 $\pm$ 0.11 & -1.80 $\pm$ 0.10 & -2.24 $\pm$ 0.13 & 8.0 $\pm$ 0.6 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V380 Cyg A & -5.06 $\pm$ 0.05 & -4.84 $\pm$ 0.05 & -2.11 $\pm$ 0.05 & 14.2 $\pm$ 0.5 & SGB & 36 & 677 $\pm$ 35 & 0.0134 $_{- 0.0006}^{+ 0.0012}$ & $O$ \\
V380 Cyg B & -2.02 $\pm$ 0.11 & -1.80 $\pm$ 0.10 & -2.24 $\pm$ 0.13 & 8.0 $\pm$ 0.6 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V453 Cyg A & -4.26 $\pm$ 0.04 & -4.00 $\pm$ 0.03 & -2.763 $\pm$ 0.030 & 15.0 $\pm$ 0.4 & MS & 100 & 1617 $\pm$ 100 & 0.0116 $_{- 0.0008}^{+ 0.0006}$ & $I$ \\
V453 Cyg B & -3.09 $\pm$ 0.05 & -2.84 $\pm$ 0.04 & -2.59 $\pm$ 0.04 & 10.6 $\pm$ 0.3 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V578 Mon A & -3.40 $\pm$ 0.04 & -3.13 $\pm$ 0.04 & -2.95 $\pm$ 0.04 & 13.7 $\pm$ 0.5 & MS & 97 & 1224 $\pm$ 78 & 0.0078 $_{- 0.0013}^{+ 0.0015}$ & $I$ \\
V578 Mon B & -2.54 $\pm$ 0.04 & -2.30 $\pm$ 0.04 & -2.61 $\pm$ 0.04 & 9.8 $\pm$ 0.4 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
\hline
  \end{tabular}
%}
 \end{table}
\end{landscape}



\begin{landscape}
 \begin{table}
  \caption{
Inferred stellar parameters of DEB stars in Sample II: absolute magnitudes in the B-band ($M_B$) and the V-band ($M_V$), bolometric correction ($BC$), mass ($M_m$), evolution stage ($ES$), probability $Pr$, distance ($d_m$), age ($\tau$), and grid used.}
%{\tiny
  \label{tab:sampleIIb}
  \begin{tabular}{cccccccccc}
    \hline
    Binary & $M_B$       &  $M_V$         & $BC$        &    $M_m$          & $ES$  &  $Pr$    & $d_m$      &  $\tau$  & Grid \\
                 & ($mag$)     & ($mag$)        &  ($mag$)  &    ($M_{\sun}$)  &            &              & ($pc$)      & ($Gyr$)  &        \\
    \hline
EPIC 203710387 A & 14.3 $\pm$ 0.8 & 12.8 $\pm$ 0.8 & -3.3 $\pm$ 0.6 & 0.22 $\pm$ 0.08 & PMS & 70 & 22 $\pm$ 8 & 1.94 $_{- 0.27}^{+ 0.26}$ & $I$ \\
EPIC 203710387 B & 12.97 $\pm$ 0.27 & 11.55 $\pm$ 0.29 & -2.37 $\pm$ 0.18 & 0.415 $\pm$ 0.013 & MS & 63 & $\shortparallel$ & $\shortparallel$ & $I$ \\
EPIC 203710387 A & 14.3 $\pm$ 0.8 & 12.8 $\pm$ 0.8 & -3.3 $\pm$ 0.6 & 0.22 $\pm$ 0.08 & PMS & 70 & 25 $\pm$ 12 & 0.034 $_{- 0.009}^{+ 0.018}$ & $I$ \\
EPIC 203710387 B & 14.0 $\pm$ 0.9 & 12.6 $\pm$ 0.8 & -3.0 $\pm$ 0.6 & 0.26 $\pm$ 0.10 & PMS & 37 & $\shortparallel$ & $\shortparallel$ & $I$ \\
EPIC 203710387 A & 12.75 $\pm$ 0.26 & 11.34 $\pm$ 0.27 & -2.32 $\pm$ 0.16 & 0.438 $\pm$ 0.015 & MS & 30 & 42 $\pm$ 11 & 13.0 $_{- 7}^{+ 0.8}$ & $I$ \\
EPIC 203710387 B & 12.97 $\pm$ 0.27 & 11.55 $\pm$ 0.29 & -2.37 $\pm$ 0.18 & 0.415 $\pm$ 0.013 & MS & 63 & $\shortparallel$ & $\shortparallel$ & $I$ \\
EPIC 203710387 A & 12.75 $\pm$ 0.26 & 11.34 $\pm$ 0.27 & -2.32 $\pm$ 0.16 & 0.438 $\pm$ 0.015 & MS & 30 & 50 $\pm$ 24 & 1.94 $_{- 0.3}^{+ 0.28}$ & $I$ \\
EPIC 203710387 B & 14.0 $\pm$ 0.9 & 12.6 $\pm$ 0.8 & -3.0 $\pm$ 0.6 & 0.26 $\pm$ 0.10 & PMS & 37 & $\shortparallel$ & $\shortparallel$ & $I$ \\
UScoCTIO 5 A & 11.43 $\pm$ 0.27 & 10.04 $\pm$ 0.28 & -2.41 $\pm$ 0.19 & 0.41 $\pm$ 0.07 & PMS & 100 & 163 $\pm$ 38 & 0.0116 $_{- 0.0026}^{+ 0.0029}$ & $I$ \\
UScoCTIO 5 B & 11.46 $\pm$ 0.27 & 10.06 $\pm$ 0.28 & -2.41 $\pm$ 0.19 & 0.41 $\pm$ 0.07 & PMS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
LSPM J1112+7626 A & 13.1 $\pm$ 0.3 & 11.6 $\pm$ 0.4 & -2.31 $\pm$ 0.25 & 0.385 $\pm$ 0.008 & MS & 84 & 50 $\pm$ 15 & 13.0 $_{- 7}^{+ 0.8}$ & $I$ \\
LSPM J1112+7626 B & 14.3 $\pm$ 0.4 & 12.8 $\pm$ 0.4 & -2.7 $\pm$ 0.3 & 0.283 $\pm$ 0.009 & MS & 94 & $\shortparallel$ & $\shortparallel$ & $I$ \\
LSPM J1112+7626 A & 13.2 $\pm$ 0.5 & 11.8 $\pm$ 0.5 & -2.4 $\pm$ 0.3 & 0.37 $\pm$ 0.06 & PMS & 16 & 48 $\pm$ 15 & 1.5 $_{- 0.5}^{+ 0.7}$ & $I$ \\
LSPM J1112+7626 B & 14.3 $\pm$ 0.4 & 12.8 $\pm$ 0.4 & -2.7 $\pm$ 0.3 & 0.283 $\pm$ 0.009 & MS & 94 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CU Cnc A & 12.6 $\pm$ 0.3 & 11.1 $\pm$ 0.3 & -2.15 $\pm$ 0.22 & 0.435 $\pm$ 0.007 & MS & 86 & 17 $\pm$ 5 & 13.0 $_{- 7}^{+ 0.8}$ & $I$ \\
CU Cnc B & 13.0 $\pm$ 0.3 & 11.6 $\pm$ 0.4 & -2.28 $\pm$ 0.24 & 0.389 $\pm$ 0.011 & MS & 85 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CU Cnc A & 12.6 $\pm$ 0.3 & 11.1 $\pm$ 0.3 & -2.15 $\pm$ 0.22 & 0.435 $\pm$ 0.007 & MS & 86 & 17 $\pm$ 5 & 2.0 $_{- 0.3}^{+ 0.4}$ & $I$ \\
CU Cnc B & 13.1 $\pm$ 0.4 & 11.6 $\pm$ 0.4 & -2.33 $\pm$ 0.29 & 0.38 $\pm$ 0.05 & PMS & 15 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CU Cnc A & 12.6 $\pm$ 0.5 & 11.2 $\pm$ 0.4 & -2.19 $\pm$ 0.29 & 0.42 $\pm$ 0.06 & PMS & 14 & 17 $\pm$ 5 & 1.94 $_{- 0.26}^{+ 0.30}$ & $I$ \\
CU Cnc B & 13.0 $\pm$ 0.3 & 11.6 $\pm$ 0.4 & -2.28 $\pm$ 0.24 & 0.389 $\pm$ 0.011 & MS & 85 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CU Cnc A & 12.6 $\pm$ 0.5 & 11.2 $\pm$ 0.4 & -2.19 $\pm$ 0.29 & 0.42 $\pm$ 0.06 & PMS & 14 & 17 $\pm$ 5 & 0.067 $_{- 0.018}^{+ 1.0}$ & $I$ \\
CU Cnc B & 13.1 $\pm$ 0.4 & 11.6 $\pm$ 0.4 & -2.33 $\pm$ 0.29 & 0.38 $\pm$ 0.05 & PMS & 15 & $\shortparallel$ & $\shortparallel$ & $I$ \\
MG1-2056316 A & 12.1 $\pm$ 0.4 & 10.7 $\pm$ 0.4 & -1.88 $\pm$ 0.24 & 0.447 $\pm$ 0.005 & MS & 87 & 168 $\pm$ 51 & 13.0 $_{- 7}^{+ 0.8}$ & $I$ \\
MG1-2056316 B & 12.9 $\pm$ 0.4 & 11.4 $\pm$ 0.4 & -2.13 $\pm$ 0.26 & 0.376 $\pm$ 0.006 & MS & 85 & $\shortparallel$ & $\shortparallel$ & $I$ \\
MG1-2056316 A & 12.1 $\pm$ 0.4 & 10.7 $\pm$ 0.4 & -1.88 $\pm$ 0.24 & 0.447 $\pm$ 0.005 & MS & 87 & 169 $\pm$ 52 & 2.0 $_{- 0.5}^{+ 0.4}$ & $I$ \\
MG1-2056316 B & 12.9 $\pm$ 0.4 & 11.5 $\pm$ 0.4 & -2.15 $\pm$ 0.28 & 0.379 $\pm$ 0.022 & PMS & 15 & $\shortparallel$ & $\shortparallel$ & $I$ \\
MG1-2056316 A & 12.1 $\pm$ 0.3 & 10.7 $\pm$ 0.3 & -1.89 $\pm$ 0.22 & 0.451 $\pm$ 0.022 & PMS & 13 & 167 $\pm$ 49 & 1.94 $_{- 0.26}^{+ 0.25}$ & $I$ \\
MG1-2056316 B & 12.9 $\pm$ 0.4 & 11.4 $\pm$ 0.4 & -2.13 $\pm$ 0.26 & 0.376 $\pm$ 0.006 & MS & 85 & $\shortparallel$ & $\shortparallel$ & $I$ \\
MG1-2056316 A & 12.1 $\pm$ 0.3 & 10.7 $\pm$ 0.3 & -1.89 $\pm$ 0.22 & 0.451 $\pm$ 0.022 & PMS & 13 & 167 $\pm$ 50 & 0.11 $_{- 0.04}^{+ 1.1}$ & $I$ \\
MG1-2056316 B & 12.9 $\pm$ 0.4 & 11.5 $\pm$ 0.4 & -2.15 $\pm$ 0.28 & 0.379 $\pm$ 0.022 & PMS & 15 & $\shortparallel$ & $\shortparallel$ & $I$ \\
MG1-78457 A & 11.86 $\pm$ 0.23 & 10.47 $\pm$ 0.24 & -1.98 $\pm$ 0.16 & 0.504 $\pm$ 0.011 & MS & 90 & 312 $\pm$ 104 & 13.0 $_{- 7}^{+ 0.8}$ & $I$ \\
MG1-78457 B & 12.22 $\pm$ 0.25 & 10.82 $\pm$ 0.26 & -2.08 $\pm$ 0.17 & 0.471 $\pm$ 0.012 & MS & 88 & $\shortparallel$ & $\shortparallel$ & $I$ \\
MG1-78457 A & 11.86 $\pm$ 0.23 & 10.47 $\pm$ 0.24 & -1.98 $\pm$ 0.16 & 0.504 $\pm$ 0.011 & MS & 90 & 313 $\pm$ 105 & 1.60 $_{- 0.26}^{+ 0.23}$ & $I$ \\
MG1-78457 B & 12.3 $\pm$ 0.3 & 10.8 $\pm$ 0.3 & -2.09 $\pm$ 0.19 & 0.46 $\pm$ 0.05 & PMS & 12 & $\shortparallel$ & $\shortparallel$ & $I$ \\
MG1-78457 A & 11.9 $\pm$ 0.3 & 10.5 $\pm$ 0.3 & -2.00 $\pm$ 0.19 & 0.48 $\pm$ 0.06 & PMS & 10 & 307 $\pm$ 104 & 1.68 $_{- 0.23}^{+ 0.15}$ & $I$ \\
MG1-78457 B & 12.22 $\pm$ 0.25 & 10.82 $\pm$ 0.26 & -2.08 $\pm$ 0.17 & 0.471 $\pm$ 0.012 & MS & 88 & $\shortparallel$ & $\shortparallel$ & $I$ \\
MG1-78457 A & 11.9 $\pm$ 0.3 & 10.5 $\pm$ 0.3 & -2.00 $\pm$ 0.19 & 0.48 $\pm$ 0.06 & PMS & 10 & 307 $\pm$ 105 & 0.064 $_{- 0.016}^{+ 0.5}$ & $I$ \\
MG1-78457 B & 12.3 $\pm$ 0.3 & 10.8 $\pm$ 0.3 & -2.09 $\pm$ 0.19 & 0.46 $\pm$ 0.05 & PMS & 12 & $\shortparallel$ & $\shortparallel$ & $I$ \\
MG1-116309 A & 10.33 $\pm$ 0.25 & 8.96 $\pm$ 0.23 & -1.21 $\pm$ 0.12 & 0.556 $\pm$ 0.014 & MS & 89 & 337 $\pm$ 68 & 1.45 $_{- 0.24}^{+ 7}$ & $I$ \\
MG1-116309 B & 10.69 $\pm$ 0.25 & 9.29 $\pm$ 0.24 & -1.33 $\pm$ 0.14 & 0.535 $\pm$ 0.010 & MS & 90 & $\shortparallel$ & $\shortparallel$ & $I$ \\
    \hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleIIb:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    Binary & $M_B$       &  $M_V$         & $BC$        &    $M_m$          & $ES$  &  $Pr$    & $d_m$      &  $\tau$  & Grid \\
                 & ($mag$)     & ($mag$)        &  ($mag$)  &    ($M_{\sun}$)  &            &              & ($pc$)      & ($Gyr$)  &        \\
    \hline
MG1-116309 A & 10.33 $\pm$ 0.25 & 8.96 $\pm$ 0.23 & -1.21 $\pm$ 0.12 & 0.556 $\pm$ 0.014 & MS & 89 & 337 $\pm$ 68 & 1.08 $_{- 0.08}^{+ 0.11}$ & $I$ \\
MG1-116309 B & 10.66 $\pm$ 0.25 & 9.27 $\pm$ 0.24 & -1.33 $\pm$ 0.14 & 0.550 $\pm$ 0.012 & PMS & 10 & $\shortparallel$ & $\shortparallel$ & $I$ \\
MG1-116309 A & 10.32 $\pm$ 0.25 & 8.95 $\pm$ 0.23 & -1.21 $\pm$ 0.12 & 0.574 $\pm$ 0.015 & PMS & 11 & 337 $\pm$ 68 & 1.08 $_{- 0.08}^{+ 0.12}$ & $I$ \\
MG1-116309 B & 10.69 $\pm$ 0.25 & 9.29 $\pm$ 0.24 & -1.33 $\pm$ 0.14 & 0.535 $\pm$ 0.010 & MS & 90 & $\shortparallel$ & $\shortparallel$ & $I$ \\
MG1-116309 A & 10.32 $\pm$ 0.25 & 8.95 $\pm$ 0.23 & -1.21 $\pm$ 0.12 & 0.574 $\pm$ 0.015 & PMS & 11 & 337 $\pm$ 69 & 0.15 $_{- 0.03}^{+ 0.6}$ & $I$ \\
MG1-116309 B & 10.66 $\pm$ 0.25 & 9.27 $\pm$ 0.24 & -1.33 $\pm$ 0.14 & 0.550 $\pm$ 0.012 & PMS & 10 & $\shortparallel$ & $\shortparallel$ & $I$ \\
MG1-506664 A & 10.73 $\pm$ 0.26 & 9.34 $\pm$ 0.27 & -1.44 $\pm$ 0.16 & 0.559 $\pm$ 0.009 & MS & 92 & 262 $\pm$ 57 & 3.2 $_{- 1.3}^{+ 6}$ & $I$ \\
MG1-506664 B & 11.25 $\pm$ 0.27 & 9.85 $\pm$ 0.28 & -1.61 $\pm$ 0.17 & 0.516 $\pm$ 0.008 & MS & 91 & $\shortparallel$ & $\shortparallel$ & $I$ \\
GU Boo A & 9.98 $\pm$ 0.29 & 8.64 $\pm$ 0.27 & -1.21 $\pm$ 0.14 & 0.622 $\pm$ 0.020 & MS & 95 & 139 $\pm$ 27 & 13.0 $_{- 8}^{+ 0.8}$ & $I$ \\
GU Boo B & 10.2 $\pm$ 0.3 & 8.86 $\pm$ 0.30 & -1.31 $\pm$ 0.16 & 0.612 $\pm$ 0.021 & MS & 95 & $\shortparallel$ & $\shortparallel$ & $I$ \\
ASAS J082552-1622.8 A & 8.7 $\pm$ 0.3 & 7.47 $\pm$ 0.28 & -0.76 $\pm$ 0.13 & 0.712 $\pm$ 0.022 & MS & 99 & 77 $\pm$ 17 & 13.0 $_{- 4}^{+ 0.8}$ & $I$ \\
ASAS J082552-1622.8 B & 8.8 $\pm$ 0.3 & 7.61 $\pm$ 0.29 & -0.82 $\pm$ 0.14 & 0.705 $\pm$ 0.021 & MS & 98 & $\shortparallel$ & $\shortparallel$ & $I$ \\
1SWASP J093010.78+533859.5 A & 7.23 $\pm$ 0.26 & 6.30 $\pm$ 0.19 & -0.34 $\pm$ 0.07 & 0.80 $\pm$ 0.03 & MS & 100 & 62 $\pm$ 9 & 13.0 $_{- 6}^{+ 0.8}$ & $I$ \\
1SWASP J093010.78+533859.5 B & 7.88 $\pm$ 0.23 & 6.80 $\pm$ 0.18 & -0.52 $\pm$ 0.07 & 0.769 $\pm$ 0.026 & MS & 89 & $\shortparallel$ & $\shortparallel$ & $I$ \\
1SWASP J093010.78+533859.5 A & 7.23 $\pm$ 0.26 & 6.30 $\pm$ 0.19 & -0.34 $\pm$ 0.07 & 0.80 $\pm$ 0.03 & MS & 100 & 67 $\pm$ 13 & 0.094 $_{- 0.009}^{+ 0.009}$ & $I$ \\
1SWASP J093010.78+533859.5 B & 8.9 $\pm$ 0.5 & 7.7 $\pm$ 0.4 & -0.92 $\pm$ 0.20 & 0.71 $\pm$ 0.04 & PMS & 11 & $\shortparallel$ & $\shortparallel$ & $I$ \\
ASAS J212954-5620.1 A & 6.96 $\pm$ 0.16 & 6.01 $\pm$ 0.13 & -0.32 $\pm$ 0.04 & 0.846 $\pm$ 0.027 & MS & 96 & 169 $\pm$ 23 & 13.0 $_{- 3.0}^{+ 0.8}$ & $I$ \\
ASAS J212954-5620.1 B & 8.6 $\pm$ 0.4 & 7.4 $\pm$ 0.3 & -0.72 $\pm$ 0.13 & 0.720 $\pm$ 0.025 & MS & 98 & $\shortparallel$ & $\shortparallel$ & $I$ \\
ASAS J045304-0700.4 A & 6.45 $\pm$ 0.22 & 5.63 $\pm$ 0.16 & -0.21 $\pm$ 0.04 & 0.87 $\pm$ 0.05 & MS & 100 & 172 $\pm$ 25 & 9.7 $_{- 6}^{+ 2.3}$ & $I$ \\
ASAS J045304-0700.4 B & 6.69 $\pm$ 0.22 & 5.82 $\pm$ 0.16 & -0.25 $\pm$ 0.05 & 0.86 $\pm$ 0.04 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
HS Aur A & 6.06 $\pm$ 0.12 & 5.23 $\pm$ 0.09 & -0.186 $\pm$ 0.019 & 0.915 $\pm$ 0.029 & MS & 100 & 122 $\pm$ 8 & 13.0 $_{- 3.0}^{+ 0.8}$ & $I$ \\
HS Aur B & 6.62 $\pm$ 0.13 & 5.74 $\pm$ 0.11 & -0.244 $\pm$ 0.025 & 0.87 $\pm$ 0.04 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CG Cyg A & 6.33 $\pm$ 0.20 & 5.51 $\pm$ 0.15 & -0.20 $\pm$ 0.04 & 0.89 $\pm$ 0.05 & MS & 100 & 101 $\pm$ 11 & 0.0432 $_{- 0.0021}^{+ 0.05}$ & $I$ \\
CG Cyg B & 7.54 $\pm$ 0.14 & 6.50 $\pm$ 0.11 & -0.50 $\pm$ 0.04 & 0.828 $\pm$ 0.026 & PMS & 76 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CG Cyg A & 6.33 $\pm$ 0.20 & 5.51 $\pm$ 0.15 & -0.20 $\pm$ 0.04 & 0.89 $\pm$ 0.05 & MS & 100 & 100 $\pm$ 11 & 13.0 $_{- 1.9}^{+ 0.8}$ & $I$ \\
CG Cyg B & 7.34 $\pm$ 0.11 & 6.31 $\pm$ 0.09 & -0.404 $\pm$ 0.025 & 0.816 $\pm$ 0.012 & MS & 24 & $\shortparallel$ & $\shortparallel$ & $I$ \\
HP Aur A & 5.43 $\pm$ 0.14 & 4.76 $\pm$ 0.10 & -0.102 $\pm$ 0.017 & 0.98 $\pm$ 0.07 & MS & 100 & 206 $\pm$ 15 & 4.5 $_{- 2.6}^{+ 4}$ & $I$ \\
HP Aur B & 6.94 $\pm$ 0.18 & 6.06 $\pm$ 0.13 & -0.28 $\pm$ 0.04 & 0.82 $\pm$ 0.04 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V1174 Ori A & 7.08 $\pm$ 0.26 & 5.93 $\pm$ 0.21 & -0.69 $\pm$ 0.10 & 0.98 $\pm$ 0.10 & PMS & 100 & 444 $\pm$ 69 & 0.0065 $_{- 0.0010}^{+ 0.0013}$ & $I$ \\
V1174 Ori B & 9.79 $\pm$ 0.28 & 8.42 $\pm$ 0.30 & -1.73 $\pm$ 0.20 & 0.62 $\pm$ 0.07 & PMS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CV Boo A & 5.00 $\pm$ 0.16 & 4.32 $\pm$ 0.12 & -0.101 $\pm$ 0.020 & 1.00 $\pm$ 0.07 & MS & 99 & 250 $\pm$ 25 & 10.2 $_{- 2.7}^{+ 1.9}$ & $I$ \\
CV Boo B & 5.24 $\pm$ 0.16 & 4.54 $\pm$ 0.12 & -0.110 $\pm$ 0.020 & 0.98 $\pm$ 0.06 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V1094 Tau A & 4.65 $\pm$ 0.11 & 4.00 $\pm$ 0.07 & -0.085 $\pm$ 0.012 & 1.07 $\pm$ 0.07 & MS & 74 & 119 $\pm$ 7 & 8.4 $_{- 1.9}^{+ 1.0}$ & $I$ \\
V1094 Tau B & 5.37 $\pm$ 0.12 & 4.67 $\pm$ 0.09 & -0.112 $\pm$ 0.016 & 0.97 $\pm$ 0.06 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V1094 Tau A & 4.74 $\pm$ 0.10 & 4.09 $\pm$ 0.07 & -0.110 $\pm$ 0.009 & 0.95 $\pm$ 0.04 & SGB & 25 & 117 $\pm$ 7 & 10.2 $_{- 0.6}^{+ 1.4}$ & $I$ \\
V1094 Tau B & 5.37 $\pm$ 0.12 & 4.67 $\pm$ 0.09 & -0.112 $\pm$ 0.016 & 0.97 $\pm$ 0.06 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
HP Dra A & 4.56 $\pm$ 0.16 & 3.95 $\pm$ 0.11 & -0.072 $\pm$ 0.017 & 1.09 $\pm$ 0.08 & MS & 94 & 76 $\pm$ 6 & 5.7 $_{- 1.9}^{+ 2.4}$ & $I$ \\
HP Dra B & 5.29 $\pm$ 0.16 & 4.65 $\pm$ 0.12 & -0.093 $\pm$ 0.018 & 1.00 $\pm$ 0.08 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
ZZ UMa A & 4.40 $\pm$ 0.08 & 3.79 $\pm$ 0.06 & -0.084 $\pm$ 0.012 & 1.04 $\pm$ 0.06 & SGB & 53 & 237 $\pm$ 11 & 9.7 $_{- 1.3}^{+ 1.4}$ & $I$ \\
ZZ UMa B & 5.67 $\pm$ 0.08 & 4.85 $\pm$ 0.06 & -0.173 $\pm$ 0.014 & 0.950 $\pm$ 0.017 & MS & 83 & $\shortparallel$ & 9.7 $_{- 1.3}^{+ 1.4}$ & $I$ \\
ZZ UMa A & 4.40 $\pm$ 0.08 & 3.79 $\pm$ 0.06 & -0.084 $\pm$ 0.012 & 1.04 $\pm$ 0.06 & SGB & 53 & 239 $\pm$ 11 & 7.8 $_{- 1.2}^{+ 1.2}$ & $I$ \\
ZZ UMa B & 5.88 $\pm$ 0.13 & 5.04 $\pm$ 0.10 & -0.227 $\pm$ 0.028 & 1.092 $\pm$ 0.026 & PMS & 11 & $\shortparallel$ & 0.0168 $_{- 0.0027}^{+ 0.0027}$ & $I$ \\
    \hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleIIb:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    Binary & $M_B$       &  $M_V$         & $BC$        &    $M_m$          & $ES$  &  $Pr$    & $d_m$      &  $\tau$  & Grid \\
                 & ($mag$)     & ($mag$)        &  ($mag$)  &    ($M_{\sun}$)  &            &              & ($pc$)      & ($Gyr$)  &        \\
    \hline
ZZ UMa A & 4.38 $\pm$ 0.09 & 3.75 $\pm$ 0.06 & -0.067 $\pm$ 0.008 & 1.16 $\pm$ 0.07 & MS & 47 & 239 $\pm$ 11 & 7.3 $_{- 0.7}^{+ 0.6}$ & $I$ \\
ZZ UMa B & 5.67 $\pm$ 0.08 & 4.85 $\pm$ 0.06 & -0.173 $\pm$ 0.014 & 0.950 $\pm$ 0.017 & MS & 83 & $\shortparallel$ & 7.3 $_{- 0.7}^{+ 0.6}$ & $I$ \\
ZZ UMa A & 4.38 $\pm$ 0.09 & 3.75 $\pm$ 0.06 & -0.067 $\pm$ 0.008 & 1.16 $\pm$ 0.07 & MS & 47 & 241 $\pm$ 11 & 5.5 $_{- 1.2}^{+ 1.2}$ & $I$ \\
ZZ UMa B & 5.88 $\pm$ 0.13 & 5.04 $\pm$ 0.10 & -0.227 $\pm$ 0.028 & 1.092 $\pm$ 0.026 & PMS & 11 & $\shortparallel$ & 0.0168 $_{- 0.0027}^{+ 0.0027}$ & $I$ \\
V2080 Cyg A & 4.24 $\pm$ 0.08 & 3.64 $\pm$ 0.06 & -0.074 $\pm$ 0.013 & 1.10 $\pm$ 0.06 & SGB & 76 & 78 $\pm$ 4 & 6.3 $_{- 0.9}^{+ 1.0}$ & $I$ \\
V2080 Cyg B & 4.25 $\pm$ 0.08 & 3.64 $\pm$ 0.06 & -0.075 $\pm$ 0.013 & 1.10 $\pm$ 0.06 & SGB & 78 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V2080 Cyg A & 4.24 $\pm$ 0.08 & 3.64 $\pm$ 0.06 & -0.074 $\pm$ 0.013 & 1.10 $\pm$ 0.06 & SGB & 76 & 77 $\pm$ 4 & 5.4 $_{- 0.6}^{+ 0.5}$ & $I$ \\
V2080 Cyg B & 4.2 $\pm$ 0.1 & 3.61 $\pm$ 0.06 & -0.060 $\pm$ 0.008 & 1.26 $\pm$ 0.04 & MS & 22 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V2080 Cyg A & 4.21 $\pm$ 0.10 & 3.60 $\pm$ 0.06 & -0.059 $\pm$ 0.008 & 1.25 $\pm$ 0.05 & MS & 24 & 78 $\pm$ 4 & 5.4 $_{- 0.5}^{+ 0.5}$ & $I$ \\
V2080 Cyg B & 4.25 $\pm$ 0.08 & 3.64 $\pm$ 0.06 & -0.075 $\pm$ 0.013 & 1.10 $\pm$ 0.06 & SGB & 78 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V2080 Cyg A & 4.21 $\pm$ 0.10 & 3.60 $\pm$ 0.06 & -0.059 $\pm$ 0.008 & 1.25 $\pm$ 0.05 & MS & 24 & 78 $\pm$ 4 & 3.85 $_{- 0.3}^{+ 0.28}$ & $I$ \\
V2080 Cyg B & 4.2 $\pm$ 0.1 & 3.61 $\pm$ 0.06 & -0.060 $\pm$ 0.008 & 1.26 $\pm$ 0.04 & MS & 22 & $\shortparallel$ & $\shortparallel$ & $I$ \\
FL Lyr A & 4.55 $\pm$ 0.12 & 3.99 $\pm$ 0.09 & -0.061 $\pm$ 0.015 & 1.11 $\pm$ 0.09 & MS & 100 & 134 $\pm$ 8 & 6.0 $_{- 2.0}^{+ 2.3}$ & $I$ \\
FL Lyr B & 6.20 $\pm$ 0.15 & 5.37 $\pm$ 0.12 & -0.196 $\pm$ 0.025 & 0.90 $\pm$ 0.04 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V2154 Cyg A & 3.64 $\pm$ 0.14 & 3.24 $\pm$ 0.11 & -0.025 $\pm$ 0.017 & 1.35 $\pm$ 0.09 & MS & 99 & 85 $\pm$ 4 & 1.3 $_{- 0.7}^{+ 0.9}$ & $I$ \\
V2154 Cyg B & 7.38 $\pm$ 0.25 & 6.45 $\pm$ 0.19 & -0.36 $\pm$ 0.07 & 0.769 $\pm$ 0.030 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V1061 Cyg A & 3.97 $\pm$ 0.10 & 3.44 $\pm$ 0.07 & -0.051 $\pm$ 0.011 & 1.24 $\pm$ 0.08 & MS & 62 & 154 $\pm$ 7 & 3.5 $_{- 0.6}^{+ 1.9}$ & $I$ \\
V1061 Cyg B & 6.05 $\pm$ 0.17 & 5.25 $\pm$ 0.13 & -0.176 $\pm$ 0.029 & 0.92 $\pm$ 0.04 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V1061 Cyg A & 4.06 $\pm$ 0.11 & 3.50 $\pm$ 0.08 & -0.064 $\pm$ 0.013 & 1.13 $\pm$ 0.07 & SGB & 38 & 153 $\pm$ 7 & 6.3 $_{- 1.6}^{+ 1.0}$ & $I$ \\
V1061 Cyg B & 6.05 $\pm$ 0.17 & 5.25 $\pm$ 0.13 & -0.176 $\pm$ 0.029 & 0.92 $\pm$ 0.04 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CF Tau A & 4.29 $\pm$ 0.17 & 3.41 $\pm$ 0.12 & -0.30 $\pm$ 0.04 & 1.11 $\pm$ 0.12 & RGB & 70 & 216 $\pm$ 23 & 4.24 $_{- 0.25}^{+ 1.0}$ & $I$ \\
CF Tau B & 3.71 $\pm$ 0.16 & 3.11 $\pm$ 0.12 & -0.076 $\pm$ 0.019 & 1.22 $\pm$ 0.06 & SGB & 63 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CF Tau A & 4.29 $\pm$ 0.17 & 3.41 $\pm$ 0.12 & -0.30 $\pm$ 0.04 & 1.11 $\pm$ 0.12 & RGB & 70 & 215 $\pm$ 22 & 3.85 $_{-undef.}^{+ 0.19}$ & $I$ \\
CF Tau B & 3.60 $\pm$ 0.16 & 3.01 $\pm$ 0.10 & -0.054 $\pm$ 0.013 & 1.40 $\pm$ 0.04 & MS & 37 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CF Tau A & 4.00 $\pm$ 0.16 & 3.17 $\pm$ 0.12 & -0.23 $\pm$ 0.03 & 1.32 $\pm$ 0.07 & SGB & 30 & 226 $\pm$ 24 & 4.0 $_{- 0.3}^{+ 0.5}$ & $I$ \\
CF Tau B & 3.71 $\pm$ 0.16 & 3.11 $\pm$ 0.12 & -0.076 $\pm$ 0.019 & 1.22 $\pm$ 0.06 & SGB & 63 & $\shortparallel$ & $\shortparallel$ & $I$ \\
CF Tau A & 4.00 $\pm$ 0.16 & 3.17 $\pm$ 0.12 & -0.23 $\pm$ 0.03 & 1.32 $\pm$ 0.07 & SGB & 30 & 225 $\pm$ 24 & 3.33 $_{- 0.16}^{+ 0.29}$ & $I$ \\
CF Tau B & 3.60 $\pm$ 0.16 & 3.01 $\pm$ 0.10 & -0.054 $\pm$ 0.013 & 1.40 $\pm$ 0.04 & MS & 37 & $\shortparallel$ & $\shortparallel$ & $I$ \\
HS Hya A & 4.16 $\pm$ 0.05 & 3.71 $\pm$ 0.04 & -0.042 $\pm$ 0.013 & 1.23 $\pm$ 0.07 & MS & 99 & 101 $\pm$ 4 & 1.3 $_{- 0.7}^{+ 1.1}$ & $I$ \\
HS Hya B & 4.37 $\pm$ 0.05 & 3.89 $\pm$ 0.04 & -0.049 $\pm$ 0.013 & 1.18 $\pm$ 0.07 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
UZ Dra A & 4.44 $\pm$ 0.13 & 3.91 $\pm$ 0.10 & -0.057 $\pm$ 0.015 & 1.13 $\pm$ 0.09 & MS & 100 & 171 $\pm$ 13 & 4.0 $_{- 1.5}^{+ 1.9}$ & $I$ \\
UZ Dra B & 4.98 $\pm$ 0.13 & 4.36 $\pm$ 0.10 & -0.078 $\pm$ 0.015 & 1.04 $\pm$ 0.09 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V1143 Cyg A & 4.13 $\pm$ 0.11 & 3.66 $\pm$ 0.08 & -0.042 $\pm$ 0.016 & 1.22 $\pm$ 0.09 & MS & 100 & 37.8 $\pm$ 2.7 & 2.1 $_{- 0.9}^{+ 1.1}$ & $I$ \\
V1143 Cyg B & 4.22 $\pm$ 0.11 & 3.74 $\pm$ 0.09 & -0.045 $\pm$ 0.015 & 1.20 $\pm$ 0.09 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
VZ Cep A & 3.65 $\pm$ 0.14 & 3.23 $\pm$ 0.11 & -0.029 $\pm$ 0.018 & 1.33 $\pm$ 0.09 & MS & 99 & 205 $\pm$ 13 & 1.9 $_{- 0.7}^{+ 1.1}$ & $I$ \\
VZ Cep B & 5.51 $\pm$ 0.16 & 4.82 $\pm$ 0.13 & -0.113 $\pm$ 0.018 & 0.96 $\pm$ 0.07 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
BF Dra A & 3.25 $\pm$ 0.15 & 2.76 $\pm$ 0.11 & -0.037 $\pm$ 0.015 & 1.44 $\pm$ 0.06 & MS & 75 & 320 $\pm$ 30 & 2.6 $_{- 0.3}^{+ 0.3}$ & $I$ \\
BF Dra B & 3.39 $\pm$ 0.14 & 2.91 $\pm$ 0.10 & -0.036 $\pm$ 0.015 & 1.40 $\pm$ 0.06 & MS & 72 & $\shortparallel$ & $\shortparallel$ & $I$ \\
BF Dra A & 3.25 $\pm$ 0.15 & 2.76 $\pm$ 0.11 & -0.037 $\pm$ 0.015 & 1.44 $\pm$ 0.06 & MS & 75 & 322 $\pm$ 30 & 3.33 $_{- 0.16}^{+ 0.3}$ & $I$ \\
BF Dra B & 3.49 $\pm$ 0.13 & 3.00 $\pm$ 0.09 & -0.057 $\pm$ 0.010 & 1.22 $\pm$ 0.05 & SGB & 27 & $\shortparallel$ & $\shortparallel$ & $I$ \\
BF Dra A & 3.37 $\pm$ 0.15 & 2.87 $\pm$ 0.10 & -0.059 $\pm$ 0.011 & 1.25 $\pm$ 0.05 & SGB & 25 & 315 $\pm$ 29 & 3.49 $_{- 0.20}^{+ 0.17}$ & $I$ \\
BF Dra B & 3.39 $\pm$ 0.14 & 2.91 $\pm$ 0.10 & -0.036 $\pm$ 0.015 & 1.40 $\pm$ 0.06 & MS & 72 & $\shortparallel$ & $\shortparallel$ & $I$ \\
    \hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleIIb:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    Binary & $M_B$       &  $M_V$         & $BC$        &    $M_m$          & $ES$  &  $Pr$    & $d_m$      &  $\tau$  & Grid \\
                 & ($mag$)     & ($mag$)        &  ($mag$)  &    ($M_{\sun}$)  &            &              & ($pc$)      & ($Gyr$)  &        \\
    \hline
BF Dra A & 3.37 $\pm$ 0.15 & 2.87 $\pm$ 0.10 & -0.059 $\pm$ 0.011 & 1.25 $\pm$ 0.05 & SGB & 25 & 317 $\pm$ 30 & 3.67 $_{- 0.17}^{+ 0.4}$ & $I$ \\
BF Dra B & 3.49 $\pm$ 0.13 & 3.00 $\pm$ 0.09 & -0.057 $\pm$ 0.010 & 1.22 $\pm$ 0.05 & SGB & 27 & $\shortparallel$ & $\shortparallel$ & $I$ \\
DM Vir A & 3.48 $\pm$ 0.10 & 3.03 $\pm$ 0.08 & -0.032 $\pm$ 0.015 & 1.37 $\pm$ 0.07 & MS & 80 & 183 $\pm$ 13 & 2.4 $_{- 0.3}^{+ 0.4}$ & $I$ \\
DM Vir B & 3.48 $\pm$ 0.10 & 3.03 $\pm$ 0.08 & -0.032 $\pm$ 0.015 & 1.37 $\pm$ 0.07 & MS & 80 & $\shortparallel$ & $\shortparallel$ & $I$ \\
DM Vir A & 3.48 $\pm$ 0.10 & 3.03 $\pm$ 0.08 & -0.032 $\pm$ 0.015 & 1.37 $\pm$ 0.07 & MS & 80 & 184 $\pm$ 13 & 3.49 $_{- 0.17}^{+ 0.25}$ & $I$ \\
DM Vir B & 3.54 $\pm$ 0.10 & 3.10 $\pm$ 0.07 & -0.056 $\pm$ 0.008 & 1.19 $\pm$ 0.04 & SGB & 20 & $\shortparallel$ & $\shortparallel$ & $I$ \\
DM Vir A & 3.54 $\pm$ 0.10 & 3.10 $\pm$ 0.07 & -0.056 $\pm$ 0.008 & 1.19 $\pm$ 0.04 & SGB & 20 & 180 $\pm$ 12 & 3.49 $_{- 0.17}^{+ 0.25}$ & $I$ \\
DM Vir B & 3.48 $\pm$ 0.10 & 3.03 $\pm$ 0.08 & -0.032 $\pm$ 0.015 & 1.37 $\pm$ 0.07 & MS & 80 & $\shortparallel$ & $\shortparallel$ & $I$ \\
DM Vir A & 3.54 $\pm$ 0.10 & 3.10 $\pm$ 0.07 & -0.056 $\pm$ 0.008 & 1.19 $\pm$ 0.04 & SGB & 20 & 181 $\pm$ 12 & 3.85 $_{- 0.25}^{+ 0.3}$ & $I$ \\
DM Vir B & 3.54 $\pm$ 0.10 & 3.10 $\pm$ 0.07 & -0.056 $\pm$ 0.008 & 1.19 $\pm$ 0.04 & SGB & 20 & $\shortparallel$ & $\shortparallel$ & $I$ \\
HD 71636 A & 3.34 $\pm$ 0.11 & 2.98 $\pm$ 0.09 & -0.015 $\pm$ 0.016 & 1.43 $\pm$ 0.08 & MS & 99 & 118 $\pm$ 7 & 1.5 $_{- 0.6}^{+ 0.5}$ & $I$ \\
HD 71636 B & 4.12 $\pm$ 0.13 & 3.65 $\pm$ 0.10 & -0.043 $\pm$ 0.016 & 1.22 $\pm$ 0.09 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
RZ Cha A & 2.98 $\pm$ 0.14 & 2.52 $\pm$ 0.11 & -0.031 $\pm$ 0.016 & 1.50 $\pm$ 0.07 & MS & 91 & 170 $\pm$ 16 & 2.36 $_{- 0.3}^{+ 0.26}$ & $I$ \\
RZ Cha B & 2.98 $\pm$ 0.14 & 2.52 $\pm$ 0.11 & -0.031 $\pm$ 0.016 & 1.50 $\pm$ 0.07 & MS & 91 & $\shortparallel$ & $\shortparallel$ & $I$ \\
EY Cep A & 3.40 $\pm$ 0.13 & 3.06 $\pm$ 0.10 & -0.019 $\pm$ 0.013 & 1.41 $\pm$ 0.08 & MS & 99 & 283 $\pm$ 26 & 0.5 $_{- 0.3}^{+ 0.6}$ & $I$ \\
EY Cep B & 3.50 $\pm$ 0.13 & 3.14 $\pm$ 0.10 & -0.021 $\pm$ 0.014 & 1.39 $\pm$ 0.08 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V442 Cyg A & 2.76 $\pm$ 0.09 & 2.40 $\pm$ 0.08 & -0.010 $\pm$ 0.016 & 1.55 $\pm$ 0.08 & MS & 99 & 321 $\pm$ 19 & 1.68 $_{- 0.29}^{+ 0.3}$ & $I$ \\
V442 Cyg B & 3.34 $\pm$ 0.09 & 2.95 $\pm$ 0.08 & -0.019 $\pm$ 0.016 & 1.41 $\pm$ 0.08 & MS & 98 & $\shortparallel$ & $\shortparallel$ & $I$ \\
PV Pup A & 3.48 $\pm$ 0.26 & 3.10 $\pm$ 0.20 & -0.022 $\pm$ 0.020 & 1.38 $\pm$ 0.11 & MS & 99 & 80 $\pm$ 13 & 1.1 $_{- 0.5}^{+ 0.7}$ & $I$ \\
PV Pup B & 3.54 $\pm$ 0.26 & 3.16 $\pm$ 0.20 & -0.024 $\pm$ 0.018 & 1.37 $\pm$ 0.11 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
FS Mon A & 2.95 $\pm$ 0.09 & 2.55 $\pm$ 0.07 & -0.019 $\pm$ 0.016 & 1.50 $\pm$ 0.08 & MS & 98 & 304 $\pm$ 16 & 2.0 $_{- 0.3}^{+ 0.3}$ & $I$ \\
FS Mon B & 3.62 $\pm$ 0.10 & 3.18 $\pm$ 0.08 & -0.033 $\pm$ 0.017 & 1.32 $\pm$ 0.08 & MS & 93 & $\shortparallel$ & $\shortparallel$ & $I$ \\
IO Aqr A & 2.88 $\pm$ 0.13 & 2.39 $\pm$ 0.09 & -0.037 $\pm$ 0.014 & 1.53 $\pm$ 0.07 & MS & 94 & 234 $\pm$ 18 & 2.36 $_{- 0.30}^{+ 0.24}$ & $I$ \\
IO Aqr B & 3.03 $\pm$ 0.13 & 2.58 $\pm$ 0.10 & -0.030 $\pm$ 0.016 & 1.48 $\pm$ 0.07 & MS & 90 & $\shortparallel$ & $\shortparallel$ & $I$ \\
EI Cep A & 2.17 $\pm$ 0.11 & 1.78 $\pm$ 0.09 & -0.010 $\pm$ 0.017 & 1.73 $\pm$ 0.09 & MS & 99 & 185 $\pm$ 12 & 1.52 $_{- 0.16}^{+ 0.18}$ & $I$ \\
EI Cep B & 2.46 $\pm$ 0.09 & 2.11 $\pm$ 0.08 & -0.005 $\pm$ 0.016 & 1.64 $\pm$ 0.09 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
XY Cet A & 2.24 $\pm$ 0.09 & 2.04 $\pm$ 0.07 & 0.003 $\pm$ 0.013 & 1.72 $\pm$ 0.09 & MS & 100 & 277 $\pm$ 19 & 0.89 $_{- 0.23}^{+ 0.24}$ & $I$ \\
XY Cet B & 2.54 $\pm$ 0.10 & 2.30 $\pm$ 0.08 & 0.002 $\pm$ 0.014 & 1.63 $\pm$ 0.09 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
MY Cyg A & 2.47 $\pm$ 0.17 & 2.13 $\pm$ 0.13 & -0.004 $\pm$ 0.017 & 1.63 $\pm$ 0.09 & MS & 100 & 226 $\pm$ 26 & 1.45 $_{- 0.20}^{+ 0.27}$ & $I$ \\
MY Cyg B & 2.47 $\pm$ 0.17 & 2.14 $\pm$ 0.13 & -0.002 $\pm$ 0.017 & 1.63 $\pm$ 0.10 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
HY Vir A & 2.14 $\pm$ 0.11 & 1.77 $\pm$ 0.09 & -0.005 $\pm$ 0.017 & 1.74 $\pm$ 0.09 & MS & 100 & 170 $\pm$ 8 & 1.52 $_{- 0.20}^{+ 0.23}$ & $I$ \\
HY Vir B & 3.78 $\pm$ 0.12 & 3.33 $\pm$ 0.09 & -0.036 $\pm$ 0.018 & 1.29 $\pm$ 0.09 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
WW Aur A & 2.2 $\pm$ 0.3 & 2.00 $\pm$ 0.24 & -0.005 $\pm$ 0.022 & 1.74 $\pm$ 0.14 & MS & 100 & 78 $\pm$ 15 & 0.89 $_{- 0.24}^{+ 0.3}$ & $I$ \\
WW Aur B & 2.5 $\pm$ 0.3 & 2.26 $\pm$ 0.25 & -0.003 $\pm$ 0.017 & 1.64 $\pm$ 0.13 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V2365 Oph A & 1.07 $\pm$ 0.07 & 1.06 $\pm$ 0.05 & -0.18 $\pm$ 0.04 & 2.23 $\pm$ 0.12 & MS & 99 & 251 $\pm$ 13 & 0.41 $_{- 0.12}^{+ 0.15}$ & $I$ \\
V2365 Oph B & 5.33 $\pm$ 0.17 & 4.77 $\pm$ 0.11 & -0.093 $\pm$ 0.010 & 0.98 $\pm$ 0.05 & MS & 96 & $\shortparallel$ & $\shortparallel$ & $I$ \\
VV Crv A & 2.07 $\pm$ 0.17 & 1.62 $\pm$ 0.12 & -0.020 $\pm$ 0.015 & 1.80 $\pm$ 0.08 & MS & 98 & 59 $\pm$ 4 & 1.52 $_{- 0.19}^{+ 0.23}$ & $I$ \\
VV Crv B & 3.52 $\pm$ 0.18 & 3.09 $\pm$ 0.14 & -0.028 $\pm$ 0.018 & 1.36 $\pm$ 0.09 & MS & 89 & $\shortparallel$ & 1.52 $_{- 0.19}^{+ 0.23}$ & $I$ \\
VV Crv A & 2.07 $\pm$ 0.17 & 1.62 $\pm$ 0.12 & -0.020 $\pm$ 0.015 & 1.80 $\pm$ 0.08 & MS & 98 & 59 $\pm$ 4 & 1.52 $_{- 0.18}^{+ 0.18}$ & $I$ \\
VV Crv B & 3.72 $\pm$ 0.17 & 3.26 $\pm$ 0.12 & -0.057 $\pm$ 0.010 & 1.17 $\pm$ 0.05 & SGB & 10 & $\shortparallel$ & 4.3 $_{- 0.8}^{+ 0.8}$ & $I$ \\
KW Hya A & 1.88 $\pm$ 0.14 & 1.70 $\pm$ 0.11 & 0.002 $\pm$ 0.014 & 1.83 $\pm$ 0.10 & MS & 100 & 84 $\pm$ 5 & 0.89 $_{- 0.21}^{+ 0.25}$ & $I$ \\
KW Hya B & 3.54 $\pm$ 0.15 & 3.16 $\pm$ 0.12 & -0.022 $\pm$ 0.016 & 1.38 $\pm$ 0.09 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
    \hline
  \end{tabular}
%}
 \end{table}
\end{landscape}

\begin{landscape}
 \begin{table}
  \contcaption{}
  \label{tab:sampleIIb:continued}
  \begin{tabular}{ccccccccccc}
    \hline
    Binary & $M_B$       &  $M_V$         & $BC$        &    $M_m$          & $ES$  &  $Pr$    & $d_m$      &  $\tau$  & Grid \\
                 & ($mag$)     & ($mag$)        &  ($mag$)  &    ($M_{\sun}$)  &            &              & ($pc$)      & ($Gyr$)  &        \\
    \hline
TV Nor A & 1.60 $\pm$ 0.06 & 1.55 $\pm$ 0.05 & -0.114 $\pm$ 0.027 & 2.01 $\pm$ 0.11 & MS & 100 & 268 $\pm$ 15 & 0.39 $_{- 0.18}^{+ 0.20}$ & $I$ \\
TV Nor B & 2.72 $\pm$ 0.08 & 2.49 $\pm$ 0.06 & -0.007 $\pm$ 0.010 & 1.60 $\pm$ 0.08 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V596 Pup A & 1.09 $\pm$ 0.07 & 1.08 $\pm$ 0.06 & -0.18 $\pm$ 0.04 & 2.23 $\pm$ 0.12 & MS & 100 & 167 $\pm$ 15 & 0.4 $_{- 0.1}^{+ 0.12}$ & $I$ \\
V596 Pup B & 1.09 $\pm$ 0.07 & 1.08 $\pm$ 0.06 & -0.18 $\pm$ 0.04 & 2.23 $\pm$ 0.12 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V335 Ser A & 1.42 $\pm$ 0.07 & 1.37 $\pm$ 0.06 & -0.096 $\pm$ 0.025 & 2.05 $\pm$ 0.11 & MS & 100 & 184 $\pm$ 12 & 0.47 $_{- 0.14}^{+ 0.17}$ & $I$ \\
V335 Ser B & 2.03 $\pm$ 0.10 & 1.91 $\pm$ 0.08 & -0.035 $\pm$ 0.018 & 1.82 $\pm$ 0.10 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
EE Peg A & 1.50 $\pm$ 0.10 & 1.42 $\pm$ 0.08 & -0.053 $\pm$ 0.027 & 2.00 $\pm$ 0.11 & MS & 100 & 133 $\pm$ 8 & 0.60 $_{- 0.17}^{+ 0.21}$ & $I$ \\
EE Peg B & 4.28 $\pm$ 0.26 & 3.78 $\pm$ 0.19 & -0.050 $\pm$ 0.019 & 1.18 $\pm$ 0.11 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V1647 Sgr A & 1.46 $\pm$ 0.11 & 1.44 $\pm$ 0.09 & -0.19 $\pm$ 0.06 & 2.11 $\pm$ 0.13 & MS & 100 & 157 $\pm$ 18 & 0.24 $_{- 0.12}^{+ 0.17}$ & $I$ \\
V1647 Sgr B & 1.86 $\pm$ 0.13 & 1.80 $\pm$ 0.10 & -0.11 $\pm$ 0.05 & 1.91 $\pm$ 0.11 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
PT Vel A & 1.26 $\pm$ 0.06 & 1.23 $\pm$ 0.05 & -0.134 $\pm$ 0.029 & 2.14 $\pm$ 0.11 & MS & 100 & 155 $\pm$ 7 & 0.47 $_{- 0.15}^{+ 0.16}$ & $I$ \\
PT Vel B & 2.83 $\pm$ 0.13 & 2.58 $\pm$ 0.11 & -0.006 $\pm$ 0.012 & 1.57 $\pm$ 0.08 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
GZ CMa A & 1.09 $\pm$ 0.17 & 1.02 $\pm$ 0.13 & -0.06 $\pm$ 0.05 & 2.14 $\pm$ 0.14 & MS & 100 & 280 $\pm$ 39 & 0.63 $_{- 0.12}^{+ 0.15}$ & $I$ \\
GZ CMa B & 1.58 $\pm$ 0.19 & 1.47 $\pm$ 0.15 & -0.03 $\pm$ 0.03 & 1.96 $\pm$ 0.13 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V624 Her A & 0.98 $\pm$ 0.10 & 0.84 $\pm$ 0.08 & 0.004 $\pm$ 0.015 & 2.14 $\pm$ 0.11 & MS & 100 & 139 $\pm$ 8 & 0.81 $_{- 0.10}^{+ 0.11}$ & $I$ \\
V624 Her B & 1.82 $\pm$ 0.11 & 1.64 $\pm$ 0.08 & 0.006 $\pm$ 0.013 & 1.84 $\pm$ 0.10 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
$\beta$ Aur A & 0.61 $\pm$ 0.07 & 0.60 $\pm$ 0.06 & -0.15 $\pm$ 0.04 & 2.38 $\pm$ 0.12 & MS & 100 & 23.7 $\pm$ 1.9 & 0.50 $_{- 0.06}^{+ 0.09}$ & $I$ \\
$\beta$ Aur B & 0.82 $\pm$ 0.08 & 0.80 $\pm$ 0.06 & -0.13 $\pm$ 0.04 & 2.28 $\pm$ 0.12 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V1031 Ori A & 0.5 $\pm$ 0.4 & 0.29 $\pm$ 0.27 & 0.017 $\pm$ 0.024 & 2.37 $\pm$ 0.16 & MS & 99 & 180 $\pm$ 37 & 0.70 $_{- 0.11}^{+ 0.13}$ & $I$ \\
V1031 Ori B & 1.0 $\pm$ 0.3 & 0.84 $\pm$ 0.24 & -0.02 $\pm$ 0.05 & 2.16 $\pm$ 0.17 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
TZ Men A & 1.01 $\pm$ 0.11 & 1.05 $\pm$ 0.09 & -0.35 $\pm$ 0.08 & 2.39 $\pm$ 0.16 & MS & 100 & 109 $\pm$ 10 & 0.22 $_{- 0.10}^{+ 0.15}$ & $I$ \\
TZ Men B & 3.46 $\pm$ 0.24 & 3.12 $\pm$ 0.19 & -0.023 $\pm$ 0.013 & 1.39 $\pm$ 0.09 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
AR Aur A & 1.13 $\pm$ 0.07 & 1.18 $\pm$ 0.06 & -0.47 $\pm$ 0.06 & 2.40 $\pm$ 0.12 & MS & 99 & 129 $\pm$ 14 & 0.09 $_{- 0.05}^{+ 0.10}$ & $I$ \\
AR Aur B & 1.23 $\pm$ 0.09 & 1.26 $\pm$ 0.07 & -0.34 $\pm$ 0.06 & 2.29 $\pm$ 0.12 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V4089 Sgr A & 0.20 $\pm$ 0.05 & 0.12 $\pm$ 0.04 & -0.015 $\pm$ 0.014 & 2.47 $\pm$ 0.11 & MS & 99 & 146 $\pm$ 4 & 0.57 $_{- 0.05}^{+ 0.07}$ & $I$ \\
V4089 Sgr B & 2.95 $\pm$ 0.08 & 2.67 $\pm$ 0.06 & -0.004 $\pm$ 0.014 & 1.53 $\pm$ 0.08 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V451 Oph A & 0.37 $\pm$ 0.21 & 0.42 $\pm$ 0.18 & -0.39 $\pm$ 0.16 & 2.68 $\pm$ 0.26 & MS & 100 & 291 $\pm$ 59 & 0.30 $_{- 0.09}^{+ 0.11}$ & $I$ \\
V451 Oph B & 1.19 $\pm$ 0.17 & 1.19 $\pm$ 0.13 & -0.2 $\pm$ 0.1 & 2.23 $\pm$ 0.17 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
$\psi$ Cen A & -0.31 $\pm$ 0.08 & -0.25 $\pm$ 0.06 & -0.37 $\pm$ 0.06 & 2.97 $\pm$ 0.15 & MS & 100 & 74 $\pm$ 5 & 0.32 $_{- 0.05}^{+ 0.05}$ & $I$ \\
$\psi$ Cen B & 1.82 $\pm$ 0.15 & 1.73 $\pm$ 0.12 & -0.06 $\pm$ 0.04 & 1.91 $\pm$ 0.12 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
IQ Per A & 0.16 $\pm$ 0.05 & 0.26 $\pm$ 0.05 & -0.74 $\pm$ 0.05 & 3.12 $\pm$ 0.16 & MS & 100 & 252 $\pm$ 12 & 0.14 $_{- 0.05}^{+ 0.07}$ & $I$ \\
IQ Per B & 2.88 $\pm$ 0.10 & 2.64 $\pm$ 0.09 & -0.010 $\pm$ 0.009 & 1.54 $\pm$ 0.07 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
$\chi^2$ Hya A & -0.99 $\pm$ 0.06 & -0.90 $\pm$ 0.05 & -0.61 $\pm$ 0.05 & 3.61 $\pm$ 0.16 & MS & 100 & 210 $\pm$ 13 & 0.196 $_{- 0.023}^{+ 0.029}$ & $I$ \\
$\chi^2$ Hya B & 0.70 $\pm$ 0.07 & 0.76 $\pm$ 0.07 & -0.48 $\pm$ 0.05 & 2.62 $\pm$ 0.15 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
$\zeta$ Phe A & -0.53 $\pm$ 0.05 & -0.39 $\pm$ 0.05 & -1.15 $\pm$ 0.06 & 4.02 $\pm$ 0.21 & MS & 100 & 76 $\pm$ 4 & 0.070 $_{- 0.027}^{+ 0.03}$ & $I$ \\
$\zeta$ Phe B & 0.85 $\pm$ 0.05 & 0.94 $\pm$ 0.04 & -0.67 $\pm$ 0.04 & 2.66 $\pm$ 0.10 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
GG Lup A & -0.14 $\pm$ 0.06 & -0.01 $\pm$ 0.06 & -1.18 $\pm$ 0.08 & 3.80 $\pm$ 0.20 & MS & 100 & 135 $\pm$ 10 & 0.025 $_{- 0.012}^{+ 0.04}$ & $I$ \\
GG Lup B & 1.28 $\pm$ 0.15 & 1.32 $\pm$ 0.12 & -0.43 $\pm$ 0.12 & 2.30 $\pm$ 0.15 & MS & 99 & $\shortparallel$ & $\shortparallel$ & $I$ \\
V760 Sco A & -0.94 $\pm$ 0.08 & -0.77 $\pm$ 0.07 & -1.53 $\pm$ 0.08 & 4.95 $\pm$ 0.28 & MS & 100 & 275 $\pm$ 32 & 0.029 $_{- 0.013}^{+ 0.018}$ & $I$ \\
V760 Sco B & -0.56 $\pm$ 0.07 & -0.40 $\pm$ 0.07 & -1.42 $\pm$ 0.08 & 4.45 $\pm$ 0.24 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
U Oph A & -1.19 $\pm$ 0.04 & -1.02 $\pm$ 0.03 & -1.46 $\pm$ 0.04 & 4.99 $\pm$ 0.22 & MS & 100 & 224 $\pm$ 14 & 0.058 $_{- 0.014}^{+ 0.014}$ & $I$ \\
U Oph B & -0.86 $\pm$ 0.04 & -0.71 $\pm$ 0.04 & -1.33 $\pm$ 0.04 & 4.51 $\pm$ 0.21 & MS & 100 & $\shortparallel$ & $\shortparallel$ & $I$ \\
    \hline
  \end{tabular}
%}
 \end{table}
\end{landscape}


